Generalized multi-view model: Adaptive density estimation under low-rank constraints

We study the problem of bivariate discrete or continuous probability density estimation under low-rank constraints.For discrete distributions, we assume that the two-dimensional array to estimate is a low-rank probability matrix. In the continuous case, we assume that the density with respect to the Lebesgue measure satisfies a generalized multi-view model, meaning that it is $\beta$-H{\"o}lder and can be decomposed as a sum of $K$ components, each of which is a product of one-dimensional functions. In both settings, we propose estimators that achieve, up to logarithmic factors, the minimax optimal convergence rates under such low-rank constraints. In the discrete case, the proposed estimator is adaptive to the rank $K$. In the continuous case, our estimator converges with the $L_1$ rate $\min((K/n)^{\beta/(2\beta+1)}, n^{-\beta/(2\beta+2)})$ up to logarithmic factors, and it is adaptive to the unknown support as well as to the smoothness $\beta$ and to the unknown number of separable components $K$. We present efficient algorithms for computing our estimators.

==> contents_low_rank/Bound_stoch.tex <==
\subsection{Controlling the multinomial noise}

For a matrix $M\in \mathbb{R}^{d_1\times d_2}$ we write for short $\| M\|_{1} = \|M\|_{1,\infty}$ to denote the maximum absolute column sum norm, that is
\begin{equation*}
	\| M\|_{1}=\underset{j}{\max}\sum_{i=1}^{d_1}| M_{ij}|.
\end{equation*}
We also write $\| M\|$ for the operator norm.
\begin{lemma}\label{lemma:bound_Poisson_matrix}
	Let $W=(w_{ij}-\lambda_{ij})_{(ij)\in \nint{d_1}\times\nint{d_2}}$ where $w_{ij}\sim \Poi(\lambda_{ij})$ are independent. 
	We set $\Lambda= (\lambda_{ij})_{(ij)\in \nint{d_1}\times\nint{d_2}}$, $\lambda= 1 \lor \hspace{-3mm} \underset {(ij)\in \nint{d_1}\times\nint{d_2}} {\max } \lambda_{ij} $,  $d=d_1\vee d_2$. 
	Then, for any $\alpha > 0$, there exists a constant $c>0$ depending only on $\alpha$ such that with probability at least $1-1/d^\alpha$,
	$$\|W\|_{op} \leq c\max\left\lbrace \sqrt{(1+\alpha)\| \Lambda^{T}\|_{1}\vee \| \Lambda\|_{1}\log (d)},\; (1+\alpha)\sqrt{\lambda}\log(d)\log\left(\frac{2\sqrt{\lambda}}{\sqrt{\| \Lambda^{T}\|_{1}\vee \| \Lambda\|_{1}}}\right) \right\rbrace.$$
\end{lemma}
Noting that $\frac{2\sqrt{\lambda}}{\sqrt{\| \Lambda^{T}\|_{1}\vee \| \Lambda\|_{1}}} \leq 2$, the second term in the maximum is dominated by the first one, which yields the following Corollary:

\vspace{2mm}

\begin{corollary}\label{cor:poisson_noise}
Set $c' = 2  \barc \alpha \log2$ where $\barc$ is the constant from Lemma~\ref{lem:concent_poisson}. Under the same assumptions as in Lemma~\ref{lemma:bound_Poisson_matrix}, for any $\alpha>0$, there exist constants $c^*>0$ depending only on $\alpha$ such that, if $\normsquare{\Lambda} \geq c'$, then with probability at least $1 - d^{-\alpha}$ we have 
$$ \|W\|_{op}^2 \leq c^* \normsquare{\Lambda} \log^2 d. $$
\end{corollary}

\begin{proof}[Proof of Corollary~\ref{cor:poisson_noise}]
Using the same notation as in Lemma~\ref{lemma:bound_Poisson_matrix}, we have 
$$\lambda = 1 \lor \max_{i,j} \lambda_{ij} \leq 1 \lor \normsquare{\Lambda} \leq \frac{\normsquare{\Lambda}}{c'} .$$
Therefore,
\begin{align*}
    (1+\alpha)\sqrt{\lambda}\log(d)\log\left(\frac{2\sqrt{\lambda}}{\sqrt{\| \Lambda^{T}\|_{1}\vee \| \Lambda\|_{1}}}\right) &\leq (1+\alpha) \sqrt{\frac{\normsquare{\Lambda}}{c'}} \log (d) \log\left(\frac{2}{\sqrt{c'}}\right)\\
    & \leq \sqrt{c^* \normsquare{\Lambda} \log^2 d}
\end{align*}
where at the last line, we set $c^* =  \frac{(1+\alpha)^2}{c'} \log^2\left(\frac{2}{\sqrt{c'}}\right)$.

\end{proof}

\vspace{2mm}


\begin{proof}[Proof of Lemma~\ref{lemma:bound_Poisson_matrix}]
The proof is based on the following result obtained by extension of Theorem 4 in  \cite{Koltchinskii2013} to rectangular matrices.
\begin{proposition}
	\label{prop:Koltchinskii2013}
	Let $W_{1},\ldots , W_n$ be independent random matrices with dimensions $d_1\times d_2$ that satisfy $\E[{W_i}]=0$. Suppose that
	\begin{equation}
		\delta_* = \sup_{i\in\nint{n}}\inf_{\delta>0} \left\lbrace\E[\exp\left(\|W_i\|/\delta\right)]\leq e\right\rbrace<+\infty.
	\end{equation}
	Then, there exists an absolute constant $c^*$ such that, for all $t>0$ and with probability at least $1-e^{-t}$ we have
	$$\left\|\frac{1}{n}\sum_{i=1}^nW_i\right\|\leq c^*\max\left\lbrace \sigma_W\sqrt{\frac{t+\log d}{n}}, \delta_*\left(\log\frac{\delta_*}{\sigma_W}\right)\frac{t+\log d}{n} \right\rbrace,$$
	where
	$$\sigma_W = \max\left\lbrace \left\|\frac{1}{n}\sum_{i=1}^{n}\E[W_{i}W_{i}^{\top}]\right\|^{1/2},\left\|\frac{1}{n}\sum_{i=1}^{n}\E[W_{i}^{\top}W_{i}]\right\|^{1/2} \right \rbrace.$$
\end{proposition}
For all $(i,j)\in\nint{d_1}\times\nint{d_2}$ define $Z_{ij} = \left(w_{ij}-\lambda_{ij}\right)E_{ij}$ where $E_{ij}$ are the matrices of the canonical basis of $\mathbb{R}^{d_1\times d_2}$.  The sub-exponentiality of the centered Poisson variables $w_{ij}-\lambda_{ij}$ implies that for all $i,j\in\nint{d_1}\times \nint{d_2}$
$$\delta_{ij}={\operatorname{inf}}_{\delta>0}\quad \left\lbrace\E[\exp\left(\left|w_{ij}-\lambda_{ij}\right|/\delta\right)]\leq e\right\rbrace\leq 2\sqrt{\lambda_{ij}}\vee \frac{-2}{\log \lambda_{ij}}\leq 2\sqrt{\lambda}.$$
We can therefore apply Proposition \ref{prop:Koltchinskii2013} to the matrices $Z_{ij}$ defined above, with the quantity
\begin{equation}
	\label{eq:sigma-def-tail}
	\sigma_Z = \max\Bigg\lbrace \left\|\frac{1}{d_1d_2}\sum_{i=1}^{d_1}\sum_{j=1}^{d_2}\E[{Z_{ij}Z_{ij}^{\top}}]\right\|^{1/2},
	\left\|\frac{1}{d_1d_2}\sum_{i=1}^{d_1}\sum_{j=1}^{d_2}\E[{Z_{ij}^{\top}Z_{ij}}]\right\|^{1/2} \Bigg \rbrace.
\end{equation}
We obtain that for all $t\geq 0$ and with probability at least $1-e^{-t}$,
\begin{equation*}
	\|W\| \leq c^*\max\Bigg\lbrace \sigma_Z\sqrt{d_1d_2(t+\log d)},
2\sqrt{\lambda}\left (t+\log d\right )	\log\left(\frac{2\sqrt{\lambda}}{\sigma_Z}\right) \Bigg\rbrace.
\end{equation*}
We compute $\sigma_Z$  as follows:
\begin{equation*}
	\sum_{i=1}^{d_1}\sum_{j=1}^{d_2}\E[{Z_{ij}Z_{ij}^{\top}}] = \sum_{i=1}^{d_1}\left\lbrace\sum_{j=1}^{d_2}\E[{\left(  w_{ij}-\lambda_{ij}\right)^2}]\right\rbrace E_{ii}(d_1) = \sum_{i=1}^{d_1}\left\lbrace\sum_{j=1}^{d_2}\lambda_{ij}\right\rbrace E_{ii}(d_1),
\end{equation*}
where $E_{ii}(n)$, $i,n\geq 1$ denotes the $n\times n$ square matrix with $1$ in the $(i,i)$-th entry and zero everywhere else. Therefore
\begin{equation*}
	\left\|\frac{1}{d_1d_2}\sum_{i=1}^{d_1}\sum_{j=1}^{d_2}\E[{Z_{ij}Z_{ij}^{\top}}]\right\|^{1/2} = \sqrt{\frac{1}{d_1d_2}\| \Lambda^{T}\|_{1}}
\end{equation*}
and 
\begin{equation}
	\label{eq:sigma-def-tail_value}
	\sigma_Z = \sqrt{\frac{1}{d_1d_2}\| \Lambda^{T}\|_{1}\vee \| \Lambda\|_{1}} = \sqrt{\frac{1}{d_1d_2}\normsquare{\Lambda}}.
\end{equation}
Setting $t = \alpha\log d$, we  obtain that with probability at least $1-d^{-\alpha}$:
$$\|W\| \leq c^*\max\left\lbrace \sqrt{(1+\alpha)\normsquare{\Lambda}\log d},\; 2\sqrt{\lambda}\log(d)\log\left(\frac{2\sqrt{\lambda}}{\sqrt{\normsquare{\Lambda}}}\right) \right\rbrace,$$
which proves the result.
\end{proof}


The following Proposition is an adaptation of Corollary~\ref{cor:poisson_noise} to the multinomial case.
\begin{proposition}\label{prop:bound_Mult_matrix}
    Let $\alpha>0$ and $P \in \R_+^{d_1\times d_2}$ be a multinomial matrix, i.e. such that $\sum\limits_{i,j} P_{ij} = 1$, and let $H \sim \M(n,P)$ for $n \in \N^*$.
    Assume also that $n \geq \barc \alpha \log d$ where $\barc$ is the constant from Lemma~\ref{lem:concent_poisson} and $d = d_1\lor d_2$.
    Let $w = \frac{H}{n} - P$ denote the multinomial noise. 
    Let $Q$ be an extraction of $P$, that is $Q = (P_{ij})_{i\in I, j \in J}$ for some sets of indices $I \subseteq [d_1]$ and  $J \subseteq [d_2]$.
    Denote by $w_Q = (w_{ij})_{i\in I, j \in J}$.
    There exists a constant $c^*$ depending only on $\alpha$ such that 
    \begin{align*}
        \mathbb{P}\left(\|W_Q\|_{op}^2 \leq c^* \frac{\normsquare{Q}}{n} \log^2 d\right)\geq 1 - 3d^{-\alpha}.
    \end{align*}
\end{proposition}


\begin{proof}[Proof of Proposition \ref{prop:bound_Mult_matrix}]
Let $\widetilde n \sim \Poi(2n)$ and $\widetilde H | \widetilde n \sim \M(\widetilde n, P)$. 
By the Poissonization trick, we have that $\forall (i,j) \in [d_1]\times [d_2], \widetilde H_{ij} \sim \Poi(2n P_{ij})$ and the random variables $\widetilde H_{ij}$ are independent.
Letting $W = \widetilde H - 2nP$ and $W_Q = (W_{ij})_{i\in I, j \in J}$, we can therefore apply Corollary~\ref{cor:poisson_noise} to obtain
\begin{align*}
    1-d^{-\alpha} &\leq \mathbb{P}\left(\|W_Q\|_{op}^2 \leq c^* \normsquare{2nQ} \log^2 d\right)\\
    &\leq \mathbb{P}\left(\widetilde n < n\right) + \mathbb{P}\left(\|W_Q\|_{op}^2 \leq c^* \normsquare{2nQ} \log^2 d ~\Big|~ \widetilde n \geq n\right)\\
    & \leq 2e^{-\frac{c}{4} n} + \mathbb{P}\left(\|W_Q\|_{op}^2 \leq c^* \normsquare{2nQ} \log^2 d ~\Big|~ \widetilde n = n\right) ~~ \text{ by~\cite{vershynin2018high} exercise 2.3.6}\\
    & \leq \frac{2}{d^{4\alpha}} +  \mathbb{P}\left(\|w_Q\|^2_{op} \leq 2 c^* \frac{\normsquare{Q}}{n} \log^2 d\right),
\end{align*}
which yields the result.
\end{proof}

==> contents_low_rank/Densities.tex <==

 \subsection{Proofs for continous distributions}
\begin{proof}[Proof of Theorem~\ref{th:densities}]
\phantom{ }
Let $f \in \mathcal G_K$ and define the function $f_1:[0,1] \longrightarrow \R$ as $f_1(x) = \int_0^1 f(x,y) dy$, which is clearly $L$-Lipschitz over $[r_1,R_1]$. 
The function $f_1$ is the density of each observation $Z_i = \Pi_1(X_i)$, which is the projection of $X_i$ over the first coordinate. 
Similarly, we define $f_2:[0,1] \longrightarrow \R$ as $f_2(y) = \int_0^1 f(x,y) dx$. 
\vspace{1mm}

For $j=1,2$, let $\Delta_j = R_j - r_j$ and $\widehat \Delta_j = \widehat R_j - \widehat r_j$ where $r_j,R_j$ are associated with $f$ as in~\eqref{eq:def_L} and $\widehat r_j,\widehat R_j$ are defined in Algorithm~\ref{alg:Alg_densities}. 
For $j=1,2$, we also define $q_-^{(j)}$ and $q_+^{(j)}$ as the quantiles  of order $1/\sqrt{n}$ and $1-1/\sqrt{n}$ of the probability measure defined by $f_j$:
    $$ \int_{-\infty}^{q_-^{(j)}}f_j = \frac{1}{\sqrt{n}} \quad \text{ and } \quad \int_{q_+^{(j)}}^{+\infty}f_j = \frac{1}{\sqrt{n}}. $$


We denote by $\widehat f_j$, $j=1,2$ the outputs of Algorithm~\ref{alg:Alg_densities_1D} with inputs $\Pi_j(X_1),\dots, \Pi_j(X_n)$ for $j=1$ and $2$ respectively.
From now on, we place ourselves on the high-probability event $\mathcal{E} \cap \mathcal{F}$, where
\begin{align*}
    \mathcal{E} &= \left\{\widehat r_j < q_-^{(j)} < q_+^{(j)} < \widehat R_j ~\Big|~ j=1,2\right\},\\
    \mathcal{F} &= \left\{\|f_j - \widehat f_j\|_1 \leq \frac{C}{n^{1/3}} ~\Big|~ j=1,2\right\}.
\end{align*}
By Lemma~\ref{lem:density_1D}, $\mathbb P(\mathcal{F}) \geq 1 - 2\exp\big(\!-n^{1/3}\big)$, and $\mathbb P(\mathcal{E}) \geq 1-4e^{-\sqrt{n}}$, so that $\mathbb P(\mathcal{E} \cap \mathcal{F}) \geq 1 - 6 \exp\big(\!-n^{1/3}\big)$.
We distinguish between two cases.
\vspace{3mm}

\textbf{First case:} Assume that $\widehat \Delta_1 \land \widehat\Delta_2 \leq h^*$. 
By symmetry, suppose that $\widehat \Delta_1 \leq h^*$. 
In this case, the estimator $\widehat f$ can be written as $\widehat f(x,y) = \frac{1}{\widehat \Delta_1}\mathbb 1_{x \in [\widehat r_1, \widehat R_1]} \cdot \widehat f_2(y)$ and we get
\begin{align*}
    \|f - \widehat f\|_1 &\leq \int_{y=0}^1 \int_{x=r_1}^{R_1} \left|f(x,y) - \frac{f_2(y)}{\Delta_1}\right| dx dy + \int_{y=0}^1 \int_{x=r_1}^{R_1}  \left|\frac{f_2(y)}{\Delta_1} - \widehat f(x,y)\right| dx dy\\
    & \leq \int_{y=0}^1 \int_{x=r_1}^{R_1}  \left\{\frac{1}{\Delta_1}\int_{r}^R \underbrace{\left|f(x,y) - f(x',y)\right|}_{\leq L\Delta_1}dx'\right\} dx dy + \int_{y=0}^1 \int_{x=r_1}^{R_1}  \left|\frac{f_2(y)}{\Delta_1} - \frac{\widehat f_2(y)}{\widehat \Delta_1}\mathbb 1_{x\in[\widehat r, \widehat R]} \right| dx dy\\
    & \leq \int_{y=0}^1 \int_{x=r_1}^{R_1}L\Delta_1 \, dxdy ~ + \int_{y=0}^1 \left|f_2(y) - \widehat f_2(y)\frac{\Delta_1}{\widehat \Delta_1} \right| dy + \int_{y=0}^1 \int_{x \in [r_1,R_1]\setminus [\widehat r_1,\widehat R_1]} \frac{f_2(y)}{\Delta_1} dxdy\\
    & \leq L\Delta_1^2 + \|f_2 - \widehat f_2\|_1 + \|\widehat f_2 \|_1 \left|1-\frac{\Delta_1}{\widehat \Delta_1} \right| + \|f_2\|_1 \frac{\Delta_1 - \widehat \Delta_1}{\Delta_1}\\
    & \leq 2 L{h^*}^2 + \frac{C}{n^{1/3}} + \frac{16}{\sqrt{n}} + \frac{16}{\sqrt{n}}\\
    & \leq C n^{-1/3},
\end{align*}
recalling that, over $\mathcal E$ and when $\widehat \Delta_1 \leq h^*$, we have $\Delta_1 - \widehat \Delta_1 \leq 16\dfrac{\widehat \Delta_1}{\sqrt n} \leq16\dfrac{\Delta_1}{\sqrt n}$ by Lemma~\ref{alg:Alg_densities_1D}, and that over $\mathcal{F}$, we have $\|f_2 - \widehat f_2\|_1 \leq C n^{-1/3}$.

\vspace{2mm}

\textbf{Second case:} Assume that $\widehat \Delta_1 > h^*$ and $\widehat \Delta_2>h^*$. 
Recalling the notation of Algorithm~\ref{alg:Alg_densities}, we let $b_1 = |E_1|$, $b_2 = |E_2|$ and $b = b_1 \lor b_2$. % and without loss of generality, assume that $b$ is an integer \ju{clarify}. For ease of notation, we will write $A_i = A_i(h)$, $B_j = B_j(h)$ and  $C_{ij} = C_{ij}(h)$.
%For some large enough constant $C>0$, we let $b = \left\lceil C(n/K)^{1/3}\right\rceil$ and, for both the upper and the lower bound, we define a binning of the domain $[0,1]^2$ into bins of edge-length $1/b$. More precisely, for any $i,j \in [b-1]$, we define $A_i = \left[\frac{i-1}{b}, \frac{i}{b}\right)$ and $A_b = \left[\frac{b-1}{b}, \;1\right]$, as well as $B_j = \left[\frac{j-1}{b}, \frac{j}{b}\right)$ and $B_b = \left[\frac{b-1}{b}, 1 \right]. $ We can now define the cells $C_{ij} = A_i \times B_j$ for any $i,j \in [b]$. The above defined cells $C_{ij}$ form a partition of the domain $[0,1]^2$. We denote by $h = 1/b$ the edge-length of each cell.\\
We construct the matrix $P = (P_{ij})_{i,j}$, where 
$$ \forall (i,j) \in [b_1]\!\times\! [b_2]: P_{ij} = \int_{C_{ij}} f dx dy = \sum_{k=1}^K \int_{A_i} u_k(x) dx \int_{B_j} v_k(y) dy =: \sum_{k=1}^K U_k(i) V_k(i). $$
In the above equation, we have defined $U_k = (U_k(1), \dots, U_k(b))$ and $V_k = (V_k(1), \dots, V_k(b))$, where  $U_k(i) = \int_{A_i} u_k(x) dx$ and $V_k(j) = \int_{B_j} v_k(y) dy$ for any $(i,j) \in [b_1]\!\times\![b_2]$ and $k \in K$.
Therefore, it holds that the matrix $$P = \sum_{k=1}^K U_k V_k^\top$$ has rank at most $K$. 
For any $i,j \in [b]$, we also recall the definition of $N_{ij}$ and $N'_{ij}$: 
$$N_{ij} = \sum_{\ell=n/2+1}^{3n/4} \mathbb 1_{X_\ell \in C_{ij}} \quad \text{ and } \quad N'_{ij} = \sum_{\ell=3n/4+1}^n \mathbb 1_{X_\ell \in C_{ij}}.$$
It is clear that the random matrix histograms $N = (N_{ij})_{i,j =1}^b$ follow a multinomial distribution with parameters $P$ and $n/4$.
We can therefore apply Algorithm~\ref{alg:Alg}, to estimate $P$ in total variation. 
We denote by $\widehat P$ its output when applied to the dataset $N = \left\{(N_{ij})_{ij}, (N'_{ij})_{ij}\right\}$.
For any $\alpha>0$, Theorem~\ref{th:main_th} ensures that, for some constant $C$ depending on $\alpha$, we have 
$$ \sup_{f \in \mathcal{G}_K} \|\widehat P - P\|_1 \leq C \sqrt{\frac{Kb}{n}} \log^3(b) \leq C\left(\frac{K}{n}\right)^{1/3} \log^3(n)$$
with probability $1-O(b^{-\alpha})$. 
To conclude, we recall that we have $\widehat f(x,y) := \widehat P_{ij}/(h_1 h_2)$ when $(x,y) \in C_{i,j}$, so that $\int_{C_{ij}} \widehat f = P_{ij}$. 
To control the bias of this estimator, we further define the function $\bar f$ by $h_1 h_2 \bar f(x,y) = P_{ij}$ when $(x,y) \in C_{ij}$.
\vspace{2mm}

For $j \in \{1,2\}$, we now define $m_j = \big\lfloor(\widehat R_j - \widehat r_j ) n^{1/3}L^{1/2}\big\rfloor$. 
By continuity of $f$, we note that over each cell $C_{ij}$ with $i \in \{0,\dots, m_1-1\}$ and $j \in \{0,\dots, m_2-1\}$, there exists a point $z_{i,j} \in C_{ij}$ such that 
$$h_1 h_2f(z_{ij}) = P_{ij} = h_1 h_2 \bar f(x,y), \forall x,y \in C_{ij}.$$ 
Over such cells $C_{ij}$, we therefore have $\left|f(x,y) - \bar f(x,y)\right| = \left|f(x,y) - f(z_{ij})\right| \leq L\|(x,y)-z_{ij}\| \leq C L h^*$, which yields that
\begin{align*}
    \sum_{i=0}^{m_1-1}\; \sum_{j=0}^{m_2-1} \int_{C_{ij}} \left|f(x,y)- \bar f(x,y) \right|dxdy \leq b^2 C Lh \cdot h^2 = C Lh.
\end{align*}
Over $\mathcal{C}:= [0,1]^2\setminus \left\{\bigcup_{i=0}^{m_1-1} \; \bigcup_{j=0}^{m_2-1} C_{ij}\right\}$, we have by definition of $\mathcal{E}$ that $\int_{\mathcal{C}} f \leq \frac{C}{\sqrt{n}}$, so that with probability $1 - \exp\left(-c\sqrt{n}\right)$, we have that 
\begin{align*}
    S := \sum_{\substack{j\in E_1 \\ j \notin \{0,\dots,m_1-1\} }} \sum_{\substack{j'\in E_2 \\ j' \notin \{0,\dots,m_2-1\} }} N_{j,j'} + N'_{j,j'} \leq C \sqrt{n}.
\end{align*}
To see this, note that $S \sim \operatorname{Bin}(n/2,p)$ where $p \leq \frac{C}{\sqrt{n}}$, so that, by Bernstein's inequality, we get 
\begin{align*}
    \mathbb P\left(S > C \sqrt{n}\right) &\leq \exp\left(-c \cdot t \land \frac{t^2}{\sqrt{n}}\right) \quad \text{ where } t = C \sqrt{n} - np\\
    & \leq \exp\left(-c \sqrt{n}\right).
\end{align*}
We recall that over $\mathcal{C}$, the estimator can be written as $\widehat f = \frac{1}{h_1h_2} \sum_{(j,j') \notin \mathcal{E}'} \frac{2}{n} (N_{j,j'} + N'_{j,j'})\mathbb 1_{C_{j,j'}}$.
Therefore, with probability $1-\exp\left(-c\sqrt{n}\right)$, we obtain 
\begin{align*}
    \int_{\mathcal{C}} |\widehat f - f| \leq \int_{\mathcal{C}} |\widehat f | +\int_{\mathcal{C}} |f| \leq  \frac{C\sqrt{n}}{n} + \frac{C}{\sqrt{n}} \leq \frac{C}{\sqrt{n}}.
\end{align*}
%\ju{Vérifier, pb sur $\mathcal{C}?$ il faut peut être mettre seulement le max de vraisemblance sur $\mathcal{C}$, plus simple à analyser.}

Therefore, summing all of the contributions, the estimation error of $\widehat f$ is upper bounded as
\begin{align*}
    \|\widehat f - f\|_{L^1} &= \|\widehat f - f\|_{L^1(\mathcal{C})} + \|\widehat f - f\|_{L^1(\mathcal{C}^c)} \leq \frac{C}{\sqrt{n}} +  \|\widehat f - \bar f\|_{L^1(\mathcal{C}^c)} +  \|\bar f - f\|_{L^1(\mathcal{C}^c)} \\
    &\leq \frac{C}{\sqrt{n}} + C\left(\frac{K}{n}\right)^{1/3} \log^3(n) + C Lh \leq C\left(\frac{K}{n}\right)^{1/3} \log^3(n)
\end{align*}
with probability at least $b^{-\alpha} \asymp n^{-\alpha/3}$, for some constant $C$ depending only on $\alpha$ and $L$.
\\

\textbf{Lower bound} The class $\mathcal{L}_{[0,1]^2} \cap\mathcal{F}_K$ is clearly smaller than $\mathcal{G}_K$, so that $\varphi_\delta^*(n,\mathcal{L}_{[0,1]^2} \cap\mathcal{F}_K) \leq \varphi_\delta^*(n,\mathcal{G}_K)$. 
By Proposition~\ref{prop:strengthened_LB}, the result follows.

\end{proof}

\begin{proof}[Proof of Proposition~\ref{prop:strengthened_LB}] 
%For $x,y \in [0,1]$, we define $f_0(x,y) = \frac{b}{K} \mathbb 1_{x\leq K/b}$.  
For $x,y \in [0,1]$, we write $f_0 = \mathbb 1_{[0,1]^2}$ and recall that,  by assumption, $K \leq c n^{1/4}$. 
For some small enough constant $c' \in \big(0,(L\lor1)^{-1}\big)$ depending only on $L$, let
$$h= c' \left(\frac{K}{n}\right)^{1/3}, \quad k = \frac{1}{K}, \quad \text{ and } \quad H = \frac{1}{h}.$$
Note that we have $h\leq 1$ since $c'\in (0,1)$, and $k \geq h$ if $c'$ is chosen small enough. 
We also set $z_{ij} = (x_i,y_j)$ where $x_i = \big(i-\frac{1}{2}\big) k$ and $y_j = \big(j-\frac{1}{2}\big)h$ for any $i,j \in \mathbb Z$,
and define the functions 
\begin{align*}
    U(x) = \begin{cases} x+\frac{1}{2} & \text{ if } x \in [-\frac{1}{2},-\frac{1}{6}]\\ \frac{1}{3} &\text{ if } x \in [-\frac{1}{6}, \frac{1}{6}]\\
    \frac{1}{2}-x &\text{ if } x \in [\frac{1}{6},\frac{1}{2}]\\
    0 & \text{ otherwise.}\end{cases} \quad\text{ and } \quad V(y) = \Big(\frac{1}{2}-|y|\Big)_+.
\end{align*}
Now, we can set $U_i(x) = U\big(\frac{x-x_i}{k}\big)$ and $V_j(y) =  V(\frac{y-y_j}{h})$.
%$U_{i} (x) = \frac{Lh}{K} \left[\left(1-\frac{|x-x_i-1/2|}{2h}\right)_+ + \left(1-\frac{|x-x_i+1/2|}{2h}\right)_+\right]$ as well as $V_{j} (y) = \frac{Lh}{K} \left[\left(1-\frac{|y-y_j-1/2|}{2h}\right)_+ - \left(1-\frac{|y-y_j+1/2|}{2h}\right)_+\right]$. 
%perturbation $\phi_+(x,y) = \left(1-|x|\right)_+\left(1-|y|\right)_+$ and 
%$\phi_h(x,y) = c\frac{Lh}{K}\phi_+\left(\frac{1}{h}\left[(x,y)-(\frac{1}{2},\frac{1}{2})\right]\right) - \frac{Lh}{K}\phi_+\left(\frac{1}{h}\left[(x,y)+(\frac{1}{2},\frac{1}{2})\right]\right)$ \ju{check}.
For any $(i,j) \in \mathbb Z^2$, we define $C_{ij} = \big[x_i\pm\frac{k}{2}\big]\times \big[y_j\pm\frac{h}{2}\big]$.
We perturb $f_0$ on each cell $C_{i,j}$ as follows. 
For any $i \in \{1,\dots,\lfloor k^{-1}\rfloor\}, j \in \{1,\dots,\lfloor\frac{H}{2}\rfloor\}$, let $\omega_{ij}$ be i.i.d. Rademacher random variables with parameter $1/2$, and, for $\omega = (\omega_{ij})$ and a sufficiently small $c>0$, we let 
\begin{align}\label{eq:def_prior}
    f_\omega(x,y) = f_0 + c'' L h \sum_{i=1}^K \sum_{j=1}^{\lfloor H/2\rfloor} \omega_{ij} U_{i}(x) \big(V_{j}(y) - V_{b-j}(y)\big).
\end{align}
First, we  verify that each $f_\omega$ belongs to $\mathcal{G}_{K+1}$: 
\begin{itemize}
    \item We have $\int_{[0,1]^2} f_\omega = 1$ by construction.
    \vspace{-2mm}
    \item Moreover, we have $K\leq c n^{1/4}$ by assumption. 
    Therefore, $\|(x,y)\mapsto U_{i}(x) V_{j}(y)\|_\infty \leq \frac{c''}{3} Lh<1$, so that $f_\omega \geq \frac{1}{2}>0$ if the constant $c''$ appearing in~\eqref{eq:def_prior} is chosen sufficiently small.
    \vspace{-2mm}
    \item The Lipschitz condition can be checked as follows. 
    In the definition of $f_\omega$, the functions $(x,y) \mapsto U_{i}(x) V_{j}(y)$ have disjoint support, and $f_\omega$ is zero on the boundary of each cell $C_{ij}$. 
    Therefore, it suffices to show that $f_\omega$ is $L$-Lipschitz over each cell $C_{ij}$ to obtain that it is Lipschitz over $[0,1]^2$. Fix any two points $z,z' \in [0,1]^2$, belonging to the same cell $C_{ij}$. Then, writing $z = (x,y)$ and $z' = (x',y')$, we obtain:
    \begin{align*}
        \big|f_\omega(z) - f_\omega(z')\big| &= c''Lh\,\Big|U_i(x)V_j(y) - U_i(x')V_j(y')\Big|\\
        &\leq c''Lh\,\big\| U_i \big\|_\infty \Big|V_j(y)-V_j(y')\Big| + c''Lh \Big|U_i(x)-U_i(x')\Big| \big\|V_j\big\|_\infty\\
        & \leq \frac{c''}{3} Lh\frac{|y-y'|}{h} + c''Lh\cdot \frac{|x-x'|}{k} \\
        &\leq L\|z-z'\|,
    \end{align*}
    recalling that $h\leq k$ since $K\leq c n^{1/4}$.
    \vspace{-2mm}
    \item Moreover, $f_\omega$ belongs to $\mathcal{F}_{K+1}$ since we can write 
\begin{align*}
    f_\omega(x,y) = f_0 + c''Lh\sum_{i=1}^K U_i(x)\left(\sum_{j=1}^{\lfloor H/2 \rfloor} \omega_{ij} (V_j(y)-V_{b-j}(y))\right).
\end{align*}
\end{itemize}

For any $\omega, \omega' \in \{\pm 1\}^{K\times \lfloor\frac{H}{2} \rfloor}$ that only differ by one entry, that is, such that for exactly one $(i_0,j_0)$, we have $\omega_{i_0,j_0}\neq \omega'_{i_0,j_0}$, we can compute the $\chi^2$ divergence between the probability distributions whose densities are  $f_\omega$ and $f_{\omega'}$ respectively. 
Let $\phi_{ij} (x,y) = c'' Lh \, U_{i}(x) \big(V_{j}(y) - V_{b-j}(y)\big)$
\begin{align*}
    \chi^2\left(f_{\omega'}|| f_{\omega}\right) &= \int_{C_{i_0,j_0}} \frac{\phi_{i_0,j_0}^2(x,y)}{f_\omega(x,y)} \leq \int_{C_{i_0,j_0}} \frac{(c''Lh)^2}{1/2} = 2(c'')^2 L^2 h^3 k \leq \frac{2 \widetilde{c}^{\,2}}{n}.
\end{align*}
Choosing the constant $c$ small enough in the definition of $\phi_h$ ensures that
\begin{align*}
    TV\left(f_\omega^{\otimes n}, f_{\omega'}^{\otimes n}\right) \leq \sqrt{-1 + \left(1+\chi^2\left(f_{\omega'}|| f_{\omega}\right)\right)^n} \leq \frac{1}{2},
\end{align*}
where we have used that for any two probability distributions $P,Q$ over the same measurable space, we have the classical relations $\operatorname{TV}(P,Q) \leq \sqrt{\chi^2(P\,||\,Q)}$, and $1+\chi^2(P^{\otimes n}\,||\,Q^{\otimes n}) = \big(1+\chi^2(P\,||\,Q)\big)^n$ (see for example~\cite{tsybakov2008introduction}, Chapter 2). 
Therefore, by Assouad's Lemma, we get that 
$$ \inf_{\widehat f} \sup_{f \in \mathcal{G}_K} \mathbb E \left[ 
    \|f-\widehat f\|_{L^1}
    \right] \geq HK \times \frac{1}{2} \times c''Lh^2 k\geq \frac{c''}{10} \left(K/n\right)^{1/3}.$$ 
\end{proof}

\begin{lemma}\label{lem:density_1D}
Let $f: \R\longrightarrow \R_+$ be a probability density. Assume that for some $r,R \in [0,1]$, the function $f$ is $L$-Lipschitz over $[r,R]$ and that $f=0$ over $\R\setminus [r,R]$. 
Assume that we observe $n$ iid data points $Z_1,\dots, Z_n \in \R$ distributed with probability density $f$, where $n$ is larger than an absolute constant.
Let $\widehat R = \max Z_i$ and $\widehat r = \min Z_i$. 
Let also $\Delta = R-r$ and $\widehat \Delta = \widehat R - \widehat r$.
Let $q_-$ and $q_+$ be the quantiles of order $1/\sqrt{n}$ and $1-1/\sqrt{n}$ of the probability measure defined by $f$:
    $$ \int_{-\infty}^{q_-}f = \frac{1}{\sqrt{n}} \quad \text{ and } \quad \int_{q_+}^{+\infty}f = \frac{1}{\sqrt{n}}, \quad \text{ and let } \quad \mathcal{E} = \left\{\widehat r < q_- < q_+ < \widehat R\right\}. $$
Let $\widehat f$ be the output of Algorithm~\ref{alg:Alg_densities_1D} with inputs $Z_1,\dots, Z_n$.
Then, defining $h^* = n^{-1/3}L^{-1/2}$, we have 
\begin{enumerate}
    \item $\mathbb P(\mathcal{E}) \geq 1 - 2e^{-\sqrt{n}}$.
    \item\label{item:Delta_leq_hat_Delta} Over $\mathcal{E}$, if $\widehat \Delta \leq h^*$, then $\Delta \leq \widehat \Delta \left[1 + 16/\sqrt n\right]$.
    \item $\mathbb P\left(\|f - \widehat f\|_{L^1} \leq C n^{-1/3}\right) \geq 1 - \exp\big(\!-n^{1/3}\big)$. 
\end{enumerate}

\end{lemma}

\vspace{1mm}

\begin{proof}[Proof of Lemma~\ref{lem:density_1D}]
    In this proof, we will use the notation defined in Algorithm~\ref{alg:Alg_densities_1D}.    
    The probability of event $\mathcal{E}$ can be controlled as follows.
    \begin{align}
        \mathbb P(\mathcal{E}^c) \leq 2\mathbb P\left(\widehat R>q_+\right) = 2 \mathbb P\left(Z_1>q_+\right)^n = 2\left(1-\frac{1}{\sqrt{n}}\right)^n \leq 2e^{-\sqrt{n}}.\label{eq:control_E}
    \end{align}
    
    From now on, we place ourselves on event $\mathcal{E}$. %and recall that $n$ is assumed to be greater than a sufficiently large absolute constant $C>0$. 
    We distinguish between two cases.
    \vspace{2mm}

    \textbf{First case:} Assume that $\widehat \Delta < h^*$. Then, over $\mathcal{E}$, and by the Lipschitz assumption, we have
    \begin{align*}
        \frac{1}{2} &\leq 1 - \frac{2}{\sqrt{n}} \leq \int_{\widehat r}^{\widehat R} f \leq \widehat \Delta \max_{[\widehat r, \widehat R]} f \\
        &\leq \widehat \Delta \min_{[\widehat r, \widehat R]} f + L \widehat \Delta^2 \leq \widehat \Delta \min_{[\widehat r, \widehat R]} f + L{h^*}^2 \\
        &\leq \widehat \Delta \min_{[\widehat r, \widehat R]} f + \frac{1}{4},
    \end{align*}
    using that $L{h^*}^2 \leq L n^{-2/3} L^{-1} \leq \frac{1}{4}$ for $n$ larger than a constant.
    Therefore, $f(\widehat r) \geq \min_{[\widehat r, \widehat R]} f \geq \frac{1}{4\widehat \Delta}$.
    
    Set $\overline r := \widehat r - \frac{2}{f(\widehat r)\sqrt{n}}$ and suppose for a contradiction that $r < \overline r$. 
    Then, still by the definition of $\mathcal{E}$ and the Lipschitz assumption, we would get
    \begin{align*}
        \frac{1}{\sqrt{n}} &\geq \int_{r}^{\widehat r} f \geq \int_{\overline r}^{\widehat r} f \geq (\widehat r-\overline r) f(\widehat r) - L(\widehat r - \overline r)^2 \\
        & = \frac{2}{\sqrt{n}} - \frac{4L}{n f(\widehat r)^2} \geq \frac{2}{\sqrt{n}} - \frac{64 L \widehat \Delta^2}{n}\\
        & \geq \frac{2}{\sqrt{n}} - \frac{64 L {h^*}^2}{n} > \frac{1}{\sqrt{n}} ~~ \text{provided that $n$ is larger than a constant,}
    \end{align*}
    which is contradictory. 
    Therefore, we can conclude that $r>\overline r> \widehat r - \frac{8\widehat \Delta }{\sqrt{n}}$ and similarly, $R <\widehat R + \frac{8 \widehat \Delta}{\sqrt{n}}$, so that $\Delta \leq \widehat \Delta + \frac{16\widehat \Delta}{\sqrt n}$. This concludes the proof of item~\ref{item:Delta_leq_hat_Delta}.
    \vspace{1mm}
    
    We recall that since $\widehat \Delta \leq h$, our estimator is $\widehat f = \frac{1}{\widehat R - \widehat r} \mathbb 1_{[\widehat r, \widehat R]}$.
By continuity of $f$ over $[r,R]$, there exists $x_0 \in [r,R]$ such that $f(x_0)(R-r) = \int_r^R f = 1$.
    Now, over $\mathcal{E}$
    \begin{align*}
    \|f-\widehat f\|_{L_1} &= \int_r^R |f(x)-\widehat f(x)|dx = \int_{r}^{\widehat r} f + \int_{\widehat r}^{\widehat R} |f(x)-\widehat f(x)|dx + \int_{\widehat R}^R f \\
    & \leq \int_{\widehat r}^{\widehat R} |f(x)-f(x_0)|dx + \int_{\widehat r}^{\widehat R} |f(x_0)-\widehat f(x)|dx + \frac{2}{\sqrt{n}}\quad \text{ over } \mathcal{E}\\
    & \leq L(R-r)^2 + \int_{\widehat r}^{\widehat R} |f(x_0)-\widehat f(x)|dx + \frac{2}{\sqrt n}\\
    & \leq L\left(\widehat \Delta + \frac{16 \widehat \Delta}{\sqrt{n}}\right)^2 + (\widehat R-\widehat r) \left|\frac{1}{R-r} - \frac{1}{\widehat R - \widehat r}\right| + \frac{2}{\sqrt n}\\
    & \leq 2L{h^*}^2 + \left|\frac{\widehat \Delta }{\widehat \Delta(1+16/\sqrt n)}-1\right| + \frac{2}{\sqrt{n}}\\
    & \leq \frac{C}{\sqrt{n}} \leq Cn^{-1/3}.
\end{align*}

\textbf{Second case:} Assume now that $\widehat \Delta > {h^*}$. 
%For any $j \in \{0,\dots, \lfloor1/h\rfloor\}$, we define $A_j = A_h(j) \cap [r,R]$ and  $h_j = \operatorname{Vol}\left\{\overline{A}_h(j)\right\}$, and we recall that $A'_h(j) = A_h(j) \cap [\widehat r, \widehat R]$. 
We recall the definition of $(A_j)_{j}$ from Algorithm~\ref{alg:Alg_densities_1D}. 
By continuity of $f$ over $A_j$, we can define $x_j \in A_j$ such that $f(x_j) \, h = \int_{A_j} f$. 
For any $j \in E$, we define 
\begin{align*}
    p_j = \int_{A_j} f, \quad \text{ and } \quad \widehat p_j = \int_{A_j} \widehat f.
\end{align*}
Then, taking $\delta = \exp\big(\!-n^{1/3}\big)$, the estimation error of $\widehat f$ is controlled as:
\begin{align*}
    \|f - \widehat f\|_1 &= \sum_{j\in E} \, \int_{A_j} \big|f-\widehat f\big| \leq \, \sum_{j\in E} \, \int_{A_j} \big|f(x) - f(x_j)\big| + \big|f(x_j)-\widehat f\,\big| \, dx\\
    & \leq \sum_{j\in E} \left\{ Lh^2 + |p_j - \widehat p_j|\right\} \leq Lh + \sqrt{\frac{|E| + \log(1/\delta)}{n}} \quad \text{ with probability } \geq 1 - \delta\\
    & \leq C n^{-1/3}\quad \text{ with probability } \geq 1-\delta,
\end{align*}
where in the second step we used Proposition~\ref{prop:samp_comp_TV_discrete}.
\end{proof}

==> contents_low_rank/Extension_to_tensors.tex <==
\section{Extension to tensors}

\subsection{Sum-up of the matrix case}
We recall the intuition of the algorithm in the matrix case. Let $P \in \R_+^{d_1\times d_2}$ with $\sum_{ij} P_{ij} = 1$ and $\rk P = K$. Assume that we observe a matrix $Y \in \R^{d_1 \times d_2}$ whose entries are independent Poisson random variables with respective distributions $\Poi(nP_{ij})$ for all $i,j$.\\

We also recall that, for any matrix $\Lambda \in \R^{d_1\times d_2}$, we define the norms
\begin{align*}
    &\|\Lambda\|_{1,\infty} = \max_{j} \sum_{i} |\Lambda_{ij}| ~\text{ (maximum column norm)}\\
    & \normsquare{\Lambda} = \|\Lambda\|_{1,\infty} \lor \|\Lambda^\top\|_{1,\infty}.
\end{align*}


We define $p_i = \sum_{j} P_{ij}, \forall i \in [d_1]$ as well as $q_j = \sum_{i} P_{ij}, \forall j \in [d_2]$. Assume that an oracle gives us $(p_1,\dots, p_{d_1})$ and $(q_1,\dots, q_{d_2})$ (in practice, use sample splitting to estimate the oracle with the first half of the data and apply the following procedure with the second half). The procedure is as follows. Fix $d = d_1 \lor d_2$. For any $t \in \{0,\dots, \lfloor\log_2(d)-1\rfloor\}$, define 
$$ I_t = \left\{i: p_i \in \left[\frac{1}{2^t}, \frac{1}{2^{t+1}}\right]\right\}$$
$$ J_{t} = \left\{j: q_j \in \left[\frac{1}{2^{t}}, \frac{1}{2^{t+1}}\right]\right\},$$
and for $t = \lfloor\log_2(d)\rfloor$, define $I_t = [d_1] \setminus \bigcup\limits_{t' < t} I_{t'}$ and $J_t = [d_2] \setminus \bigcup\limits_{t' < t} J_{t'}$.\\

Fix $t,t' \in \{0,\dots, \log_2(d)\}$ and define $k = (t,t')$. We further define $\Mk = \frac{1}{n} Y_{I_t\times J_{t'}}$, 
where $Y_{I_t \times J_{t'}} = \left[Y_{ij} \mathbb{1}_{(i,j) \in I_t \times J_{t'}}\right]_{ij}$, as well as $\Pk = \left[P_{ij} \mathbb{1}_{(i,j) \in I_t \times J_{t'}}\right]_{ij}$. 
Then $\rk \Pk \leq K$ and $\normsquare{\Pk} \leq \frac{1}{2^{t\land t'}}$ by construction. We perform a soft-thresholding of the SVD of $\Mk$ and obtain $\hatPk$ that satisfies 
\begin{align*}
    \left\|\Pk - \hatPk\right\|_F^2 \lesssim \frac{K}{n} \normsquare{\Pk} \lesssim \frac{K}{n2^{t \land t'}} \text{ by Olga's lemma (Proposition~\ref{prop:bound_Mult_matrix})}
\end{align*}
up to a $\log d$. We treat separately the pathological cases for which the assumptions of Proposition~\ref{prop:bound_Mult_matrix} are not met, and we show that they have a negligible contribution to the estimation rate. We can then control the $\ell_1$ norm as
\begin{align*}
    \left\|\Pk - \hatPk\right\|_1 \lesssim \sqrt{\frac{K}{2^{t \land t'} n} |I_t||J_{t'}|},
\end{align*}
which yields an overall estimation rate controlled as
\begin{align*}
    \|\hat P - P\|_1 &\lesssim \sum_{t,t' = 0}^{\log d} \sqrt{\frac{K}{2^{t \land t'} n} |I_t||J_{t'}|} \leq \sqrt{\sum_{t,t' = 0}^{\log d} \frac{K}{2^{t \land t'} n} |I_t||J_{t'}| \sum_{t,t'=0}^{\log d} 1} ~\text{ (Cauchy-Schwarz)}\\
    & \leq \sqrt{\sum_{t,t' = 0}^{\log d} \frac{K}{n}\left(\frac{1}{2^{t}} + \frac{1}{2^{t'}} \right) |I_t||J_{t'}|} \cdot \log d\\
    & \leq \sqrt{\frac{K (d_1+d_2)}{n}} \cdot \log d.
\end{align*}
At the last line, we used the fact that $\sum\limits_{t=0}^{\log d} I_t = d_1$ and $\sum\limits_{t=0}^{\log d} 2^{-t} I_t \leq 1$ (by the definition of $I_t$), and symmetrically for the family $(J_t)_t$.\\

\subsection{Ideas for tensors}
For any tensor $A \in \R^{d_1\times \dots \times d_M}$ and $u_1\in \R^{d_1},\dots, u_M\in \R^{d_M}$, we define the classical tensor product:
$$ A[u_1,\dots, u_M] := \sum_{j_1 = 1}^{d_1} \dots \sum_{j_M = 1}^{d_M} A_{j_1,\dots, j_M} \prod_{\ell = 1}^M u_\ell(j_\ell).$$

We fix a probability tensor $P \in \R_+^{d_1\times \dots \times d_M}$ with $\sum\limits_{j_1, \dots, j_M} P_{j_1,\dots, j_M} = 1$ and assume that $P$ has Tucker rank $(K,\dots, K)$. The goal is to estimate $P$ in total variation loss from a histogram of observations $Y \sim \M\left(P,n\right)$.
We indifferently write $P_{j_1,\dots, j_M}$ or $P(j_1,\dots, j_M)$.\\

For any $\ell \in [M]$, we can write $P$ as $\left(P^{(\ell)}(1), \dots, P^{(\ell)}(d_\ell)\right)$ where 
for any $j \in [d_\ell]$, $P^{(\ell)}(j)$ denotes the slice of $P$ defined by fixing coordinate $j$ on axis $\ell$:
$$ P^{(\ell)}(j) := P\left({\cdot, \dots, \cdot, j, \cdot, \dots, \cdot}\right) = \Big(P\big(j_1,\dots,j_{\ell-1}, \, j \, , j_{\ell+1}, j_M\big)\Big)_{\left\{j_{\ell'}\right\}_{\ell' \neq \ell}}.$$
We also define $p^{(\ell)}(j)$ as the sum of the elements of $P^{(\ell)}(j)$:
$$p^{(\ell)}(j) = \sum_{\ell' \neq \ell} \, \sum_{j_{\ell'}=1}^{d_{\ell'}} P\left(j_1, \dots, j_{\ell-1}, j, j_{\ell +1}, \dots, j_m\right),$$
and we define the probability vector $p^{(\ell)} = \left(p^{(\ell)}(1),\dots, p^{(\ell)}(d_\ell)\right)$.
Inspecting the proof of the matrix case, it would be natural to define an exponential grid for each of the vectors $p^{(\ell)}$: 
Letting $d = \sum_{\ell=1}^M d_\ell$, define
$$ I_t^{(\ell)} = \left\{j \in [d_\ell]: p^{(\ell)}(j) \in \left[\frac{1}{2^{t+1}}, \frac{1}{2^t}\right]\right\}, ~ \forall \ell \in [M], ~\forall t \in \{0,\dots, \lfloor\log (d) -1\rfloor\},$$
and $I_T^{(\ell)} = [d_\ell] \setminus \bigcup\limits_{t' < T} I_{t'}^{(\ell)}$ for $T = \lfloor\log(d)\rfloor$.\\

Considering the papers~\cite{tomioka2014spectral} and ~\cite{zhang2018tensor}, Theorems 1 and 2, we propose the following conjecture:
\begin{conjecture}\label{conj:rate_low_rank_tensors}
Let $A,W,Y \in \R^{d_1\times \dots \times d_M}$ such that $Y = A+W$ and assume that $A$ has Tucker rank equal to $(K,\dots,K)$. Then, denoting by $\hat A$ the estimator obtained by applying the procedure from~\cite{zhang2018tensor}, we conjecture that
$$ \|\hat A - A\|_F^2 \lesssim K\|W\|_{op}, $$
with high probability or in expectation \ju{to be clarified}, where $$\|W\|_{op}:= \max_{\|u_1\| = \dots = \|u_M\|} W[u_1,\dots, u_M].$$
\end{conjecture}
The analogous tensor procedure should be as follows. Assume that an oracle gives us $p^{(\ell)}(j)$ for any $\ell \in [M]$ and $j \in [d_\ell]$ (in practice, estimate it with one half of the data). 
Fix any $k =\left(t_1,\dots, t_M\right) \in \{0,\log d\}^M$ and to consider the sub-tensors 
$$ \Mk = \frac{1}{n} Y^{(k)} ~\text{ and }~ W^{(k)} = \Pk - \Mk $$
where $Y^{(k)} := \left(Y(j_1,\dots,j_M) \cdot  \mathbb 1\left\{\forall \ell: j_l\in I_{t_\ell}^{(\ell)}\right\} \right)_{j_1,\dots, j_M}$ 
and similarly for $W^{(k)}$ and $\Pk$. In order to have an analogous estimation guarantee to the matrix case, it seems necessary to have the following guarantee:
\begin{conjecture}\label{conj:bound_Wk}
For any $k =\left(t_1,\dots, t_M\right) \in \{0,\dots,\log d\}^M$:
$$
\|W^{(k)}\|_{op} \lesssim \frac{1}{n}\sum_{\ell = 1}^M \frac{2^{t_\ell}}{2^{\sum_{\ell=1}^M t_\ell}}.
$$
    
\end{conjecture}
Note that for $M=2$, Conjecture~\ref{conj:bound_Wk} is compatible with the matrix case as we recover $\|W^{(k)}\|_{op} \lesssim 2^{-t\land t'}$.\\

Given Conjecture~\ref{conj:rate_low_rank_tensors}, this conjecture seems to be the condition needed to prove our rate.
Indeed, for any $k$, it implies that  we can construct an estimator $\hatPk$ using Conjecture~\ref{conj:rate_low_rank_tensors}, satisfying the following bound:
\begin{align*}
    \|\Pk - \hatPk\|_F^2 \lesssim K \sum_{\ell = 1}^M \frac{2^{t_\ell}}{2^{\sum_{\ell=1}^M t_\ell}}.
\end{align*}
We can then control the $\ell_1$ norm as follows:
\begin{align*}
    \|\Pk - \hatPk\|_1^2 \lesssim K \sum_{\ell = 1}^M \frac{2^{t_\ell}}{2^{\sum_{\ell=1}^M t_\ell}} \prod_{\ell=1}^M \left|I_{t_\ell}^{(\ell)}\right|.
\end{align*}
Then, the overall $\ell_1$ estimation risk is controlled as:
\begin{align*}
    \|\hat P - P\|_1 &\lesssim \sum_{t_1,\dots,t_M = 0}^{\log d} \sqrt{\frac{K}{n}\sum_{\ell = 1}^M\frac{2^{t_\ell}}{2^{\sum_{\ell=1}^M t_\ell}} \prod_{\ell=1}^M \left|I_{t_\ell}^{(\ell)}\right|}\\
    &\leq \sqrt{\frac{K}{n}\sum_{t_1,\dots,t_M = 0}^{\log d}\sum_{\ell = 1}^M \frac{2^{t_\ell}}{2^{\sum_{\ell=1}^M t_\ell}} \prod_{\ell=1}^M \left|I_{t_\ell}^{(\ell)}\right|}\sqrt{ \sum_{t_1,\dots,t_M = 0}^{\log d} 1} ~\text{ (Cauchy-Schwarz)}\\
    & = \sqrt{\frac{K}{n} \sum_{\ell=1}^M \left(\sum_{t_\ell=1}^{d_\ell}\left|I^{(\ell)}_{t_\ell}\right|\right) ~ \prod_{\ell'\neq \ell} \left(\sum_{t_{\ell'}=1}^{d_{\ell'}} 2^{-t_{\ell'}}\left|I^{(\ell')}_{t_{\ell'}}\right|\right)} ~ \cdot ~ \log^{M/2}(d)\\
    & \lesssim \sqrt{\frac{K}{n}(d_1+ \dots+ d_M)}  \cdot  \log^{M/2}(d),
\end{align*}
At the last line, we used the fact that $\sum\limits_{t_\ell=0}^{\log d} \left|I^{(\ell)}_{t_\ell}\right| = d_\ell$ and $\sum\limits_{t_\ell=0}^{\log d} 2^{-t_\ell} \left|I^{(\ell)}_{t_\ell}\right| \leq 1$ (by the definition of $I^{(\ell)}_{t_\ell}$).\\

If this is the correct estimation procedure, then Conjecture~\ref{conj:bound_Wk} should be the largest upper bound on $\|W^{(k)}\|_{op}$ that we can hope for \ju{How to check this properly?}.\\

\textbf{\underline{Tensor Bernstein}}

Now, we can look at the tensor Bernstein inequality from~\cite{luo2019bernstein} and see if it gives a tight enough control over $\|W\|_{op}$. 
The theorem proved in~\cite{luo2019bernstein} is very easy to generalize to our setting.
It just amounts to unfolding the tensors to matrices and to take the spectral norm of all such defined matrices.\\


To simplify the analysis, assume that our multinomial tensor $P$ has even order $2m$ and that $d_1 = \dots = d_{2m} = d$ . Assume moreover that $P$ is Einstein-symmetric, in the sense that 
$$ \forall i_1,\dots, i_m, j_1, \dots, j_m \in [d], P(j_1,\dots,j_m, i_1, \dots, i_m) = P(i_1,\dots,i_m, j_1, \dots, j_m).$$

For the matrix unfolding, define the function $f$ as in the paper~\cite{luo2019bernstein}: given an order $2m$ tensor $\mathcal{A} \in \R^{d \times \dots \times d}$, define the matrix $A = f(\mathcal{A})$ through $A_{ij} = \mathcal{A}_{i_1,\dots, i_m, j_1,\dots, j_m}$, where
$$ i = i_1+\sum_{k=2}^m \left((i_k-1)d^{k-1}\right), ~~~~~~ j = j_1+\sum_{k=2}^m \left((j_k-1)d^{k-1}\right).$$

Recalling the notation of the paper~\cite{luo2019bernstein}, we have 
$$ \lambda^{\square}_{\max} (\mathcal{A}) = \lambda_{\max}(f(\mathcal{A}))$$
for any symmetric tensor $\mathcal{A}$, hence
$$ \|\mathcal{A}\|^{\square} = \|f(\mathcal{A})\|_{op}.$$

Inspecting the proof of Theorem 3.1 in~\cite{luo2019bernstein}, we see that this theorem just amounts to rewriting the matrix Bernstein inequality to $f(\mathcal{A})$ using the equivalence
$ \|\mathcal{A}\|^{\square} = \|f(\mathcal{A})\|_{op}.$ 
Hence, using this theorem in our case will yield the following result. Let $\Lambda \in \R^{d\times \dots \times d}$ be an Einstein-symmetric, order $2m$ tensor with non-negative entries and let $W \in \R^{d\times \dots \times d}$ be a random tensor defined by 
$$ W_{i_1,\dots, i_{2m}} \sim \Poi(\Lambda_{i_1,\dots, i_{2m}}) - \Lambda_{i_1,\dots, i_{2m}}. $$
Then, with probability at least $1 - d^{-\alpha}$:
$$ \|W\|^{\square} \leq c\max\left\lbrace \sqrt{(1+\alpha)\| f(\Lambda^{T})\|_{1,\infty}\vee \| f(\Lambda)\|_{1,\infty}\log (d)},\; (1+\alpha)\sqrt{\lambda}\log(d)\log\left(\frac{2\sqrt{\lambda}}{\sqrt{\| f(\Lambda^{T})\|_{1,\infty}\vee \| f(\Lambda)\|_{1,\infty}}}\right) \right\rbrace,$$
and as explained above, the leading term is always the first one, so that 
$$ \|W\|^{\square} \lesssim  \sqrt{\| f(\Lambda^{T})\|_{1,\infty}\vee \| f(\Lambda)\|_{1,\infty}}\log (d).$$
Now, we can compute $\|f(\Lambda)\|_{1,\infty}$.
\begin{align*}
    \|f(\Lambda)\|_{1,\infty} = \max_{j=1}^{d^m}~\left[ \sum_{i=1}^{d^m} f(\Lambda)_{ij} \right] = \max_{j_1,\dots,j_m=1}^{d}  \sum_{i_1,\dots, i_m=1}^d \Lambda_{i_1,\dots,i_m,j_1,\dots,j_m}.
\end{align*}
Let $k=(t_1,\dots, t_{2m})\in \{0,\dots, \lfloor \log d\rfloor\}$ and recall the definitions of $I_{t_\ell}^{(\ell)}$ for all $\ell \in [2m]$.
Assume that we place ourselves on $Y^{(k)}$ with underlying tensor parameter $\Pk$. Then, we would have:
\begin{align*}
    \|W^{(k)}\|^{\square} \leq \log d \sqrt{\frac{1}{n}\left(\max_{j_1,\dots,j_m=1}^{d}  \sum_{i_1,\dots, i_m=1}^d \Lambda_{i_1,\dots,i_m,j_1,\dots,j_m}\right) \lor \left( \max_{i_1,\dots,i_m=1}^{d}  \sum_{j_1,\dots, j_m=1}^d \Lambda_{i_1,\dots,i_m,j_1,\dots,j_m} \right)}.
\end{align*}
We argue that this bound is too large. 
In the particular case where $P$ is the uniform distribution over $[d]^{2m}$, i.e. for $P_{i_1,\dots,i_m,j_1,\dots,j_m} = d^{-2m} \forall i_1,\dots,i_m,j_1,\dots,j_m$, we get $$\max_{i_1,\dots,i_m=1}^{d}  \sum_{j_1,\dots, j_m=1}^d P_{i_1,\dots,i_m,j_1,\dots,j_m} = \max_{i_1,\dots,i_m=1}^{d}  \sum_{j_1,\dots, j_m=1}^d d^{-2m} = d^m \cdot d^{-2m} =  \frac{1}{d^m},$$
so that $\|W\|^{\square} \lesssim\sqrt{\frac{1}{n d^m}}$.
However, for fixed $d,m$ and for $n \to \infty$, using the Poissonization trick, we get that
\begin{align*}
    W & = \left[\frac{1}{n} \Poi\left(\frac{1}{n}d^{-2m}\right) - \frac{1}{n}d^{-2m}\right]_{i_1,\dotsi_m, j_1,\dots,j_m} \\
    &\\
    &\approx \left[\mathcal{N}(0, \sigma^2)\right]_{i_1,\dots i_m, j_1,\dots,j_m} ~~ \hspace{5mm} \text{ where } \sigma^2 = \frac{1}{n}d^{-2m}
\end{align*}
Using the result in~\cite{tomioka2014spectral}, we get that $\|W\|_{op} \lesssim \sqrt{2  \sigma^2 m d \log(m)} \asymp \sqrt{\frac{m \log m}{nd^{2m-1}}} \ll \sqrt{\frac{1}{n d^m}}$, hence the Einstein-Bernstein inequality does not give a sufficiently tight result.
\newpage

==> contents_low_rank/Introduction.tex <==

\section{Introduction}

Estimating discrete and continuous probability distributions is one of fundamental problems in statistics and machine learning. 
A classical density estimator for both discrete and continuous data is the histogram, while for continuous densities the most popular method is kernel density estimator (KDE) see, e.g., \cite{Silverman86,DevroyeGyofri, Scott1992Multivariate,tsybakov2008introduction,Gramacki2017NonparametricKDE,wang2019nonparametric}.
%In the continuous case, the histogram is defined by discretizing the domain into cubic bins with edge length $h$, 
%where $h$ can be adjusted to optimize the quality of density estimation.
%Another widely used nonparametric method for continuous density estimation is the kernel density estimator (KDE), which incorporates each data point via small density bumps, which are then summed together. 
%To construct a KDE, the bandwidth, denoted by $h$, is an important parameter that controls the amount of smoothing applied to the density estimate. %To build a KDE, one needs to tune $h$, the  bandwidth that controls the amount of smoothing. The choice of  the bandwidth $h$ and the number of bins play a key role in the quality of these two classical estimation methods (histogram and KDE). 
Asymptotically, these estimators can consistently recover any density in the total variation ($L_1$) distance, if $nh^{m}\rightarrow \infty$, where $m$ is the dimension, $n$ is the sample size, $h$ is the tuning parameter (bin width for the histogram in the continuous case and bandwidth for the KDE), and we assume that $h\rightarrow 0$, $n\rightarrow \infty$, see, e.g., \cite {DevroyeGyofri}. However, the rate of convergence of these estimators is known to be drastically deteriorating with the dimension, even when $h$ is chosen optimally under general smoothness assumptions on the underlying density. This leads to suggestions of other density estimators that overcome the curse of dimensionality under more assumptions on the underlying density than only smoothness. An early suggestion is Projection Pursuit density estimation (PPDE) \cite{FriedmanStuetzle1984projection-pursuit}, which is an iterative algorithm to find the subspace spanned by a few significant components. PPDE is addressing the setting where there exists a linear map that transforms the underlying random vector to a smaller dimensional random vector with independent components. This technique is rather popular but, to the best of our knowledge, theoretical bounds on the performance of PPDE are not available, see a recent survey on PPDE in \cite{wang2019nonparametric}. A close but different model for density estimation arises from independent component analysis (ICA), where one assumes the existence of a linear bijection of the underlying random vector to a random vector of the same dimension with independent components \cite{samarov2004nonparametric}. It is shown that under this model there is no curse of dimensionality in the sense that there exist estimators achieving one-dimensional rates \cite{samarov2004nonparametric,samarov2005aggregated,amato2010noisy,v2020structural}. 
Finally, a recent line of work starting from \cite{pmlr-v32-songa14} and further developed in \cite{9779133,9740538, pmlr-v89-kargas19a, 10.5555/2999792.2999972, vandermeulen2021beyond,Vandermeulen2023} deals with the multi-view model for density estimation, that is, a finite mixture model whose components are products of one-dimensional Lipschitz continuous probability densities. The fact that this model is free from the curse of dimensionality is demonstrated in  \cite{vandermeulen2021beyond} through a theoretical analysis of its sample complexity. However, \cite{vandermeulen2021beyond} does not develop computationally tractable density estimators. 
\vspace{1mm}
%
%In nonparametric estimation, it is usually assumed that the unknown density $f$ over $\R^d$ belongs to
%some “massive” class $\mathcal{G}$ of densities.  In particular, distribution-free bounds for nonparametric density estimation have been obtained assuming that the target distribution is in  Sobolev or H\"{o}lder class with parameter $\beta>0$. 
%Over such classes, the classical minimax estimation rate in quadratic loss over $\R^d$ is known to be $n^{-\frac{\beta}{2\beta+d}}$, where $n$ denotes the number of observations, see~\cite{tsybakov2008introduction}.


%In the present paper, we propose a new histogram-style estimator for two-dimensional density estimation. 
%Our estimator  is  piecewise constant on bins defined by a grid.   
%Under the assumption that the target distribution belongs to a multi-view model, we %remove the square penalty on the convergence rate on $h\rightarrow 0$ which 
%explicitly construct estimators achieving faster rates compared to the standard histogram estimator.  The potential for faster convergence rates under low-rank constraint has been acknowledged in previous work, such as \cite{9779133,9740538, pmlr-v89-kargas19a, pmlr-v32-songa14,  10.5555/2999792.2999972, vandermeulen2021beyond}. In particular, \cite{vandermeulen2021beyond} was the first to demonstrate it through a theoretical analysis of the sample complexity. 

 In this paper, we focus on two-dimensional density estimation and consider a new model that generalizes the multi-view model in two aspects. We call it the {\it generalized multi-view model}. First, in contrast to the usual multi-view model, we do not assume the additive components to be products of densities but rather products of arbitrary functions. Second, we do not assume these functions to be Lipschitz continuous. We only need Lipschitz continuity of the overall two-dimensional density, which is a sum of $K$ such products. We propose a new estimator that is both computationally tractable and offers improved statistical guarantees
 by achieving the one-dimensional estimation rate to within a logarithmic factor. We also provide a numerical evidence that our estimator outperforms classical estimators.  Though the $L_2$-norm risk is by far the most studied in the literature on density estimation, our analysis deals with its $L_1$-norm counterpart. 
As argued in \cite{DevroyeGyofri}, using the $L_1$ norm to characterize the error of density estimation has several advantages. Indeed, the $L_1$ distance between two densities is equivalent, up to a multiplicative constant factor, to the total variation distance between the corresponding probability measures. 
Moreover, the $L_1$ norm is transformation invariant. 
On the technical side, dealing with the $L_1$ rather than the $L_2$ norm is more difficult. 

\vspace{1mm}

Our approach to tackle generalized multi-view models is based on a reduction to the problem of estimating multivariate discrete distributions under low-rank structure that we also consider in detail.
This problem is of independent interest and it arises in many applications, 
in particular, if the aim is to find correlations between categorical random variables, which is a particularly relevant subject \cite{}.
%The interaction between discrete random variables can be fully characterized by determining their joint distribution. 
%However, the problem's dimensionality can rapidly increase for multivariate discrete data, making dimension reduction techniques such as PCA, as well as low-rank assumption, an attractive way of overcoming this difficulty.
Without structural assumptions, estimating a discrete distribution on a set of cardinality $D$ in total variation distance 
%over $d$ elements with $n$ iid observations 
is associated with the minimax risk of the order of $\sqrt{{D}/{n}}$, where $n$ is the number of observations (see \cite{kamath2015learning,han2015minimax}).
However, by imposing certain structure assumptions, it is possible to reduce the estimation risk. Several assumptions, including monotonicity, unimodality, $t$-modality, convexity, log-concavity or $t$-piecewise degree $k$-polynomial structure have been considered in the literature (see, for example, ~\cite{canonne2018testing,diakonikolas2015differentially,durot2013least}).
In the present paper, we deal with a different setting where a multivariate discrete distribution is estimated under a low-rank structure. 
Specifically, for two integers $d_1, d_2 \geq 2$, we consider the problem of estimating a discrete distribution on a set of cardinality $D=d_1d_2$ defined by a matrix of probabilities $P = (P_{ij})_{i \in [d_1] ,j \in [d_2]}$ with rank at most $K \geq 1$. 
This setting arises, for example, in the analysis of data represented as a table with $n$ rows and 2 columns.
Each row corresponds to one individual, while each column contains information about one feature of the individual, for instance, $(1)$ eye color, and  $(2)$ hair color.
%, $\dots$, $(M)$ height. 
We assume that the value of the cell in the table is a categorical random variable, for example, that hair color can only take $6$ possible values: black, brown, red, blond, gray, white. 
Thus, each element of the $\ell$-th column has a discrete distribution over $\{1,\dots,d_\ell\}$, for some $d_\ell \geq 2$, $\ell=1,2$.
The individuals are assumed to be iid but the columns can be correlated. For instance, hair color can be correlated with eye color.
In other words, each row can be viewed as a realization of a pair of correlated discrete random variables.
%$M$-tuple $(j_1,\dots, j_M) \in [d_1]\times \dots \times [d_M]$, the random values $j_1,\dots, j_M$ being correlated. 
If we are interested in possible associations between the two variables, we are lead to estimating their joint distribution. Assuming that $P$ has low rank means that there exists a reduced representation of the correlation structure.
A basic unbiased estimator of $P$ is a histogram $Y/n$ where $Y$ is a $d_1\times d_2$ matrix such that its $(i,j)$-th entry $Y_{ij}$ is the number of individuals whose row in the data table equals $(i,j)$. 
However, the histogram does not take advantage of low rank structure and it only attains the slow rate $\sqrt{d_1d_2/n}$ in the total variation distance. We will suggest an estimator attaining a faster rate and show that it is minimax optimal up to logarithmic factors.  
% Another common model relying on low-rank structures for multinomial data is topic modeling, which has recently attracted a great deal of attention~\cite{ke2022using,cai2023testing,klopp2021assigning}.


%Now, consider the order-$M$ tensor $Y \in \R^{d_1 \times \dots \times d_M}$ defined as follows. For any $j = (j_1,\dots, j_M) \in [d_1]\times \dots \times [d_M]$, assign to $Y_j$ the number of individuals whose row in the database exactly equals $(j_1,\dots, j_M)$. The tensor of observations $Y$ therefore represents an $M$-dimensional histogram. Define $P = \E\frac{Y}{n}$. The tensor $P$ therefore represents the underlying probability distribution of the individuals in the database. 
 %\\

%The natural notion of rank which we would like to choose is a superposition of $K$ rank-1 tensors: $P = \sum\limits_{k=1}^K ~ \pi_k \hspace{-1mm} \bigotimes\limits_{\ell=1}^M p_\ell^{(k)}$. This assumption is natural if we assume a mixture model with $K$ unobserved components. Namely, if $\pi = (\pi_k)_k$ and $p_\ell^{(k)}$ are probability vectors for all $k,\ell$, then this model poses the existence of a latent variable $Z$ that can take up to $K$ values and that, conditional on $Z$, each row of the database has independent entries. \\

%In this paper, we only consider the matrix case ($M=2$) and leave the tensor case for future work.
%A classical motivation for low-rank matrix estimation or completion is the Netflix challenge. 
%Given $k \approx 5\cdot 10^7$ users and $m \approx 5 \cdot 10^4$ movies, we consider a $m \times k$ matrix $Y$ where each entry $a^*_{ij}$ denotes the rating given by user $j$ to movie $i$.
%Each user has only rated a small number of the $m$ movies so that most of the entries of $Y$ are unobserved.
%A natural assumption is that $Y = A^* + W$ where $A^*$ has a small rank, and that $W$ is some $\sigma$-subgaussian matrix noise.
%The low-rank assumption allows to dramatically reduce the numbers of degree of freedom in the estimation problem, by making it much smaller than the total number of entries. 
%This allows recovering the whole matrix even when only a tiny number of entries are observed. 
%Without the low-rank assumption, the minimax estimation rate in squared Frobenius norm is $\sigma^2 mk$ %\ju{vérifier avec le $\delta$} 
%whereas under the assumption that $A^*$ has rank at most $K$, the minimax rate scales as $\sigma^2 K (m+k)$.\\

%The paradigm of LRMC has received much attention \cite{candes2009exact, candes2010power}. Over the years, there have been lots of works
%on this topic~\cite{candes2015phase, hu2012fast,mishra2014fixed,dai2010set}.
%The classical technique to achieve this rate relies on a hard or soft thresholding of the SVD \cite{giraud2021introduction, johnstone2002function, bunea2011optimal,hastie2015matrix}.




%There are a variety of scenarios where the number of observed entries of a matrix is tiny. In the recommendation systems, for example, users are recommended to submit
%the feedback in a form of rating number, e.g., 1 to 5 for the purchased product.

\section{Contributions and related work}
%\ju{\cite{vandermeulen2021beyond}: Density estimation with low-rank structure, but no explicit algorithm and no lower bounds + Udell, + Papier Olga avec Moulines + Cécile Durot}


%Convergence in different norms ($L_1$, $L_2$, $L_\infty$) of the two most popular nonparametric density estimators, KDE and the histogram, have been extensively studied in the literature, such as in \cite{daglib,DevroyeGyofri, pmlr-v70-jiang17b, tsybakov2008introduction}. 
%Several variations of the classical KDE estimator have also been proposed, including robust KDE \cite{JMLR:v13:kim12b, pmlr-v30-Vandermeulen13} and KDE with variable bandwidth \cite{10.1214/aos/1176348768}. 
%Further nonparametric density estimators include the forest density estimator \cite{JMLR:v12:liu11a},  $k$-nearest neighbor density estimator \cite{MackRosenblatt}, estimators via  measure transport \cite{Wang2022OnMD} and etc. The problem of multivariate density estimation was studied in, e.g., \cite{samarov2004nonparametric, samarov2005aggregated,  amato2010noisy,  Rebelles2015pointwise, lepski2013mutivariate, rebelles2015adaptive, v2020structural}.


The importance of low-rank structures in nonparametric density estimation has been discussed in several papers suggesting and analyzing various estimation methods \cite{9779133,9740538, pmlr-v89-kargas19a, pmlr-v32-songa14,  10.5555/2999792.2999972, vandermeulen2021beyond}. In \cite{pmlr-v32-songa14}, the authors introduce the multi-view model and propose a kernel method for learning it but do not study whether it can lead to an improvement in nonparametric density estimation. 
The paper \cite{10.5555/2999792.2999972} provided empirical evidence that hierarchical low-rank decomposition of kernel embeddings can lead to improved performance in density estimation. 
More recently \cite{9779133,9740538} use a low-rank characteristic function to improve nonparametric density estimation. Finally, \cite{vandermeulen2021beyond} shows that there exists a universally consistent histogram-type estimator that converges in $L_1$ norm
to any multi-view model with a finite number of Lipschitz continuous components
at a rate $O\big(n^{-1/3}\big)$. This estimator is not constructed explicitly and is not computationally tractable in general. Furthermore, \cite{vandermeulen2021beyond} shows that the standard histogram estimator
can converge at a rate slower than $O\big(n^{-1/d}\big)$ on the same class of densities, where $d$ is the dimension. 

\vspace{1mm}
 
A closely related problem of estimating a low-rank probability matrix from discrete counts has been considered in~\cite{Jain2020linear}, where the authors propose a polynomial time algorithm (called the curated SVD) for the case of square matrix, $d_1=d_2=d$, and requiring the exact knowledge of the rank $K$. {\color{red}They prove an upper bound on the total variation error of the curated SVD that scales as $\psi(K,d,n):=1 \land \sqrt{\frac{Kd}{n}}$ (to within a logarithmic factor in $K,n$) with probability at least $1-d^{-2}$. They also provide a lower bound with the rate $\psi(K,d,n)$ {\it in expectation} by referring to the lower bounds of ~\cite{han2015minimax,kamath2015learning} for general discrete distributions on a set of cardinality $D=Kd$. Based on that, the authors in~\cite{Jain2020linear} claim minimax optimality of the rate $\psi(K,d,n)$, up to logarithmic factors. However, their argument only proves this optimality under significant restrictions on $K,d,n$ that they do not indicate. First, the lower bounds of~\cite{han2015minimax,kamath2015learning} are only meaningful under some specific conditions on $D,n$. For example, the lower bound of \cite[Theorem 1]{han2015minimax} is vacuous for $D\asymp 1$ and the lower bound of \cite[Lemma 8]{kamath2015learning} is vacuous for $D\asymp \sqrt{n}$. Second, comparing lower bounds in expectation with upper bounds in probability needs some care. Direct comparison is obviously not legitimate but the upper bound in probability in~\cite[Theorem 2]{Jain2020linear} can be transformed into a bound in expectation at the expense of adding a $O(d^{-2})$ term to the rate. This adds one more restriction $d^{-2} \lesssim \psi(K,d,n)$ to match the lower bound up to a logarithmic factor.}
The algorithm in~\cite{Jain2020linear} is based on normalization of the probability matrix by rescaling each row and column. 
Similar ideas have been developed in the literature on topic models, where topic matrices are estimated using an SVD-based technique on a rescaled corpus matrix~\cite{ke2022using}.
In contrast, our algorithm does not need to rescale the input matrix and rather relies on splitting of the matrix into sub-matrices with entries of similar order of magnitude. 

\vspace{2mm}


The contributions of the present work are as follows. 
\begin{itemize}
    \item For discrete distributions, {\color{red} we first prove minimax lower bounds in the total variation norm for discrete distributions on a set of cardinality $D$. We generalize~\cite{han2015minimax,kamath2015learning} in the sense that we derive lower bounds not only in expectation but also in probability and, in contrast to those works, we obtain the lower rate $1 \land \sqrt{\frac{D}{n}}$ for all $D,n\ge 1$ with no restriction. Under the low-rank matrix structure, this implies lower bounds of the order of $\psi(K,d,n)$  both in expectation and in probability, with no restriction on $K,d,n$.} 
    Next, we propose a computationally efficient algorithm to estimate a low-rank probability matrix  $P$ and show that it attains the same rate $\psi(K,d,n)$. Thus, we prove the minimax optimality of this rate with no restriction on $K,d,n$. Our algorithm is adaptive to the unknown rank $K$, which is not the case of the curated SVD~\cite{Jain2020linear}.
    %prove  that the minimax estimation rate under the low-rank assumption on matrix $P$ is
%for all $\alpha \geq 1$ and for $\delta = d^{-\alpha}$, we have
%$1 \land \sqrt{\frac{Kd}{n}}$ up to logarithmic factors (see Theorem \ref{th:main_th}), and that it can be attained adaptively to the unknown rank $K$. Here, $d=d_1\vee d_2$.
%\ju{Vérifier l'exposant avec la preuve de Koltchinkskii}
%We can compare this rate with the classical rate for multinomial estimation.
%With no structure assumption on $P$, the problem is equivalent to estimating a multinomial distribution of size $d_1 d_2$ based on a sample of size $n$.
%By~\cite{han2015minimax,kamath2015learning}, 
%the minimax rate under the total variation risk associated with this problem is $\sqrt{\frac{d_1d_2}{n}} \land 1$ in expectation. Also, \cite{canonne2020short} provides an upper bound with this rate in probability. 
%In other words, $d_1d_2/\epsilon^2$ observations are needed in order to estimate $P$ to within $\epsilon$ total variation error. 
%This becomes prohibitive in the high-dimensional setting where $d_1d_2 \gg n$.
%Under  the low-rank structure assumption, Theorem~\ref{th:main_th} ensures that even in the regime where $d_1d_2 \gg n$, estimating $P$ remains possible provided that  $n\gtrsim \frac{K d}{\epsilon^2}$ up to logarithmic factors. %where $K \ll d_1 \land d_2$.  
% On the difference from \cite{Jain2020linear} our estimator is adaptive to $K$, and we have no condition that $d$ is big enough compared to $n$ to match the upper and lower bounds. We provide a numerical study that supports our theoretical findings. 
\item We propose a new method of estimating continuous densities under the generalized multi-view model.  
Our algorithm achieves the rate of convergence $\left (K/n\right)^{1/3}$ (up to logarithmic factors) on the class of densities that are (i) Lipschitz continuous over an unknown sub-rectangle of $[0,1]^2$ and (ii) represented as a sum of $K$ separable components. We improve upon the prior work~\cite{vandermeulen2021beyond} in several aspects:
\begin{itemize}
    \item Our estimator attains the rate $\left (K/n\right)^{1/3}$ under the generalized multi-view model described above, and not only under the standard multi-view model.
     \item Our estimator is computationally tractable.
    \item Our algorithm is adaptive to the unknown number of separable components $K$ and to the unknown support of the density.
    \item We derive an information-theoretic lower bound proving that the above convergence rate is minimax optimal.
\end{itemize}
\item {\color{red} We conduct a numerical experiment demonstrating the efficiency of our estimators both in discrete and continuous settings, and we provide a package for their computation available at https://github.com/hi-paris/Lowrankdensity}
\end{itemize}
 




\section{Notation}

For any two real numbers $x,y$, we define $x\land y := \min(x,y)$ and $x \lor y := \max(x,y)$. 
For any $d \in \N$, we define $[d] = \{1, \dots, d\}$ and for any matrix $A$, we denote by $\rk(A)$ the rank of $A$.
For any vector or matrix  $P$ and for any $n \in \N^*$, we will denote by $\M(P,n)$ the multinomial distribution with probability parameter $P$ and sample size $n$. 
We denote by $\|A\|$ the operator norm and by $\|A\|_*$ the nuclear norm of any matrix $A \in \R^{d_1\times d_2}$. For any matrix $\Lambda $, and we write 
\begin{align*}
    &\|\Lambda\|_{1,\infty} = \max_{j} \sum_{i} |\Lambda_{ij}| ~\text{ for the maximum column norm,}\\
    & \normsquare{\Lambda} = \|\Lambda\|_{1,\infty} \lor \|\Lambda^\top\|_{1,\infty}.
   % & \Yl = \frac{H^{(\ell)}}{n}, ~~ \text{ for } \ell=1,2
\end{align*}

We denote by $\|\cdot\|$ the Euclidean norm over $\R^2$, and we denote by $\Supp (f) = f^{-1}\left(\R\setminus\{0\}\right)$ the support of any real-valued function $f$. 
 If $A$ is a one-dimensional set, i.e. $A\subset \R$, then $\mathbb 1_A$ denotes the function $x \mapsto \mathbb 1_{x\in A}$. If $A$ is a two-dimensional set, then $\mathbb 1_A$ denotes the function $(x,y) \mapsto \mathbb 1_{(x,y)\in A}$. 
Note that in the present paper, the absolute constants denoted by $C$ may take different values on each appearance.


==> contents_low_rank/Lower_bound.tex <==
\subsection{Lower bound: Proof of Proposition~\ref{prop:LB}}

We first state the following two propositions which guarantee that a  lower bound for estimating rank-$K$ multinomial matrices of size $d_1 \times d_2$ is of the order of $\left(K(d_1+d_2)/n\right)^{1/2}$. In what follows, the absolute constants are allowed to vary from line to line.


\begin{lemma}\label{LB_expectation}(Lower bound in expectation)
There exists an absolute constant $c>0$ such that $$R^* \geq c \, \sqrt{\frac{K(d_1+d_2)}{n}}.$$
\end{lemma}


\begin{lemma}\label{LB_proba}(Lower bound in high probability)
There exist two absolute constants $c, c'>0$ such that, for all $\delta \in (0, c')$ and any estimator $\hat P$, we have:
$$ \inf_{\hat P} \sup_{P \in \mathcal{D}_K} ~ \mathbb{P}_P\left(\|\hat P - P\|_1 \geq c \; \sqrt{\frac{K(d_1+d_2)}{n}}\right) \geq \delta$$
where $\mathcal{D}_K$ is defined in \eqref{def_DK}.
\end{lemma}

%\subsection{Proof of the lower bound}

\begin{proof}[Proof of Lemma~\ref{LB_expectation}]
Without loss of generality, assume that $d_2 \geq d_1$ and set $D_2 = \lfloor d_2/2 \rfloor$ and $d = 2 K D_2$. We also define $\gamma = \mbox{\fontsize{13pt}{12pt}\(\left(\frac{\cgamma}{\sqrt{n d}}\land \frac{1}{2d}\right)\)}$ where $\cgamma$ is an absolute constant which can be chosen small enough. For all $\epsilon=(\epsilon_{ij}) \in \{\pm 1\}^{K \times D_2}$, define the matrix $P_\epsilon$ as follows:

\begin{equation}\label{def_perturbed_mat_expect}
    \forall (i,j) \in \big[d_1\big] \times \big[d_2\big]: ~ P_\epsilon(i,j) =  \begin{cases}\mbox{\fontsize{13pt}{12pt}\(\frac{1}{d}\)} + \mbox{\fontsize{13pt}{12pt}\( \epsilon_{ij}\)}\gamma & \text{ if } i \leq K \text{ and } j \leq D_2, \\  \mbox{\fontsize{13pt}{12pt}\(\frac{1}{d}\)} - \mbox{\fontsize{13pt}{12pt}\( \epsilon_{i(j-D_2)}\)} \gamma & \text{ if } i \leq K \text{ and } 2D_2 \geq j > D_2, \\  0 & \text{ otherwise,}\end{cases}
\end{equation}
Consider the set of hypotheses 
\begin{equation}\label{Hypotheses_LB_expectation}
\mathcal{P} = \left\{P_\epsilon ~\big|~ \epsilon \in \{\pm 1\}^{K \times D_2} \right\}.
\end{equation}

This set contains $2^m$ hypotheses where $m = KD_2$. All matrices $P \in \mathcal{P}$ are of rank $K$ and have nonnegative entries summing to $1$. 
Over $\mathcal{P}$, the $\ell_1$ distance simplifies as follows:
\begin{align}
    \forall \epsilon, \epsilon' \in \{\pm 1\}^{K \times D_2}: \|P_\epsilon - P_{\epsilon'}\|_1 = 4\gamma\; \rho(\epsilon, \epsilon'), \label{TV_Hamming}
\end{align}
where $\rho(\epsilon,\epsilon') = \sum\limits_{i=1}^K \sum\limits_{j=1}^{D_2} \mathbb{1}_{\epsilon_{i,j} \neq \epsilon'_{i,j}}$ denotes the Hamming distance between $\epsilon$ and $\epsilon'$. 

Next, we apply Assouad's Lemma (see, e.g.,  Theorem 2.12. $(ii)$ in \cite{tsybakov2008introduction}). Let $\epsilon, \epsilon' \in \{\pm 1\}^{K \times d_2}$ such that $\rho(\epsilon,\epsilon') = 1$ and denote by $i_0 \in [d_1]$ and $j_0 \in [D_2]$ the unique indices such that $\epsilon_{i_0, j_0} = -\epsilon'_{i_0, j_0}$. By Lemma 2.7 in \cite{tsybakov2008introduction}, we have
\begin{align}
   TV\left(P_\epsilon^{\otimes n}, P_{\epsilon'}^{\otimes n}\right) &\leq \sqrt{\chi^2\left(P_\epsilon^{\otimes n} \; || \; P_{\epsilon'}^{\otimes n}\right)}  = \sqrt{\left(1+\chi^2\left(P_\epsilon \; || \; P_{\epsilon'}\right)\right)^n -1}, \label{TV_leq_chi2}
\end{align}

and 
\begin{align*}
    \chi^2\left(P_\epsilon \; || \; P_{\epsilon'}\right) &= \sum_{i=1}^K \sum_{j=1}^{d_2} \frac{\left(P_{\epsilon}(i,j) - P_{\epsilon'}(i,j)\right)^2}{P_{\epsilon'}(i,j)} \\
    &= \frac{\left(P_{\epsilon}(i_0,j_0) - P_{\epsilon'}(i_0,j_0)\right)^2}{P_{\epsilon'}(i_0,j_0)} + \frac{\left(P_{\epsilon}(i_0,j_0+D_2) - P_{\epsilon'}(i_0,j_0+D_2)\right)^2}{P_{\epsilon'}(i_0,j_0+D_2)} \\
    & \leq  \frac{4\gamma^2}{\frac{1}{d} - \gamma} \times 2 \leq 16 \gamma^2 d ~~ \text{ since } \gamma \leq \frac{1}{2d}\\
    & = 16 \left(\frac{\cgamma^2}{n} \land \frac{1}{4d}\right) \leq 16 \frac{\cgamma^2}{n}.
\end{align*}

Therefore, by \eqref{TV_leq_chi2}: $TV\left(P_\epsilon^{\otimes n}, P_{\epsilon'}^{\otimes n}\right) \leq \sqrt{\exp\left(16\cgamma^2\right) - 1} \leq \frac{1}{2}$ if the absolute constant $\cgamma$ is chosen small enough. 
Now Assouad's Lemma and  \eqref{TV_Hamming} imply
$$\inf\limits_{\widehat P} \max\limits_{P \in \mathcal{D}_K} \E\left[\|\widehat P - P\|_1\right] \geq \frac{4\cgamma}{\sqrt{nd}} \frac{d}{2} \left(1-\frac{1}{2}\right) \geq \frac{\cgamma}{2} \sqrt{\frac{d}{n}} \geq \frac{\cgamma}{4}\sqrt{\frac{K(d_1+d_2)}{n}}.$$

\end{proof}

\begin{proof}[Proof of Lemma \ref{LB_proba}]
Recall the definition of the cubic set of hypotheses $\mathcal{P}$ from \eqref{Hypotheses_LB_expectation} and set $d=Kd_2$, where \textit{wlog}: $d_1 \leq d_2$.
Let $\widehat{P}$ be any estimator of the probability parameter and write
\begin{equation}\label{def_r}
    r = \sqrt{\frac{K(d_1+d_2)}{n}}.
\end{equation}
We first justify that for this particular set of hypotheses, it is possible to assume without loss of generality that 
\begin{equation}\label{maximum_discrepancy}
    \|P - \widehat P\|_1 \leq 6 \gamma d \,\leq\, 6 \, \cgamma r.
\end{equation} 
Indeed, define $U = \left[\frac{1}{d} \,\mathbb{1}_{i \leq K }\right]_{i,j}$. If for some observation $Y$ the estimate $\widehat{P}(Y)$ satisfies $\|\widehat P(Y) - U\|_1 > 4\gamma d$, then it is possible to improve $\widehat{P}$ by replacing it with the estimator $\bar{P}$ satisfying $\|\bar P(Y) - P\|_1 \leq 6 \gamma d$ and defined as:
\begin{align*}
    \bar{P} := \widehat P \mathbb{1}\left\{\big\|\widehat P - U\big\|_1 \leq 4 \gamma d\right\} + U \mathbb{1}\left\{\big\|\widehat P - U\big\|_1 > 4 \gamma d\right\}.
\end{align*}
Indeed, recalling that $\forall P \in \mathcal{P}: \big\|U - P\big\|_1 = 2 \gamma d$, there are two cases.
\begin{itemize}
    \item If $\big\|\widehat P(Y) - U\big\|_1 \leq 4\gamma d$, then $\widehat P = \bar P$ so that $\big\|P - \bar{P}\big\|_1 \leq \big\|P - U\big\|_1 + \big\|U - \bar{P}\big\|_1 \leq 2 \gamma d + 4 \gamma d = 6 \gamma d$.
    \item  Otherwise, $\bar{P} = U$ and we get
\begin{align*}
    \big\|\bar P(Y) - P\big\|_1 & = 2\gamma d = 4 \gamma d - 2 \gamma d< \big\|\widehat P(Y) - U\big\|_1 -  \big\|U - P\big\|_1 \leq \big\|\widehat P(Y) - P\big\|_1,
\end{align*}
\end{itemize}

which proves that \eqref{maximum_discrepancy} can be assumed \textit{wlog}. Now, from the proof of Proposition \ref{LB_expectation}, we also have
\begin{align}
    \sup_{P \in \mathcal{P}} \E_P\big\|\widehat P - P\big\|_1 \, \geq \, \frac{\cgamma}{4} r =: Cr. \nonumber
\end{align}
Now, we can write $p := \sup\limits_{P \in \mathcal{P}} \mathbb{P}_P\left(\|\hat P - P\|_1 \geq cr\right)$ for $c = \cgamma \left(\frac{1}{4} - 6 \delta\right)> 0 $ for $\delta < \frac{1}{24} =: c'$. 
It follows that
\begin{align*}
    C r &\leq \sup_{P \in \mathcal{P}} ~ \E_P\big\|\widehat P - P\big\|_1 \\
    & = \sup_{P \in \mathcal{P}}\left\{~ \E_P\Bigg[\big\|\widehat P - P\big\|_1 \; \mathbb{1}\left\{\big\|\widehat P - P\big\|_1 \geq cr\right\}\Bigg] ~+ ~ \E_P\Bigg[\big\|\widehat P - P\big\|_1\; \mathbb{1}\left\{\big\|\widehat P - P\big\|_1 < cr\right\}\Bigg]~\right\}\\
    & \leq 6 \cgamma r \cdot p \, + \, cr \hspace{3mm} \text{ by equation \eqref{maximum_discrepancy}, so that } ~ p \geq \frac{C-c}{6\cgamma} \geq \delta.
\end{align*}

\end{proof}



==> contents_low_rank/Motivation.tex <==
\subsection{Motivation}
Consider a database gathering information about $M$ particular features for $n$ iid individuals. 
For example, suppose that for each individual, we observe $(1)$ their eye color, $(2)$ their hair color, $\dots$, $(M)$ their height. 
Denote by $P$ the unknown distribution of each individual $X_i$.
For all $i=1,\dots,n$, the observation $X_i$ therefore consists of $M$ pieces of information which are allowed to be correlated: $X_i = \big(X_i^1, \dots, X_i^M\big)$. 
In this setting, each marginal random variable $X_i^{m} $ (for $m=1, \dots, M$) follows some unknown discrete distribution with parameter $p_m = \left(p_m(1), \dots, p_m(d_m)\right)$ over $\{1, \dots, d_m\}$ for some $d_m \geq 2$, i.e. $\forall j \in \{1, \dots, d_m\} : p_m(j) \geq 0$ and $\sum_{j=1}^{d_m} p_m(j) = 1$.
However, the joint distribution $P$ does not correspond to the product distribution of the marginals: $P \neq \bigotimes\limits_{m=1}^M p_m$. 
Rather, we assume that $P$ has a structure of low rank tensor. This assumption encompasses all mixture models with $K$ components: $P = \sum\limits_{k=1}^K ~ \pi_k \hspace{-1mm} \bigotimes\limits_{m=1}^M p_m^{(k)}$ but is not restricted to this case.  \\

%\ju{We need $K \ll d_1 \land \dots \land d_M$ which means that each dimension has to be quite large in order to have a real improvement. To justify this, just consider numerical variable rather than actual categorical variable that are discrete (example : height, salary)}

==> contents_low_rank/Notation.tex <==
\section*{Notation to keep throughout}
Below are listed a few commands that need to be used systematically throughout the paper. For example, if you need to use the notation $\cgamma$ somewhere, please always use \verb+\cgamma+ in the code rather than \verb+c_\gamma+. If at some point we need to change the notation, it will be very easy to do so: Indeed, all the commands are defined around line 60 in the main file. With this system, it is possible to change some notation in the whole document by just changing it once in the main file where it is defined. If you need to introduce some new notation too, please define it in the main file and report it here so that everyone can use it easily.
\begin{itemize}
    \item $\cgamma$: \verb+\cgamma+
    \item $\rk$: \verb+\rk+
    \item $\M$: \verb+\M+
    \item $\Poi$: \verb+\Poi+
    \item $\Yone$: \verb+\Yone+; ~$\Ytwo$: \verb+\Ytwo+ ; ~ $\Yl$: \verb+\Yl+
    \item $\hatCone$: \verb+\hatCone+; ~$\hatCtwo$: \verb+\hatCtwo+; ~$\hatCl$: \verb+\hatCl+
    \item $\hatLone$: \verb+\hatLone+ ; ~ $\hatLtwo$: \verb+\hatLtwo+; ~ $\hatLl$: \verb+\hatLl+
    \item $\Mk$: \verb+\Mk+; ~$\Minfty$: \verb+\Minfty+; ~$\Pk$: \verb+\Pk+;$\Pinfty$: \verb+\Pinfty+; ~ ~$\hatPk$: \verb+\hatPk+ ; ~$\hatPinfty$: \verb+\hatPinfty+ 
\end{itemize}



==> contents_low_rank/Pb_statement_matrix.tex <==

For $K \geq 1$ and $d_1, d_2 \geq 2$, we denote the class of multinomial matrices of rank at most $K$ by 
\begin{equation}\label{def_DK}
    \mathcal{D}_K = \left\{P \in \mathbb{R}^{d_1 \!\times\! d_2} ~ \Big| ~ \text{rk}(P) \!\leq\! K, ~ \forall (i,j) \in [d_1] \!\times\! [d_2] : P_{ij} \geq 0 ~ \text{ and} \hspace{-1mm} \sum\limits_{(i,j) \in [d_1] \!\times [d_2\!]} \hspace{-5mm} P_{ij} = 1\right\}.
\end{equation}

Assume that for some unknown $P \in \mathcal{D}_K$, we are given iid observations $X_, \dots, X_n, ~ n \geq 1$ with distribution $P$, in other words, such that $\forall k \in [n], \forall (i,j)\in [d_1] \times [d_2]: \mathbb{P}(X_k = (i,j)) = P_{ij}$. We consider here the problem of minimax estimation of $P$ in the total variation distance

==> contents_low_rank/Pb_statement_tensors.tex <==

For all $d \in \N$, we define $[d] = \{1, \dots, d\}$ and for any tensor $A$ denote by $\rk(A)$ the rank of $A$. \ju{Define the notion of rank.} For $M,K \geq 1$ and $d_1, \dots, d_M \geq 2$, we denote by 
\begin{equation}\label{def_DK}
    \mathcal{D}_K = \left\{P \in \mathbb{R}^{d_1 \!\times\! \dots \!\times\! d_M} ~ \Big| ~ \text{rk}(P) \!=\! K, ~ \forall \omega \in [d_1] \!\times\! \dots \!\times\! [d_M] : P_\omega \geq 0 ~ \text{ and} \hspace{-1mm} \sum\limits_{\omega \in [d_1] \!\times \dots \times\! [d_M\!]} \hspace{-5mm} P_\omega = 1\right\},
\end{equation}

the class of multinomial tensors of order $M$, of dimension $d_1 \times \dots \times d_M$ and of rank $K$. Assume that for some unknown $P \in \mathcal{D}_K$, we are given iid observations $X_, \dots, X_n, ~ n \geq 1$ with distribution $P$, in other words, such that for each multi-index $\omega \in [d_1] \times \dots \times [d_M]: \mathbb{P}(X_i = \omega) = P_\omega$. We are interested in the minimax estimation of $P$ with high probability.

==> contents_low_rank/Poubelle.tex <==
We finally handle the case of $I_{T+1}$ and $J_{T+1}$. By definition we have $\|\Pinfty\|_{1,\infty} \lor \big\|{\Pinfty}^\top\big\|_{1,\infty} \leq 2^{-T -1}$. Therefore, 
\begin{align*}
    \|\hatPinfty - \Pinfty\|_F^2 &\leq K \|W_{\infty}\|_{op} \\
    &\leq K \frac{1}{n} \log d \|\Pinfty\|_{1,\infty} \lor \big\|{\Pinfty}^\top\big\|_{1,\infty} ~~ \text{with probability $\geq 1-\frac{1}{d}$ by Olga's Lemma}\\
    & \leq \frac{1}{n}\frac{K \log d}{2^{T +1}}.
\end{align*}

Moreover, using $\|\cdot\|_1 \leq \|\cdot\|_F \sqrt{d_1d_2}$ over $\R^{d_1\times d_2}$, and using $2^{-T-1} \leq e^{-(C_T \log d)\log 2} \leq 1/d$ for $C_T$ large enough, we get:
\begin{align*}
    \|\hatPinfty - \Pinfty\|_1 \leq \sqrt{d_1d_2} \sqrt{\frac{1}{n}\frac{K \log d}{2^{T +1}}} = \sqrt{d_1d_2}\sqrt{\frac{ K \log d}{nd} } \leq \sqrt{\frac{K d\log d}{n}},
\end{align*}
with probability $\geq 1-\frac{1}{d}$.
We can now combine all of our estimators. Let $(i,j) \in [d_1]\times [d_2]$. Note that each pair $(i,j)$ belongs to at least one of  the $U_k$ and to at most two of them \ju{(clarify this)}. 
For fixed $(i,j)$, let $t(i,j)$ be the set of integers $t$ such that $(i,j) \in U_k$. For this pair, we average the estimates $\hatPk(i,j)$ for $t \in t(i,j)$. We repeat for all pairs in order to get our final estimator $\widehat P$. We can now analyze its estimation guarantees:
\begin{align*}
    \|\widehat P - P\|_1 &\leq \sum_{t=0}^{T+1} \|\hatPk - \Pk\|_1 \leq (C_T \log d +1)\sqrt{\frac{8 K d\log d}{n}} + \sqrt{\frac{K d\log d}{n}}\\
    & \leq \sqrt{\frac{Kd}{n}} \log^{3/2} d,
\end{align*}
with probability $1-O\big(\frac{\log d}{d}\big)$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ju{\begin{lemma}\label{lem:Poisson_small}
Let $C,C'>0$ be absolute constants and $N \leq C \log^2 d$. Let $\lambda_1,\dots, \lambda_N \geq C' \log N$ and let $Z_i \sim \Poi(\lambda_i)$ be mutually independent random variables.
It holds
$$ \mathbb{P} \left(\min_{i=1}^N Z_i < \right)$$
\end{lemma}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


    
    \textbf{First case:} Assume that $L(R-r)^2 \leq \frac{1}{2}$. 
    %Since $f$ is supported over the interval $[r,R]$, whose length is smaller than $h = Cn^{-1/3} L^{-1/2}$, we show that we can estimate $f$ by a constant over $[\widehat r, \widehat R]$. 
    %In the present case, our estimator is $\widehat R - \widehat r \leq n^{-1/3} L^{-1/2}$ so that $\widehat f = \frac{1}{\widehat R - \widehat r} \mathbb 1_{[\widehat r, \widehat R]}$. 
    %We can also bound the maximum and the minimum of $f$ as follows. 
    We have the following relations
    \begin{itemize}
        \item First, $1 = \int_{\R} f \leq (R-r)\max f$, so that $\max f \geq (R-r)^{-1}$, and similarly, $\min f \leq (R-r)^{-1}$. 
        \item Moreover, by the Lipschitz assumption, we also have $\max f \leq \min f + L(R-r) \leq (R-r)^{-1} + L(R-r) \leq 2(R-r)^{-1}$, so that $(R-r) \max f\leq 2$.
        \item Similarly, $\min f \geq \max f - L(R-r) \geq (R-r)^{-1} - L(R-r) \geq \frac{1}{2}(R-r)^{-1}$.
    \end{itemize}
    %As for the minimum, by continuity of $f$ over $[r,R]$, there exists $x_0 \in [r,R]$ such that $f(x_0) (R-r) = \int_r^R f$.     Therefore, $1 \geq \int_{\R} f \geq \int_r^R \min f(x) + L|x-x_0| dx = (R-r)\min f + L(R-r)^2/4$ so that $\min f \leq (R-r)^{-1} - L\frac{R-r}{4} \leq \frac{3}{4} (R-r)^{-1}$ by assumption.

These relations show that $\frac{1}{2} \leq (R-r) f \leq 2$ over $[r,R]$.
We consider the following event 
\begin{align*}
    \mathcal{E} = \left\{\frac{\widehat R - \widehat r}{R-r} \geq 1 - 1/\sqrt n\right\}.
\end{align*}
We have 
$\mathbb P(\mathcal{E}^c) \leq \mathbb P\left(\frac{R-\widehat R}{R-r} > \frac{1}{2\sqrt n}\right) + \mathbb P\left(\frac{\widehat r - r}{R-r} > \frac{1}{2\sqrt n}\right)$. 
Moreover,
\begin{align}
    \mathbb P\left(\frac{R-\widehat R}{R-r} > \frac{1}{2\sqrt n}\right) &= \mathbb P \left(X_1 < R - \frac{R-r}{2\sqrt n}\right)^n = \left(1 - \int_{R - \frac{R-r}{2\sqrt n}}^Rf\right)^n \label{eq:control_widehat_R}\\
    & \leq \left(1-\frac{R-r}{2\sqrt n}\min f\right)^n \leq \left(1-\frac{1}{4\sqrt{n}}\right)^n \leq e^{-\sqrt n/4},\nonumber
\end{align}
so that $\mathbb P (\mathcal{E}) \geq 1 - 2 e^{-\sqrt{n}/4}$. From now on, we place ourselves on the event $\mathcal{E}$ and recall that $n \geq C$ where $C$ is an absolute constant \ju{check si pas de double emploi de $C$}. 
Assume first that $\widehat R - \widehat r < h$. \ju{modifier l'algo en conséquence} 
Then, on $\mathcal{E}$, we have $R-r < h/(1-1/\sqrt{n})$. 
In this case, $\widehat f = \frac{1}{\widehat R - \widehat r} \mathbb 1_{[\widehat r, \widehat R]}$.
By continuity of $f$ over $[r,R]$, there exists $x_0 \in [r,R]$ such that $f(x_0)(R-r) = \int_r^R f = 1$.
We have:
\begin{align*}
    \|f-\widehat f\|_{L_1} &= \int_r^R |f(x)-\widehat f(x)|dx \leq \int_{\widehat r}^{\widehat R} |f(x)-\widehat f(x)|dx + \left(R - \widehat R + \widehat r - r\right) \max f\\
    & \leq \int_{\widehat r}^{\widehat R} |f(x)-f(x_0)|dx + \int_{\widehat r}^{\widehat R} |f(x_0)-\widehat f(x)|dx + \frac{R-r}{\sqrt n} \max f \quad \text{ over } \mathcal{E}\\
    & \leq L(R-r)^2 + \int_{\widehat r}^{\widehat R} |f(x_0)-\widehat f(x)|dx + \frac{2}{\sqrt n}\\
    & \leq \frac{Lh^2}{1-1/\sqrt{n}} + (R-r) \left|\frac{1}{R-r} - \frac{1}{\widehat R - \widehat r}\right| + \frac{2}{\sqrt n}\\
    & \leq \frac{C}{\sqrt{n}} \leq Cn^{-1/3}.
\end{align*}

Now, assume that $\widehat R - \widehat r \geq h$, so that, necessarily, $R-r\geq h$. 
Let $m = \left\lfloor r/h \right\rfloor$ and $M = \left\lfloor R/h \right\rfloor$, and recall that $\hat m = \lfloor \min Z_i/h \rfloor$, and $\hat M = \lfloor \max Z_i/h \rfloor$. 
We have $m\leq \widehat m \leq \widehat M \leq M$. 
Moreover, for any $j \in \{m,\dots,M\}$, we set $p_j = \int_{A_j(h)} f$ and $\widehat p_j = \int_{A_j(h)} \widehat f$. 
For $j \in \{m+1,M-1\}$, we also let $x_j \in A_j(h)$ be such that $h \cdot f(x_j) = \int_{A_j(h)} f$. 
Such a family $(x_j)_j$ exists since $f$ is continuous over $A_j(h)$ if $j \in \{m+1,M-1\}$.
Therefore, we have
\begin{align*}
    \int_\R |\widehat f - f| &= \int_{A_m(h) \cup A_M(h)} |\widehat f - f| + \sum_{j=m+1}^{M-1} \int_{A_j(h)} |\widehat f - f|\\
    & \leq \int_{A_m(h) \cup A_M(h)} \Big\{|\widehat f| + \max f\Big\} + \sum_{j=m+1}^{M-1} \int_{A_j(h)} |\widehat f(x) - f(x_i)| + |f(x_i) - f(x)| dx \\
    & \leq \frac{N_m + N_M}{n} + \int_{A_m(h) \cup A_M(h)} \max f dx + \sum_{j=m+1}^{M-1} \left\{|p_j - \widehat p_j| + Lh^2\right\}\\
    & \leq 
\end{align*}

\textbf{Second case}: Assume that $(R-r) \in \left[ n^{-1/3} L^{-1/2}, h\right]$, where we recall that $h = Cn^{-1/3} L^{-1/2}$. 
In this case, we show that $\widehat R - \widehat r$ is of the same order as $n^{-1/3} L^{-1/2} \asymp h$ with high probability. 
In this case, we prove that it is equivalent to split the estimated support $[\widehat r, \widehat R]$ into at most two cells of length $h$, since $R-r \leq h$, or to directly estimate $f$ by $\frac{1}{\widehat R - \widehat r}\mathbb 1_{[\widehat r, \widehat R]}$. 

Letting $x_0 \in [r,R]$ such that $f(x_0) = (R-r)^{-1}$ as above, we have $1 = \int_r^R f \leq \int_r^R \min f + L|x-x_0|dx \leq (R-r) \min f + L (R-r)^2$, so that $\min f \geq (R-r)^{-1} - L (R-r) \geq (R-r)^{-1}\left(1-Cn^{-1/3}\right) \geq \frac{1}{2}(R-r)^{-1}$ for $n \geq (2C)^3$.
We consider the following event:
\begin{align*}
    \mathcal{E}_2 = \left\{\widehat R - \widehat r \geq h/2C\right\}.
\end{align*}
We have $\mathbb P(\mathcal{E}_2^c) \leq \mathbb P \left(R-\widehat R > h/4C\right) + \mathbb P \left(\widehat r - r > h/4C\right)$. We have
\begin{align*}
    \mathbb P\left(R-\widehat R > h/4C\right) \leq \left(1- \int_{R-h/4C}^R f\right)^n \leq \left(1- \frac{h}{4C} \min f\right)^n \leq \left(1- \frac{R-r}{4C} \min f\right)^n \leq \left(1-\frac{1}{8C}\right)^n,
\end{align*}
so that $\mathbb P(\mathcal{E}_2) \leq 2\left(1-\frac{1}{8C}\right)^n$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Moreover, for $h = \frac{C}{n^{1/3}\sqrt{L}}$ where $C>0$ denotes an absolute constant, large enough, we define
\begin{align*}
    A_j(h) &= \left[jh, (j+1) h \right) \text{ for any } j \in \mathbb Z,\\
    C_{j,j'}(h) &:= A_j(h) \times A_{j'}(h) \text{ for any } j,j' \in \mathbb Z.
\end{align*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\ju{
\begin{itemize}
    %\item Example of low rank matrix which is not a mixture.
    \item Our result rely on the assumption that our underlying matrix has a low rank structure. An interesting development would be the problem of testing whether this low rank assumption is satisfied. + What happens in the miss-specified case?
    \item Explain why just one SVD does not work + Differences compared to usual isotropic noise. Développer
    \item Our estimator is improper (it does not necessarily have rank at most $K$) but is in the simplex and is minimax optimal for  estimating $P$. 
\end{itemize}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% simul K

\hfill 
\begin{minipage}[b]{0.3\textwidth}
    \centering
    \includegraphics[width = 1\textwidth]{New/Simulations/discret_K.png}
    \caption{Total variation error between our estimator from Algorithm~\ref{alg:Alg} and the probability matrix to estimate, as a function of the dimension the rank $K$. }
    \label{fig:simul_discrete_K}
\end{minipage}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Controlling multinomial noise 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



We will need the following auxiliary lemma on the concentration of Poisson random matrices.
\begin{lemma}\label{lemma:bound_Poisson_matrix}
	Consider the matrix $W=(w_{ij}-\lambda_{ij})_{(i,j)\in \nint{d_1}\times\nint{d_2}}$, where the $w_{ij}$ are independent Poisson random variables, $w_{ij}\sim \Poi(\lambda_{ij})$, with means  $\lambda_{ij}\in (0,1)$, $(i,j)\in \nint{d_1}\times\nint{d_2}$. 
	Set $\Lambda= (\lambda_{ij})_{(i,j)\in \nint{d_1}\times\nint{d_2}}$ and   $d=d_1\vee d_2$. 
	Then, for any $\alpha > 0$ there exists a constant $c>0$ depending only on $\alpha$ such that with probability at least $1-1/d^\alpha$,
	$$\|W\| \leq c
 \max\left\lbrace \sqrt{\normsquare{\Lambda}\log d},\; \log(d)\log\left(\sqrt{\frac{d_1d_2}{\normsquare{\Lambda}}}\right) \right\rbrace.
 $$
\end{lemma}
The following corollary is an immedeiate consequence of Lemma \ref{lemma:bound_Poisson_matrix}.

\vspace{2mm}

\begin{corollary}\label{cor:poisson_noise}
Let the assumptions of Lemma~\ref{lemma:bound_Poisson_matrix} be satisfied and $\normsquare{\Lambda} \geq c'$, where $c'>0$ is a constant. Then there exists a constant $c^*>0$ depending only on $\alpha$ and $c'$ such that with probability at least $1 - d^{-\alpha}$ we have 
$$ \|W\|^2 \leq c^* \normsquare{\Lambda} \log^4 d. $$
\end{corollary}





\vspace{2mm}


\begin{proof}[Proof of Lemma~\ref{lemma:bound_Poisson_matrix}]
The proof is based on the following proposition, which is  a straightforward generalization of Theorem 4 in  \cite{Koltchinskii2013} to rectangular matrices based on a self-adjoint extension.
\begin{proposition}
	\label{prop:Koltchinskii2013}
	Let $W_{1},\ldots , W_n$ be independent random matrices in $\mathbb{R}^{d_1\times d_2}$ such that $\E[{W_i}]=0$. Assume that
	\begin{equation}
		\delta_* = \max_{k\in\nint{n}}\, \inf %_{\delta>0}
  \left\lbrace \delta>0: \E[\exp\left(\|W_k\|/\delta\right)]\leq e\right\rbrace<+\infty.
	\end{equation}
	Then, there exists an absolute constant $c_*>0$ such that, for all $t>0$, with probability at least $1-e^{-t}$ we have
	$$\left\|\frac{1}{n}\sum_{k=1}^nW_k\right\|\leq c_*\max\left\lbrace \sigma_W\sqrt{\frac{t+\log d}{n}}, \delta_*\left(\log\frac{\delta_*}{\sigma_W}\right)\frac{t+\log d}{n} \right\rbrace,$$
	where $d=d_1\vee d_2$ and
	$$\sigma_W = \max\left\lbrace \left\|\frac{1}{n}\sum_{k=1}^{n}\E[W_{k}W_{k}^{\top}]\right\|^{1/2},\left\|\frac{1}{n}\sum_{k=1}^{n}\E[W_{k}^{\top}W_{k}]\right\|^{1/2} \right \rbrace.$$
\end{proposition}
In our case, we take $n=d_1d_2$ and apply Proposition \ref{prop:Koltchinskii2013} to the matrices $W_{k}=Z_{ij} = \left(w_{ij}-\lambda_{ij}\right)E_{ij}$, $k=(i,j)\in\nint{d_1}\times\nint{d_2}$, where $E_{ij}$ are the matrices of the canonical basis of $\mathbb{R}^{d_1\times d_2}$.  Notice that for the centered Poisson variables $w_{ij}-\lambda_{ij}$ we have, for all $i,j\in\nint{d_1}\times \nint{d_2}$, 
$$
\delta_{ij}={\operatorname{inf}}
\left\lbrace \delta>0: \E[\exp\left(\left|w_{ij}-\lambda_{ij}\right|/\delta\right)]\leq e\right\rbrace\leq 1. 
$$
It follows that $\delta_*\le 1$. 
Thus, applying Proposition \ref{prop:Koltchinskii2013} with 
\begin{equation}
	\label{eq:sigma-def-tail}
	\sigma_Z = \max\Bigg\lbrace \left\|\frac{1}{d_1d_2}\sum_{i=1}^{d_1}\sum_{j=1}^{d_2}\E[{Z_{ij}Z_{ij}^{\top}}]\right\|^{1/2},
	\ \left\|\frac{1}{d_1d_2}\sum_{i=1}^{d_1}\sum_{j=1}^{d_2}\E[{Z_{ij}^{\top}Z_{ij}}]\right\|^{1/2} \Bigg \rbrace
\end{equation}
we obtain that, for the matrix $W=\sum_{i=1}^{d_1}\sum_{j=1}^{d_2} Z_{ij}$ and any $t> 0$, the following inequality holds with probability at least $1-e^{-t}$: 
\begin{equation*}
	\|W\| \leq c_*\max\Bigg\lbrace \sigma_Z\sqrt{d_1d_2(t+\log d)},
\left (t+\log d\right )	\log\left(\frac{1}{\sigma_Z}\right) \Bigg\rbrace.
\end{equation*}
The value $\sigma_Z$ can be obtained explicitly. Indeed,
\begin{equation*}
	\sum_{i=1}^{d_1}\sum_{j=1}^{d_2}\E[{Z_{ij}Z_{ij}^{\top}}] = \sum_{i=1}^{d_1}\left\lbrace\sum_{j=1}^{d_2}\E[{\left(  w_{ij}-\lambda_{ij}\right)^2}]\right\rbrace E_{ii}(d_1) = \sum_{i=1}^{d_1}\left\lbrace\sum_{j=1}^{d_2}\lambda_{ij}\right\rbrace E_{ii}(d_1),
\end{equation*}
where $E_{ii}(d_1)$ denotes the $d_1\times d_1$ square matrix with $(i,i)$-th entry equal to 1 and all other entries 0. Therefore
\begin{equation*}
	\left\|\frac{1}{d_1d_2}\sum_{i=1}^{d_1}\sum_{j=1}^{d_2}\E[{Z_{ij}Z_{ij}^{\top}}]\right\|^{1/2} = \sqrt{\frac{1}{d_1d_2}\| \Lambda^{\top}\|_{1,\infty}}
\end{equation*}
and 
\begin{equation}
	\label{eq:sigma-def-tail_value}
	\sigma_Z = \sqrt{\frac{1}{d_1d_2}\| \Lambda^{\top}\|_{{1,\infty}}\vee \| \Lambda\|_{1,\infty}} = \sqrt{\frac{1}{d_1d_2}\normsquare{\Lambda}}.
\end{equation}
Setting $t = \alpha\log d$ we  obtain that, with probability at least $1-d^{-\alpha}$,
$$
\|W\| \leq c_*\max\left\lbrace \sqrt{(1+\alpha)\normsquare{\Lambda}\log d},\; (1+\alpha)\log(d)\log\left(\sqrt{\frac{d_1d_2}{\normsquare{\Lambda}}}\right) \right\rbrace,
$$
which proves the lemma.
\end{proof}


The next proposition provides a control on the operator norm of multinomial matrices. In the proofs of the main results, we use it with $c' = 2  \barc \alpha \log2$ where $\barc$ is the constant from Lemma~\ref{lem:concent_poisson}.
\begin{proposition}\label{prop:bound_Mult_matrix}
    Let $\alpha>0$ and let $P \in \R_+^{d_1\times d_2}$ be a matrix such that $\sum\limits_{i,j} P_{ij} = 1$, and  $H \sim \M(n,P)$ for $n \in \N^*$.
    Assume also that $n \geq \barc \alpha \log d$ where $\barc$ is the constant from Lemma~\ref{lem:concent_poisson} and $d = d_1\lor d_2$.
    Let $W = \frac{H}{n} - P$ denote the multinomial noise. 
    Let $Q$ be an extraction of $P$, that is $Q = (P_{ij})_{i\in I, j \in J}$ for some sets of indices $I \subseteq [d_1]$ and  $J \subseteq [d_2]$.
    Assume that $\normsquare{Q}\geq c'/n$ where $c'$ is the constant from Corollary~\ref{cor:poisson_noise} and set $W_Q = (W_{ij})_{i\in I, j \in J}$.
    There exists a constant $c^*$ depending only on $\alpha$ such that 
    \begin{align*}
        \mathbb{P}\left(\|W_Q\|^2 \leq c^* \frac{\normsquare{Q}}{n} \log^4 d\right)\geq 1 - 3d^{-\alpha}.
    \end{align*}
\end{proposition}


\begin{proof}[Proof of Proposition \ref{prop:bound_Mult_matrix}]
Let $\widetilde n \sim \Poi(2n)$ and $\widetilde H | \widetilde n \sim \M(\widetilde n, P)$. 
Using the Poissonization argument (Proposition \ref{poissonization_trick}) we have that $\forall (i,j) \in [d_1]\times [d_2], \widetilde H_{ij} \sim \Poi(2n P_{ij})$ and the random variables $\widetilde H_{ij}$ are independent.
Letting $\widetilde W = \widetilde H - 2nP$ and taking its extraction $\widetilde W_Q = (\widetilde W_{ij})_{i\in I, j \in J}$, we can therefore apply Corollary~\ref{cor:poisson_noise} to obtain
\begin{align*}
    1-d^{-\alpha} &\leq \mathbb{P}\left(\|\widetilde W_Q\|^2 \leq c^* \normsquare{2nQ} \log^2 d\right)\\
    &\leq \mathbb{P}\left(\widetilde n < n\right) + \mathbb{P}\left(\|\widetilde W_Q\|^2 \leq c^* \normsquare{2nQ} \log^2 d
    ~\Big|~\widetilde n \geq n\right)\\
    & (\text{faux})\leq 2e^{-\frac{c}{4} n} + \mathbb{P}\left(\|\widetilde W_Q\|^2 \leq c^* \normsquare{2nQ} \log^2 d ~\Big|~ \widetilde n = n\right) ~~ \text{ by~\cite[Exercise 2.3.6]{vershynin2018high} }\\
    & \leq \frac{2}{d^{4\alpha}} +  \mathbb{P}\left(\|W_Q\|^2 \leq 2 c^* \frac{\normsquare{Q}}{n} \log^2 d\right),
\end{align*}


Writing a better bound than in the above display (using joint probability instead of conditional probability) we get
\begin{align*}
    1-d^{-\alpha} &\leq \mathbb{P}\left(\|\widetilde W_Q\|^2 \leq c^* \normsquare{2nQ} \log^4 d\right)\\
    &\leq \mathbb{P}\left(\widetilde n < n\right) + \mathbb{P}\left(\|\widetilde W_Q\|^2 \leq c^* \normsquare{2nQ} \log^4 d  , \quad \widetilde n \geq n\right).
\end{align*}
Here
\begin{align*}
     \mathbb{P}\left(\|\widetilde W_Q\|^2 \leq c^* \normsquare{2nQ} \log^4 d  , \quad \widetilde n \geq n\right)
     &=
     \sum_{k=n}^\infty \mathbb{P}\left(\|\widetilde W_Q\|^2 \leq c^* \normsquare{2nQ} \log^4 d ~\Big|~ \widetilde n =k \right)
     \mathbb{P}( \widetilde n =k).
\end{align*}
Thus, to grant the inequality 
$$
\mathbb{P}\left(\|\widetilde W_Q\|^2 \leq c^* \normsquare{2nQ} \log^4 d  , \quad \widetilde n \geq n\right)
\le 
\mathbb{P}\left(\|\widetilde W_Q\|^2 \leq c^* \normsquare{2nQ} \log^4 d ~\Big|~ \widetilde n =n \right)
$$
it suffices to show  that, for all $k>n$,
\begin{align*}
    \mathbb{P}\left(\|\widetilde W_Q\|^2 \leq c^* \normsquare{2nQ} \log^4 d ~\Big|~ \widetilde n =k \right)
     &\le 
     \mathbb{P}\left(\|\widetilde W_Q\|^2 \leq c^* \normsquare{2nQ} \log^4 d ~\Big|~ \widetilde n =n \right).
\end{align*}
Is it true?

\end{proof}


%%%%%%%%%%%%%%%%%%%%
% Algorithm 1
%%%%%%%%%%%%%%%%%%%%


\begin{algorithm}[H]\label{alg:Alg}
\SetAlgoLined
\textbf{Input:} $\alpha>0$, integers $n, d$, matrices $\Yone, \Ytwo$.\\

\textbf{Output:} Estimator $\widehat P$ of $P$ %s.t. $\mathbb P\left(\|\widehat P - P\|_1 \geq C\sqrt{\frac{K(d_1+d_2)}{n}} \log^3(d_1+d_2)\right) \leq 1-Cd^{-\alpha}$.

\vspace{3mm}

\textbf{If } $n < \barc \alpha d \log d$, \textbf{then return} $\frac{1}{2}(\Yone + \Ytwo)$.

\vspace{2mm}

\textbf{Else:} $T\leftarrow \lfloor \log_2 d -1\rfloor$

\vspace{2mm}

\hspace{5mm} {\textbf{For} $t,t'=0, \dots, T+1$:}
\begin{enumerate}
    \item $k \leftarrow (t,t')$; $\tau_k \leftarrow \sqrt{c^* \frac{\log^2 d}{n}2^{1-t\land t'}}$; and define $\Mk$ as in~\eqref{eq:def_Mk}
    \item \textbf{If} $\normsquare{\Mk} < 2\barc \alpha \frac{\log d}{n}$ \textbf{then} $\hatPk \leftarrow \Mk$.
    \item \textbf{Else} $\hatPk \leftarrow \arg \min_{A \in \R^{d_1\times d_2}} \|\Mk - A\|_F^2 + \tau_k \|A\|_*$
    \item $\widehat P \leftarrow \sum_{k \in \{0,\dots, T\!+\!1\}^2} \hatPk$
    \item $\widehat P_+ \leftarrow \big(\widehat P_{ij} \lor 0\big)_{ij} $
\end{enumerate}
\textbf{Return} $\frac{\widehat P_+}{\|\widehat P_+\|_1}$.
\caption{Estimation procedure}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Over $\mathcal{C} := \bigcup_{i,j \in \mathcal{B}} C_{ij}$, we have by definition of $\mathcal{E}$ that $\int_{\mathcal{C}} f \leq \frac{C}{\sqrt{n}}$, so that with probability $1 - \exp\left(-c\sqrt{n}\right)$, we have that 
\begin{align*}
    S := \sum_{\substack{j\in E_1 \\ j \notin \{0,\dots,m_1-1\} }} \sum_{\substack{j'\in E_2 \\ j' \notin \{0,\dots,m_2-1\} }} N_{j,j'} + N'_{j,j'} \leq C \sqrt{n}.
\end{align*}
To see this, note that
\begin{align*}
    S = \sum_{i=n/2+1}^n \mathbb 1\Bigg\{X_i \in \! \bigcup_{\substack{j\in E_1 \\ j \notin \{0,\dots,m_1-1\} }} \bigcup_{\substack{j'\in E_2 \\ j' \notin \{0,\dots,m_2-1\} }} C_{j,j'}\Bigg\} ~\sim~ \operatorname{Bin}(n/2,p),
\end{align*}
where $p \leq \frac{C}{\sqrt{n}}$. 


Therefore, by Bernstein's inequality, we get 
\begin{align*}
    \mathbb P\left(S > C \sqrt{n}\right) &\leq \exp\left(-c \bigg( t \land \frac{t^2}{\sqrt{n}}\bigg)\right) \quad \text{ where } t = C \sqrt{n} - np\\
    & \leq \exp\left(-c \sqrt{n}\right).
\end{align*}
We recall that over $\mathcal{C}$, the estimator can be written as $\widehat f = \frac{1}{h_1h_2} \sum_{(j,j') \notin \mathcal{E}'} \frac{2}{n} (N_{j,j'} + N'_{j,j'})\mathbb 1_{C_{j,j'}}$.
Therefore, with probability $1-\exp\left(-c\sqrt{n}\right)$, we obtain 
\begin{align*}
    \int_{\mathcal{C}} |\widehat f - f| \leq \int_{\mathcal{C}} |\widehat f | +\int_{\mathcal{C}} |f| \leq  \frac{C\sqrt{n}}{n} + \frac{C}{\sqrt{n}} \leq \frac{C}{\sqrt{n}}.
\end{align*}
%\ju{Vérifier, pb sur $\mathcal{C}?$ il faut peut être mettre seulement le max de vraisemblance sur $\mathcal{C}$, plus simple à analyser.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

is 
    Note that the choice of $E_j = \big\{-\big\lceil 1/h_j\big\rceil,\dots, \big\lceil 1/h_j\big\rceil\big\}$ for $j \in \{1,2\}$ is not the only one having these properties, and simply a matter of notation convenience. {\color{red} Sasha: why it is so convenient? Quelle est la logique?} For example, it would have been possible to define $E_1$ and $E_2$ as follows:
    \begin{align*}
        E_j' = \big\{-\big\lceil \widehat r_j/h_j\big\rceil,\dots, \big\lceil (1-\widehat r_j)/h_j \big\rceil\big\}, \qquad j\in \{1,2\}
    \end{align*}
    for the associated grid $(C_{jj'})_{j\in E_1',j'\in E_2'}$ to be the smallest grid containing $[0,1]^2$.
    {\color{red} Sasha: quelle est l'inconvenience de cette définition?}


    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


$\log^{-\frac{3}{2} \frac{2\beta + 1}{\beta}}(n)$







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Moreover, we can only have $K' \neq K$ if $\big(\frac{K}{n}\big)^{\frac{\beta}{2\beta+1}} \log^{3/2}(n) > n^{-\frac{\beta}{2\beta+2}}$, that is 
\begin{align*}
    K > \frac{n^{\frac{1}{2\beta+2}} }{ \left(\log(n)\right)^{\frac{3}{2} \frac{2\beta+1}{\beta}}}.
\end{align*}

{\color{magenta}
In this case, $K' = n^{\frac{1}{2\beta+2}} \leq K \left(\log(n)\right)^{\frac{3}{2} \frac{2\beta+1}{\beta}} \leq K \log^{9/2}(n) \leq n \big[(8L)^{-1}\wedge (8L)^{-3/2} \wedge 1 \big]$ by assumption.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{2mm}

{\color{magenta} If $\beta \leq -\frac{2 \log((8L)^{-1} \land 1 )}{\log(n)}$: 
\vspace{2mm}

\hspace{5mm} \textbf{Return} $\mathbbm 1_{[0,1]^2}$.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Figure~\ref{fig:simul_discrete} shows that the behavior of the histogram estimator exhibits a phase transition around ${\color{blue} d = 800}$. 
This is coherent with its estimation risk in $\ell_1$ loss given by $\sqrt{\frac{2}{\pi}\frac{d_1 d_2}{n}} \land 2 = \frac{d}{\sqrt{n}}\land 2$ (see~\cite{han2015minimax}, where the phase transition arises around $d = \sqrt{2\pi n} = 793$ {\color{magenta} (Sasha: why? I don't see any phase transition at $d\asymp n$.)}. 
In contrast, our estimator does not exhibit this phase transition around $d \asymp n$ since its estimation risk is given by $\sqrt{\frac{Kd}{n}} \land 1 = \sqrt{\frac{d}{n}} \land 1$. {\color{magenta} (Sasha: I don't see any phase transition in the plot and moreover the value $d=n= 10^5$ is not given by the plot.)}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{proof}[Proof of Theorem~\ref{th:lower bound for density estimation}] 
Without loss of generality, we prove the lower bound over the class $\mathcal{G}_{K+1,\beta}$ rather than over $\mathcal{G}_{K,\beta}$.
%For $x,y \in [0,1]$, we define $f_0(x,y) = \frac{b}{K} \mathbb 1_{x\leq K/b}$.  
We define $f_0 = \mathbbm{1}_{[0,1]^2}$ and set $K' = \lfloor n^{1/(2\beta+2)} \rfloor \land K$, $H=\lceil (n/K')^{1/(2\beta+1)} \rceil$, $h_x=1/K'$, $h_y=1/H$.
%For some small enough constant $c' \in \big(0,(L\lor1)^{-1}\big)$ depending only on $L$, we define
%$$h= c' \left(\frac{K'}{n}\right)^{1/(2\beta+1)}, \quad k = \frac{1}{K'}, \quad \text{ and } \quad H = \frac{1}{h}.$$
%Note that we have $h\leq 1$ since $c'\in (0,1)$, and $k \geq h$ if $c \leq 1$. 
Let $\varphi:\mathbb{R}\to [0,1]$ be a {\color{red} non identically zero} infinitely many times differentiable function with support $(-1/2,1/2)$ satisfying the $\beta$-H\"older condition with H\"older constant $1/2$ (see (2.34) in \cite{tsybakov2009introduction} for an example of such function).
%and define the functions 
%\begin{align*}
%    U(x) = \left(\frac{1}{3} - \Big(|x| - \frac{1}{6}\Big)_{+}\right)_{+}^\beta = \begin{cases} (x+\frac{1}{2})^\beta & \text{ if } x \in [-\frac{1}{2},-\frac{1}{6}]\\ \frac{1}{3^\beta} &\text{ if } x \in [-\frac{1}{6}, \frac{1}{6}]\\
%    (\frac{1}{2}-x)^\beta &\text{ if } x \in [\frac{1}{6},\frac{1}{2}]\\
%    0 & \text{ otherwise.}\end{cases} \quad\text{ and } \quad V(y) = \Big(\frac{1}{2}-|y|\Big)_+^\beta.
%\end{align*}
For $i,j \in \mathbb Z$, set $V_{i,h_x}(x) = \varphi\big(\frac{x-x_i^-}{h_x/2}\big)-\varphi\big(\frac{x-x_i^+}{h_x/2}\big)$, where
$x_i^- = \big(i-\frac{3}{4}\big)h_x$ and $x_i^+ = \big(i-\frac{1}{4}\big)h_x$  
and analogously $V_{j,h_y}(y) = \varphi\big(\frac{y-y_j^-}{h_y/2}\big)-\varphi\big(\frac{y-y_j^+}{h_y/2}\big)$, where
$y_j^- = \big(j-\frac{3}{4}\big)h_y$ and $y_j^+ = \big(j-\frac{1}{4}\big)h_y$. The supports of functions $\varphi\big(\frac{\cdot-x_i^-}{h_x/2}\big)$ and $\varphi\big(\frac{\cdot-x_i^+}{h_x/2}\big)$ are disjoint and each of these functions is $\beta$-H\"older with H\"older constant $(1/2)(h_x/2)^{-\beta}$. Hence, $V_{i,h_x}(\cdot)$ is $\beta$-H\"older with H\"older constant $(h_x/2)^{-\beta}$. Note also that the functions $V_{i,h_x}$ integrate to 0 and 
have disjoint supports in $[0,1]$ for different $i$'s. The same is true for the functions $V_{j,h_y}$. 
\ju{We also set $U_i(x) := \varphi\big(\frac{x-x_i}{h_x/2}\big)$ where $x_i = \big(i-\frac{1}{2}\big) h_x$}

%$U_{i} (x) = \frac{Lh}{K} \left[\left(1-\frac{|x-x_i-1/2|}{2h}\right)_+ + \left(1-\frac{|x-x_i+1/2|}{2h}\right)_+\right]$ as well as $V_{j} (y) = \frac{Lh}{K} \left[\left(1-\frac{|y-y_j-1/2|}{2h}\right)_+ - \left(1-\frac{|y-y_j+1/2|}{2h}\right)_+\right]$. 
%perturbation $\phi_+(x,y) = \left(1-|x|\right)_+\left(1-|y|\right)_+$ and 
%$\phi_h(x,y) = c\frac{Lh}{K}\phi_+\left(\frac{1}{h}\left[(x,y)-(\frac{1}{2},\frac{1}{2})\right]\right) - \frac{Lh}{K}\phi_+\left(\frac{1}{h}\left[(x,y)+(\frac{1}{2},\frac{1}{2})\right]\right)$ \ju{check}.
Set $c_*=1/4\wedge 1/(2L)$.  
%For any $(i,j) \in \mathbb Z^2$, we define $C_{ij} = \big[x_i\pm\frac{k}{2}\big]\times \big[y_j\pm\frac{h}{2}\big]$.
%We perturb $f_0$ on each cell $C_{i,j}$ as follows. %
For $\omega = (\omega_{ij})$, where $\omega_{ij}\in \{0,1\}$ for all $i,j$, we define the functions $f_\omega$ as follows:
\begin{align*}%\label{eq:def_prior}
    f_\omega(x,y) = f_0(x,y) + c_* L h_y^\beta \sum_{i=1}^{K'} \sum_{j=1}^{H} \omega_{ij} V_{i,h_x}(x) V_{j,h_y}(y). 
\end{align*}
\ju{We can replace this definition with the following one:
\begin{align*}
    f_\omega(x,y) &= \sum_{i=1}^{K'} U_i(x) \bigg(C_0 + \sum_{j=1}^{H}  \omega_{ij} c_* L h_y^\beta V_{j,h_y}(y)\bigg),
\end{align*}
where $C_0$ is such that $C_0 \int_{0}^1\sum_{i=1}^{K'} U_i(x) = 1$, i.e. $C_0 K' \frac{h_x}{2} \int_{0}^1 \varphi = 1$. 
It suffices to take $C_0 = \frac{2}{\int_{0}^1 \varphi}$. 
Defining $f_0(x,y) = \sum_{j=1}^{K'} U_i(x)$, we obtain
\begin{align*}
    f_\omega(x,y) = f_0(x,y) + \sum_{i=1}^{K'} U_i(x)\Big(\sum_{j=1}^{H} c_*Lh_y^\beta \omega_{ij} V_{j,h_y}(y)\Big)
\end{align*}
which is analogous to the expression we have below.
}
{\color{red} Moreover, we can rewrite $f_\omega$ as a mixture of separable densities that are products of Hölder-smooth $1$-dimensional densities
\begin{align*}
    f_\omega(x,y) = \frac{1}{K'} \sum_{k=1}^{K'} K' C_0 U_i(x)\bigg(1 + \frac{1}{C_0}\sum_{j=1}^{H}  \omega_{ij} c_* L h_y^\beta V_{j,h_y}(y)\bigg).
\end{align*}
The functions $K'C_0 U_i$ are non-negative and are therefore densities by definition of $C_0$. 
They are also Hölder-smooth over their support by definition of $U_i$. 
Moreover, it suffices to take $c_*$ small enough to guarantee that $1 + \frac{1}{C_0}\sum_{j=1}^{H}  \omega_{ij} c_* L h_y^\beta V_{j,h_y}$ is non-negative, ensuring that $1 + \frac{1}{C_0}\sum_{j=1}^{H}  \omega_{ij} c_* L h_y^\beta V_{j,h_y}$ is a $\beta$-Hölder density over $[0,1]$ since the $V_{j,h_y}$'s have a zero integral and are $\beta$-Hölder.
}


First, we check that each $f_\omega$ belongs to $\mathcal{G}_{K'+1,{\beta}} \subseteq \mathcal{G}_{K+1,{\beta}}$.  
\begin{itemize}
    \item We have $\int_{[0,1]^2} f_\omega = 1$ by construction.
    \vspace{-2mm}
    \item 
   We have $f_\omega(x,y) \geq {1}/{2}$ for all $(x,y)\in [0,1]^2$ since $c_*\le (2L)^{-1}$, $h_y\le 1$, and the functions $(x,y) \mapsto V_{i,h_x}(x) V_{j,h_y}(y)$ have disjoint supports and take values in $[-1,1]$.
%
    \vspace{-2mm}
    \item We now check the H\"older condition. 
    \ju{In the rest of the proof, simply replace $V_{i,h_x}(x)$ with $U_i(x)$ everywhere}
%    In the definition of $f_\omega$,
   As the supports $C_{ij}$ of functions $(x,y) \mapsto V_{i,h_x}(x) V_{j,h_y}(y)$ are disjoint and $f_\omega = 1$ at the boundary of each cell $C_{ij}$, it suffices to show that $f_\omega$ is $\beta$-H\"older with H\"older constant $L/2$ on each cell $C_{ij}$ to obtain that $f_\omega$ is $\beta$-H\"older with H\"older constant $L$ on $[0,1]^2$. Fix any two points $z,z' \in [0,1]^2$, belonging to the same cell $C_{ij}$. Then, writing $z = (x,y)$, $z' = (x',y')$ and recalling that $V_{i,h_x}, V_{j,h_y}$ take values in $[-1,1]$ and are $\beta$-H\"older with H\"older constants $(h_x/2)^{-\beta}$, $(h_y/2)^{-\beta}$ we obtain: 
    \begin{align*}
        \big|f_\omega(z) - f_\omega(z')\big| &= c_*Lh_y^\beta\,\Big|V_{i,h_x}(x) V_{j,h_y}(y) - V_{i,h_x}(x') V_{j,h_y}(y')\Big|\\
        &\leq c_*Lh_y^\beta \Big|V_{i,h_x}(x)-V_{i,h_x}(x')\Big| + c_*Lh_y^\beta \Big|V_{j,h_y}(y)- V_{j,h_y}(y')\Big| 
         \\
        & \leq c_* Lh_y^\beta \left[ \left(\frac{|x-x'|}{h_x/2}\right)^\beta+\left(\frac{|y-y'|}{h_y/2}\right)^\beta \right]
          \\
        &\leq \frac{L}{2} \|z-z'\|^\beta_{\infty},
    \end{align*}
    where we have used the facts that $h_y\leq h_x$ and $c_*\le 1/4$.
    \vspace{-2mm}
    \item Function $f_\omega$ belongs to $\mathcal{F}_{K'+1} \subseteq \mathcal{F}_{K+1}$ since it admits a separable representation 
\begin{align*}
    f_\omega(x,y) = f_0(x,y) + \sum_{i=1}^{K'} U_i(x)\Big(\sum_{j=1}^{H} c_*Lh_y^\beta \omega_{ij} V_{j,h_y}(y)\Big), \quad U_i(x): = V_{i,h_x}(x).
\end{align*}
\end{itemize}

Thus, $\mathcal{G}':=\{f_\omega: \omega\in \{0,1\}^{K'\times H}\}$ is a subset of $\mathcal{G}_{K'+1,{\beta}}$, and it  suffices to prove the lower bound with the required rate on this subset. We first prove the lower bound in expectation~\eqref{eq:th:LBdiscr3}. We use the version of Assouad's lemma
given in \cite[Theorem 2.12(\it{iv})]{tsybakov2009introduction}.
For any $\omega, \omega' \in \{0,1\}^{K' \times H}$ that only differ in one entry, that is, for exactly one $(i_0,j_0)$, we have $\omega_{i_0,j_0}\neq \omega'_{i_0,j_0}$ and $\omega_{i,j}= \omega'_{i,j}$ for all other $i,j$, the $\chi^2$-divergence between the densities $f_\omega$ and $f_{\omega'}$ is bounded as follows:
\begin{align*}    \chi^2\left(f_{\omega'}, f_{\omega}\right) &= \int \frac{(c_* L h_y^\beta V_{i_0,h_x}(x) V_{j_0,h_y}(y))^2}{f_\omega(x,y)} \leq \int_{C_{i_0,j_0}} 2(c_*Lh_y^\beta)^2 {\color{red} \leq } 2(c_*Lh_y^\beta)^2 h_x h_y \leq \frac{ \widetilde{c}}{n},
\end{align*}
where $\widetilde{c}>0$ depends only on $L, \beta$. Using  Lemma 2.7 in ~\cite{tsybakov2009introduction} we obtain that  the $\chi^2$-divergence between the corresponding product densities satisfies
\begin{align*}
    \chi^2\left(f_{\omega'}^{\otimes n}, f_{\omega}^{\otimes n}\right) = \left(1+\chi^2\left(f_{\omega'}, f_{\omega}\right)\right)^n-1 \leq e^{\widetilde{c}}-1.
\end{align*}
Also, note that for all $i,j$ we have 
\begin{align*}
     \|V_{i,h_x}(x) V_{j,h_y}\|_{L_1}
     & 
     = 4 \int \varphi\Big(\frac{x}{h_x/2}\Big)  dx \int \varphi\Big(\frac{y}{h_y/2}\Big)  dy
     = 16 h_x h_y \Big(\int \varphi(x)  dx\Big)^2.
\end{align*}
Therefore, applying \cite[Theorem 2.12(\it{iv})]{tsybakov2009introduction} and arguing as in  \cite[Example 2.2]{tsybakov2009introduction} we obtain 
\begin{align}\label{eq-lb-in-exp}
 \inf_{\widehat f} \sup_{f_\omega\in \mathcal{G}'} \mathbb E  
    \|\widehat f-f_\omega\|_{L_1}
     &\geq \frac{K'H}{8} (c_*Lh_y^\beta) c'' h_x h_y  = \frac{c_*c''}{8} L h_y^\beta  \geq c \Big((K/n)^{\beta/(2\beta+1)} \land n^{-{\beta}/{(2\beta+2)}}\Big),   
\end{align} 
    where $c''=16\big(\int \varphi(x)  dx\big)^2 \exp(1-e^{\widetilde{c}})$ and  $c>0$ is a constant depending only on $L$ and $\beta$.    This implies the lower bound in expectation~\eqref{eq:th:LBdiscr3}. 
    \vspace{1mm}
    
    To obtain the lower bound in probability~\eqref{eq1:th:lower bound for density estimation} we apply Lemma~\ref{lem:reduction of lower bound}
    with $\mathcal{P} = \mathcal{P}_0 = \mathcal{G}'$,  $v(f,g) = \|f-g\|_{L^1}$ for any $ f,g \in \mathcal{G}'$, and 
    $U = \mathbbm 1_{[0,1]^2} \in \mathcal{G}'$.  
    Note that there exists a constant $C>0$ such that for any $f \in \mathcal{G}'$ we have
    $
        v(U,f) \leq s,
    $ 
    where $s =  C \big(\left(K/n\right)^{\beta/(2\beta+1)} \land n^{-{\beta}/{(2\beta+2)}}\big)$. 
    Therefore, taking into account the bound in expectation \eqref{eq-lb-in-exp} we can apply Lemma~\ref{lem:reduction of lower bound} with  a small enough constant $a>0$ to get~\eqref{eq1:th:lower bound for density estimation}.
\end{proof}

==> contents_low_rank/Problem_statement.tex <==
\section{Discrete distributions}


In this section, we consider the setting with discrete distributions, which provides a base for studying continuous distributions in Section~\ref{sec:densities}.


%\subsection{Problem Statement}
\input{contents_low_rank/Pb_statement_matrix}

\begin{definition}\label{Def_minimax_risk}
Given $\delta>0$, the minimax rate of estimation  of $P \in \mathcal{D}_K$, given $(X_1,\dots, X_n)$, is defined as 
\begin{equation}\label{def:minimax_rate}
    \psi_\delta^*(n,\mathcal{D}_K) = \inf \Bigg\{\psi>0 ~\Big|~ \inf_{\hat P}\, \sup_{P \in \mathcal{D}_K} \mathbb{P}\Big( \big\|\widehat{P}(X_1,\dots,X_n)-P\big\|_1 > \psi\Big) \leq \delta\Bigg\},
\end{equation}
where the infimum is taken over all estimators $\widehat P$ that are allowed to depend on $\delta$.
\end{definition}
Next, we derive the rate $\psi_\delta^*(n,\mathcal{D}_K)$ (up to multiplicative constants and logarithmic factors) and propose a computationally efficient estimator $\widehat P$ achieving this rate. 


==> contents_low_rank/References_for_tensors.tex <==
\section{Papers to read for tensors decomposition}

\cite{yuan2016tensor}, \cite{zhang2019cross}, \cite{xia2021statistically}
\\
For an excellent introduction to tensor SVD: ~ https://anruzhang.github.io/slides/2019-tensor-svd.pdf \\

Paper Vandermeulen https://arxiv.org/pdf/2204.00930.pdf\\

\cite{dudeja2022statistical}\\

\cite{luo2019bernstein}\\

\cite{raskutti2019convex}

Crash course on tensors : https://tensorvoices.de/

\cite{zhang2018tensor}: ``Tensor SVD: statistical and computational limits''

\cite{tomioka2014spectral}
Spectral norm for random tensors suzuki: https://arxiv.org/pdf/1407.1870.pdf:


Review on tensor decompositions: \cite{kolda2009tensor}

==> contents_low_rank/Results.tex <==
%\subsection{Estimation procedure}\label{sec:results}

%\ju{Attention on a besoin de $\widetilde n_1$ et $\widetilde n_2$ car conditionnellement à $Y_1$ il faut que $Y_2$ soit poisson}

%In this work, we restrict ourselves to the matrix case and therefore consider the case $M=2$. 

\subsection{Estimator}\label{subsec:discrete_Estimator}

Our algorithm is inspired by the literature on the low-rank matrix estimation and is based on the nuclear norm penalization. 
Note that our setting  requires several non-trivial modifications to the basic PCA technique. We start by describing our algorithm. In the next section we will provide an intuition on our construction and the main ideas behind the proofs of the upper bounds on the risk of our estimator.
\vspace{2mm}

Without loss of generality, assume that the total number of observations is even and equal to $2n$.
We use sample splitting to define $H^{(1)} \sim \text{Hist}(X_1,\dots, X_n)$ and $H^{(2)} = \text{Hist}(X_{n+1}, \dots, X_{2n})$ as the histograms of $(X_1,\dots, X_n)$ and $(X_{n+1},\dots, X_{2n})$ respectively. 
We also consider the renormalized observations $Y^{(1)} = \frac{2}{n} H^{(1)}$ and $Y^{(2)} = \frac{2}{n} H^{(2)}$.
In what follows, it will be useful to express the matrices $P$, $Y^{(1)}$ and $Y^{(2)}$ as the family of their columns and of their rows:
\begin{align*}
    P = \Big[C_1,\dots, C_{d_2}\Big] = \left[\begin{array}{ccc}
     \!\!L_1\!\! \\
     \!\!\vdots\!\!\\
     \!\!L_{d_1}\!\!
\end{array}\right] ~~ \text{ and } ~~ \Yl = \Big[\hatCl_1,\dots, \hatCl_{d_2}\Big] = \left[\begin{array}{ccc}
     \!\!\hatLl_1\!\! \\
     \!\!\vdots\!\!\\
     \!\!\hatLl_{d_1}\!\!
\end{array}\right], \text{ for } \ell=1,2.
\end{align*}

%\textbf{\underline{Idea (heuristic!)}}: The first half of the sample, represented by $\Yone$, is used to select rows and columns that have `similar' $\ell_1$ norm. More precisely, for each $t=0,\dots, O(\log(d))$, we select from $\Yone$ the indices of the rows and columns whose $\ell_1$ norms is bracketed between $\left[\frac{1}{2^{T\!+\!1}}, \frac{1}{2^t}\right]$. On these rows and columns, the noise $W$ will be roughly homogeneous by Olga's Lemma.\\

%After having selected the indices, we extract the submatrix $\Mk$ of $\Ytwo$ whose entries are those of $\Ytwo$ on each selected index and $0$ everywhere else. We perform an SVD of this matrix. We repeat for all $t=0,\dots, T$ where $T = \lfloor C_T \log d \rfloor$ and $C_T$ is a large enough absolute constant. We finally combine all of these estimators to get the final one. \\

%Let $T = \lfloor C_T \log d \rfloor$ where $C_T$ is a large enough absolute constant. 
We set $d = d_1 \lor d_2$ and $T = \lfloor \log_2 d \rfloor -1$.
For any $t \in \{0,\dots, T\}$, define 
\begin{align}
    I_t &= \bigg\{i \in [d_1]: \big\|\hatLone_i\big\|_1 \in \left(\frac{1}{2^{t+1}}, \frac{1}{2^t}\right]\bigg\}, \label{def_I}\\
    J_t &= \bigg\{j \in [d_2]: \big\|\hatCone_j\big\|_1 \in \left(\frac{1}{2^{t+1}}, \frac{1}{2^t}\right]\bigg\}, \label{def_J}
\end{align}

Moreover, we define 
\begin{align}
    I_{T+1} &= \bigg\{i \in [d_1]: \big\|\hatLone_i\big\|_1 \leq \frac{1}{2^{T+1}}\bigg\}, \label{def_I_infty}\\
    J_{T+1} &= \bigg\{j \in [d_2]: \big\|\hatCone_j\big\|_1 \leq \frac{1}{2^{T+1}}\bigg\}, \label{def_J_infty}
\end{align}

For any $k = (t, t') \in \{0,\dots, T\!+\!1\}^2$ we define 
\begin{align}
    &U_k = I_t \times J_{t'}, \label{def_U}\\
    &\Mk = \left(\Ytwo_{ij}\,\mathbb{1}\left\{(i,j) \in U_k\right\}\right)_{i,j},\label{eq:def_Mk}\\
    &\Pk = \left(P_{ij}\,\mathbb{1}\left\{(i,j) \in U_k\right\}\right)_{i,j}, \label{eq:def_Pk}\\
    &W_k = \Mk - \Pk. \label{eq:def_Wk}
\end{align}

In the following algorithm, we denote by $\barc$ the absolute constant from Lemma~\ref{lem:concent_poisson} and by $c^*$ the constant from Proposition~\ref{prop:bound_Mult_matrix}.\\

\begin{algorithm}[H]\label{alg:Alg}
\SetAlgoLined
\textbf{Input:} $n, \alpha, d, \Yone, \Ytwo$.\\

\textbf{Output:} An estimate $\widehat P$ of $P$ %s.t. $\mathbb P\left(\|\widehat P - P\|_1 \geq C\sqrt{\frac{K(d_1+d_2)}{n}} \log^3(d_1+d_2)\right) \leq 1-Cd^{-\alpha}$.

\vspace{3mm}

\textbf{If } $n < \barc \alpha d \log d$, \textbf{then return} $\frac{1}{2}(\Yone + \Ytwo)$.

\vspace{2mm}

\textbf{Else:} $T\leftarrow \lfloor \log_2 d -1\rfloor$

\vspace{2mm}

\hspace{5mm} {\textbf{For} $t,t'=0, \dots, T+1$:}
\begin{enumerate}
    \item $k \leftarrow (t,t')$; $\tau_k \leftarrow \sqrt{c^* \frac{\log^2 d}{n}2^{1-t\land t'}}$; and define $\Mk$ as in~\eqref{eq:def_Mk}
    \item \textbf{If} $\normsquare{\Mk} < 2\barc \alpha \frac{\log d}{n}$ \textbf{then} $\hatPk \leftarrow \Mk$.
    \item \textbf{Else} $\hatPk \leftarrow \arg \min_{A \in \R^{d_1\times d_2}} \|\Mk - A\|_F^2 + \tau_k \|A\|_*$
    \item $\widehat P \leftarrow \sum_{k \in \{0,\dots, T\!+\!1\}^2} \hatPk$
    \item $\widehat P_+ \leftarrow \big(\widehat P_{ij} \lor 0\big)_{ij} $
\end{enumerate}
\textbf{Return} $\frac{\widehat P_+}{\|\widehat P_+\|_1}$.
\caption{Estimation procedure}
\end{algorithm}

\subsection{Intuition of the estimator 
 construction}

To estimate a low-rank matrix from noisy observations, the classical approach is to use SVD-based methods. 
The main drawback of such methods is that they can be sub-optimal under a non-isotropic noise, which is precisely the case for the multinomial noise in our setting: Any coordinate $Y_{ij}$ of a random histogram $Y\sim \mathcal{M}(P,n)$ is distributed as $Y_{ij} \sim \operatorname{Bin}(n,P_{ij})$, and has a variance of $nP_{ij}(1-P_{ij})$, which varies across the indices $(i,j)$. 
To overcome this difficulty, our algorithm splits the multinomial matrix into a logarithmic number of sub-matrices, on which the multinomial noise can be more carefully controlled. Then, each sub-matrix is denoised separately using a soft-thresholding estimator. 
\vspace{1mm}

To understand why we split the multinomial matrix as in equations~\eqref{def_I}-\eqref{def_J_infty}, assume that $H\sim \mathcal{M}(P,n)$ and for any two subsets $I \subset [d_1]$ and $J \subset [d_2]$, define the extractions according to $I$ and $J$ as $$H_{IJ} = (H_{ij})_{(i,j)\in I\times J}, \quad P_{IJ} = (P_{ij})_{(i,j)\in I\times J}, \quad \text{ and } 
 \quad W_{IJ} = \frac{H_{IJ}}{n} - P_{IJ}.$$ 
Then, by Proposition~\ref{prop:bound_Mult_matrix} (ignoring logarithmic factors) the operator norm of $W_{IJ}$ can be controlled as a function of the column-wise and row-wise sum of the entries of $P_{IJ}$:
\begin{align*}
    \|W_{IJ}\|_{op}^2 &\lesssim \frac{1}{n}\normsquare{P_{IJ}} = \frac{1}{n} \max\Big(\max_{i \in I} \sum_{j\in J} P_{ij},~ \max_{j \in J} \sum_{i\in I} P_{ij}\Big)\\
    & \leq \frac{1}{n} \max\Big(\max_{i \in I} p_i,~ \max_{j \in J} q_j\Big),
\end{align*}
where $p_i = \sum\limits_{j=1}^{d_2} P_{ij}$ and $q_j = \sum\limits_{i=1}^{d_1} P_{ij}$ are the marginal mass functions. 
The above expression suggests taking the subsets $I, J$ such that 
\begin{align*}
    \forall i \in I: ~ p_i \asymp \max_{i' \in I} p_{i'}
    \quad\quad \text{ and } \quad \quad
    \forall j \in J: ~ q_j \asymp \max_{j' \in J} q_{j'},
\end{align*}
that is, to split the multinomial matrix according to similar values of the $p_i$'s and $q_j$'s, in order for the multinomial noise to be close to isotropic over the considered sub-matrix.\\

Of course, the values $(p_1,\dots, p_{d_1})$ and $(q_1,\dots, q_{d_2})$ are not known to us, which is why we use sample splitting to obtain sufficiently precise estimators $(\hat p_1,\dots, \hat p_{d_1})$ and $(\hat q_1,\dots, \hat q_{d_2})$ from the first half of the data.
%(in our algorithm, we use sample splitting to estimate the oracle with the first half of the data, and then, we apply the following procedure with the second half).
In this paragraph, we assume that an oracle gives us $(p_1,\dots, p_{d_1})$ and $(q_1,\dots, q_{d_2})$ to simplify the discussion below. 
Fix $d = d_1 \lor d_2$, and for any $t \in \{0,\dots, \lfloor\log_2(d)-1\rfloor\}$, define the following index sets
$$ \widetilde I_t = \left\{i: p_i \in \left(\frac{1}{2^t}, \frac{1}{2^{t+1}}\right]\right\}, \quad \widetilde J_{t} = \left\{j: q_j \in \left(\frac{1}{2^{t}}, \frac{1}{2^{t+1}}\right]\right\},$$
and, for $T = \lfloor\log_2(d)\rfloor$, let 
$$\text{$\widetilde I_T = [d_1] \setminus \bigcup\limits_{t' < T} I_{t'}$ and $\widetilde J_T = [d_2] \setminus \bigcup\limits_{t' < T} J_{t'}$.}$$
Fix $t,t' \in \{0,\dots, T\}$ and define $k = (t,t')$. %\ol{(1) Should we replace everywhere in what follows $I_t, J_t$ by $\widetilde{I_t}, \widetilde{J_t}$?? (2) add explanation why do we need cut the set of indices in such "uniform" sets.} \ju{(1) Oui (2) To get optimal rate, we need to split our matrix into submatrices with similar ranges of values, in order to get a more isotropic noise} 
On each grid's cell,  we further define $\widetilde M_k = \frac{1}{n} Y_{\widetilde I_t \times \widetilde J_{t'}}$, and $P_k = P_{\widetilde I_t \times \widetilde J_{t'}}$. 
Then $\rk (P_k) \leq K$ and $\normsquare{P_k} \leq \frac{1}{2^{t\land t'}}$ by construction. 
To obtain an estimator $\widehat P_k$ of $P_k$, the idea is to perform a soft-thresholding of the SVD of $\widetilde M_k$, provided that the assumptions of Proposition~\ref{prop:bound_Mult_matrix} are met, which controls the multinomial noise. 
We need to treat separately the pathological cases for which the assumptions of Proposition~\ref{prop:bound_Mult_matrix} are not met, and show that they have a negligible contribution to the estimation rate. This strategy allows us  to get  the following risk bound in Frobenius norm (up to a $\log(d)$ factor):
\begin{align*}
    \left\|P_k - \widehat P_k\right\|_F^2 \lesssim \frac{K}{n} \normsquare{\widehat P_k} \lesssim \frac{K}{n \, 2^{t \land t'}}. %\text{ by Proposition~\ref{prop:bound_Mult_matrix}}
\end{align*}
 We can then control the $\ell_1$ norm as
\begin{align*}
    \left\|\Pk - \hatPk\right\|_1 \lesssim \sqrt{\frac{K}{2^{t \land t'} n} |\widetilde I_t|\,|\widetilde J_{t'}|}.
\end{align*}
Summing over all the cells yields an overall estimation rate 
\begin{align*}
    \|\hat P - P\|_1 &\lesssim \sum_{t,t' = 0}^{\log d} \sqrt{\frac{K}{2^{t \land t'} n} |\widetilde I_t|\,|\widetilde J_{t'}|} \leq \sqrt{\sum_{t,t' = 0}^{\log d} \frac{K}{2^{t \land t'} n} |\widetilde I_t||\widetilde J_{t'}| \sum_{t,t'=0}^{\log d} 1} ~\text{ (Cauchy-Schwarz)}\\
    & \leq \sqrt{\sum_{t,t' = 0}^{\log d} \frac{K}{n}\left(\frac{1}{2^{t}} + \frac{1}{2^{t'}} \right) |\widetilde I_t|\,|\widetilde J_{t'}|} \cdot \log d\\
    & \leq \sqrt{\frac{K (d_1+d_2)}{n}} \cdot \log d.
\end{align*}
At the last line, we used the fact that $\sum\limits_{t=0}^{\log d} |\widetilde I_t| = d_1$ and $\sum\limits_{t=0}^{\log d} 2^{-t} |\widetilde I_t| \leq 1$ (by the definition of $\widetilde I_t$), and symmetrically for the family $(\widetilde J_t)_t$.
%In order to prove Theorem~\ref{th:main_th}, we will prove the following two Propositions.

We apply this strategy to prove Proposition \ref{prop:UB} which provides the upper bound on the risk of our estimator. %Here an additional difficulty comes from the fact that we do not have access to the oracle marginal mass functions and we estimate them using the sample splitting.

\subsection{Results for discrete distributions}

\begin{proposition}[Upper bound]\label{prop:UB}
Let $\alpha >0$ and let $\widehat P^*$ be the output of Algorithm~\ref{alg:Alg} with inputs $n, \alpha, d, \Yone, \Ytwo$. Then, there exist two absolute constants $C_0,C_1>0$ such that with probability at least $1-C_0 d^{-\alpha}$
$$ \sup_{P \in \mathcal{D}_K} \|\widehat P^* - P\|_1 \leq C_1 \bigg\{\sqrt{\frac{Kd}{n}} \log^3 \!d \land 1 \bigg\}.$$
\end{proposition}
Next we prove that this convergence rate is minimax optimal up to a logarithmic factor and thus can not be improved by any method:
\begin{proposition}[Lower bound]\label{prop:LB}
Let $\alpha >0$. There exists an absolute constant $c$ such that for any algorithm $\widehat P$, there exists $P \in \mathcal{D}_K$ such that with probability at least $ d^{-\alpha}$, we have 
$$ \|\widehat P - P\|_1 \geq c\bigg\{\sqrt{\frac{Kd}{n}} \land 1\bigg\}.$$
\end{proposition}

Propositions \ref{prop:UB} and \ref{prop:LB} lead to our main result which provide the minimax optimal rate of convergence for the problem of estimating  a discrete distributions under low-rank structure assumption:

\begin{theorem}\label{th:main_th}
Let $\alpha > 0$ and $\delta = O(d^{-\alpha})$. There exists two constants $c,C>0$ depending only on $\alpha$ such that 
$$ c\bigg\{\sqrt{\frac{Kd}{n}} \land 1\bigg\} \leq \psi_\delta^*(n,\mathcal{D}_K) \leq C \bigg\{\sqrt{\frac{Kd}{n}} \log^3 \!d \land 1 \bigg\}.$$ 
\end{theorem}
When $K$ is substantially smaller than $d_1 \land d_2$, the rate of convergence provided by Theorem \ref{th:main_th}, $\sqrt{\frac{Kd}{n}}$ is much faster than the  estimation rate for  $D=d_1d_2$-dimensional discrete distributions in total variation distance, $\sqrt{\frac{D}{n}}$, (see \cite{han2015minimax}).

\section{Continuous distributions}\label{sec:densities}
In this section we extend our algorithm to case of continuous distributions. 
%\ju{Rem: The problem of estimating in $L^1$ if the support is allowed to be $\R^2$ or $\R$ is trivial, therefore we consider $[0,1]^2$. Ref + développer + minimax} \ol{We should provide more details here}
We start by defining our class of densities. 
We let $L>0$ be a constant, and we denote by $\mathcal{L}$ the set of densities supported on a rectangle contained in  $[0,1]^2$, and that are $L$-Lipschitz on its support
\begin{align}
    \mathcal{L} = \left\{f: [0,1]^2 \to \R \,\bigg|\, \exists \, r_1, r_2, R_1, R_2 \in [0,1] \text{ s.t.} \begin{cases} 
    f \text{ is $L$-Lipschitz over } [r_1,R_1]\times [r_2,R_2],\\
    \int_{\Supp(f)} f = 1 \text{ and } f \geq 0.    \end{cases}\!\right\}\label{eq:def_L}
\end{align}

Moreover, for any integer $K\geq 1$, we define $\FK$ as the set of real-valued functions over $[0,1]^2$ that are superpositions of $K$ separable functions:
\begin{align*}
    \FK = \left\{(x,y)\in [0,1]^2 \longmapsto \sum_{k=1}^K u_k(x)v_k(y) \in \R ~\bigg|~ \forall k \in [K], u_k,v_k: [0,1] \longrightarrow \R \right\}.
\end{align*}

We consider the following set of $L$-Lipschitz probability densities
\begin{align}
    \mathcal{G}_K := \mathcal{L} \cap \FK.
\end{align}

We emphasize that any function $f \in \mathcal{G}_K$ is only assumed to be $L$-Lipschitz over a suitable rectangle of the form $[r_1,R_1]\times [r_2,R_2]$, and not necessarily over the whole domain $[0,1]^2$. 
Moreover, the functions $u_k$ and $v_k$ appearing in the decomposition $f(x,y) = 
\sum_{k=1}^K u_k(x) v_k(y)$ can take negative values and need not be Lipschitz-continuous themselves. 
The set $\mathcal{G}_K$ especially contains all of the densities that are $L$-Lipschitz over their support, and that can be expressed as mixtures of separable densities.
\vspace{2mm}

%Our class is defined as the set of densities that are Lipschitz-continuous over a sub-rectangle of $[0,1]^2$, and satisfy a low-rank type assumption, namely, that they can be decomposed as a superposition of separable functions.
It is not restrictive to impose that the support must be contained in $[0,1]^2$. 
Indeed, it has been highlighted in \cite{ibragimov1984more}, \cite{juditsky2004minimax}, \cite{goldenshluger2014adaptive}, \cite{chhor2021goodness} that in the minimax sense, the problem of estimating Lipschitz densities with unbounded support in total variation has a trivial rate of order $1$, regardless of the number of observations. 
The assumption that the support of $f$ is a sub-rectangle of $[0,1]^2$ allows us to handle densities that are not necessarily Lipschitz over the whole domain $[0,1]^2$, and whose support of the form $[r_1,R_1] \times [r_2,R_2]$ may be unknown.
\vspace{2mm}

We now assume that for some unknown $K \in \N\setminus \{0\}$ and some unknown $f \in \mathcal{G}_K$, we observe $n$ iid observations $X_1,\dots, X_n$ distributed with probability density $f$.
Our goal is to estimate $f$. 
%Note that the support of $f$ is not assumed to be known as well. 
For some $\delta>0$, the minimax estimation rate over $\mathcal{G}_K$ with probability $\delta>0$ is defined as
\begin{equation}\label{def:minimax_rate_densities}
    \varphi_\delta^*(n,\mathcal{G}_K) = \inf \Bigg\{\varphi>0 ~\Big|~ \inf_{\hat f}\, \sup_{f \in \mathcal{G}_K} \mathbb{P}\Big( \big\|\widehat{f}(X_1,\dots,X_n)-f\big\|_1 > \varphi\Big) \leq \delta\Bigg\},
\end{equation}

\begin{theorem}\label{th:densities}
For any constant $\alpha>0$ and for $\delta = n^{-\alpha}$, there exist two constants $c,C>0$ depending on $\alpha$ and $L$, and an absolute constant $C'$, such that, if $n \geq C'$ and if $K\leq c n^{1/4}$, then, we have $$c\left(K/n\right)^{1/3}\leq \varphi_\delta^*(n,\mathcal{G}_K) \leq C \left(K/n\right)^{1/3} \log^3 n.$$ 
\end{theorem}


Theorem \ref{th:densities} demonstrates the advantage of including a constraint analogous to the matrix rank in nonparametric density estimation. 
Namely, the classical minimax rate for Lipschitz-continuous density estimation over $[0,1]^2$ in total variation is known to be $n^{-1/4}$,  much slower than our estimation rate $(K/n)^{1/3}$ (see \cite{DevroyeGyofri,daglib}). 
Note that the condition $K \leq C_1 n^{1/4}$ is natural since for $K \gg n^{1/4}$, our rate $(K/n)^{1/3}$ becomes slower than the classical rate $n^{-1/4}$.
\vspace{2mm}

It turns out that the lower bound from Theorem~\ref{th:densities} can even be strengthened, by showing that it can be achieved by densities that have support exactly $[0,1]^2$. 
To prove this, introduce the set of probability densities that are $L$-Lipschitz over $[0,1]^2$.
\begin{align}
    \mathcal{L}_{[0,1]^2} = \left\{f: [0,1]^2 \to \R \text{ s.t. }  \begin{cases} 
    f \text{ is $L$-Lipschitz over } [0,1]^2\\
    \int_{\Supp(f)} f = 1 \text{ and } f \geq 0.    \end{cases}\!\right\}\label{eq:def_L_[0,1]}
\end{align}

Then, we can prove the following proposition. 
\begin{proposition}\label{prop:strengthened_LB} 
    For any constant $\alpha>0$ and for $\delta = n^{-\alpha}$, there exist a small enough constant $c>0$ depending on $\alpha$ and $L$, and an absolute constant $C'$, such that, if $n \geq C'$ and if $K\leq c n^{1/4}$, then we have $c\left(K/n\right)^{1/3}\leq \varphi_\delta^*(n,\mathcal{L}_{[0,1]^2} \cap\mathcal{F}_K)$. 
\end{proposition}
The class $\mathcal{L}_{[0,1]^2} \cap\mathcal{F}_K$ is clearly smaller than $\mathcal{G}_K$, so that $\varphi_\delta^*(n,\mathcal{L}_{[0,1]^2} \cap\mathcal{F}_K) \leq \varphi_\delta^*(n,\mathcal{G}_K)$. 
Comparing Proposition~\ref{prop:strengthened_LB} with Theorem~\ref{th:densities}, one directly obtains that our procedure achieves adaptation to the unknown support at most at a logarithmic price. \\



Next we provide a histogram-style estimator outputting a density that is piecewise constant on a grid and achieves this faster rate of convergence. 
%The upper bound of Theorem~\ref{th:densities} is achieved by the Algorithm \ref{alg:Alg_densities}.
It proceeds in two steps. 
In the first step, we use sample-splitting to estimate the support $[r_1,R_1] \times [r_2,R_2]$ by the smallest rectangle of the form $[\widehat r_1, \widehat R_1]\times [\widehat r_2, \widehat R_2]$ containing all of the data points in the first half of the sample. 
In the second step, whenever possible, we split the estimated support $[\widehat r_1, \widehat R_1]\times [\widehat r_2, \widehat R_2]$ into disjoints rectangular cells of edge-lengths $h_1$ and $h_2$, where $h_1 \asymp h_2  \asymp n^{-1/3}$ and output the estimator that takes a constant value in each cell, proportional to the number of observations contained in the cell. 
However, it may be impossible to partition the rectangle $[\widehat r_1, \widehat R_1]\times [\widehat r_2, \widehat R_2]$ if $\min(\widehat R_1 - \widehat r_1, \widehat R_2 - \widehat r_2) \ll n^{-1/3}$. 
In that case, if by symmetry $\widehat R_1 - \widehat r_1 < n^{-1/3}$, the idea is to neglect the variations of $f$ with respect to $x$ due to Lipschitz continuity: $\forall x,x' \in [r_1,R_1]: f(x,\cdot\,) \approx f(x',\cdot\,)$. 
We therefore recover a $1$-dimensional estimation problem, which allows us to only partition the segment $[\widehat r_2, \widehat R_2]$ if $\widehat R_2-\widehat r_2\gtrsim n^{-1/3}$, or to estimate $f$ by a constant over $[\widehat r_1, \widehat R_1]\times [\widehat r_2, \widehat R_2]$ in the opposite case. Outside of $[\widehat r_1, \widehat R_1]\times [\widehat r_2, \widehat R_2]$ we estimate the unknown density using the histogram.
\vspace{1mm}

Next we define our algorithm. 
In what follows, without loss of generality, we assume that $n$ is a multiple of $4$. We denote by $\Pi_1$ and $\Pi_2$ the orthogonal projectors over the first and the second vector of the canonical basis, respectively: $\forall x,y \in\R: \Pi_1(x,y) = x \text{ and } \Pi_2(x,y) = y$.

\vspace{2mm}

\begin{algorithm}[H]\label{alg:Alg_densities}
\SetAlgoLined
\textbf{Input:} $X_1,\dots, X_n \in \R^2, \alpha>0$.\\

\vspace{3mm}

For $j \in [2]$, set $\widehat r_j \leftarrow \min \left\{\Pi_j(X_i): i \in \{1,\dots,\frac{n}{2}\}\right\}$ and 
$\widehat R_j \leftarrow \max \left\{\Pi_j(X_i): i \in \{1,\dots,\frac{n}{2}\}\right\}$.

\vspace{2mm}

$h^* \leftarrow n^{-1/3}L^{-1/2}$.

\vspace{2mm}

\textbf{If } $\widehat R_1 - \widehat r_1 < h^*$: 

\vspace{1mm}

\hspace{5mm} $\widehat g \leftarrow \text{Algorithm \ref{alg:Alg_densities_1D}}\big(\Pi_2(X_{n/2+1}),\dots, \Pi_2(X_{n}
)\big)$

\vspace{1mm}

\hspace{5mm} \textbf{Return} $\widehat f: (x,y) \longmapsto \frac{1}{\widehat R_1 - \widehat r_1}\mathbb 1_{x \in [\widehat r_1, \widehat R_1]} \cdot \widehat g(y)$.

\vspace{2mm}

\textbf{If } $\widehat R_2 - \widehat r_2 < h^*$:

\vspace{1mm}

\hspace{5mm} $\widehat g \leftarrow \text{Algorithm \ref{alg:Alg_densities_1D}}\big(\Pi_1(X_{n/2+1}),\dots, \Pi_1(X_{n}
)\big)$

\vspace{1mm}

\hspace{5mm} \textbf{Return} $\widehat f: (x,y) \longmapsto \widehat g(x) \cdot \frac{1}{\widehat R_2 - \widehat r_2} \mathbb 1_{y \in [\widehat r_2, \widehat R_2]}$.

\vspace{3mm}

\textbf{Else:} %\textbf{For} $j\in[2]$: $\hat m_j = \lfloor \widehat r_j/h \rfloor$, $\hat M_j = \lfloor \widehat R_j/h \rfloor$


\vspace{2mm}

\hspace{5mm}  For $j\in\{1,2\}$, set $h_j = \Big\lfloor(\widehat R_j - \widehat r_j ) n^{1/3}L^{1/2}\Big\rfloor^{-1}(\widehat R_j - \widehat r_j)$

\vspace{2mm}

\hspace{5mm} For $j\in\{1,2\}$, set $E_j = \big\{-\big\lfloor \widehat r_j/h_j\big\rfloor,\dots, \big\lceil (1-\widehat r_j)/h_j -1\big\rceil\big\}.$

\vspace{2mm}

\hspace{5mm} \textbf{For} $(j,j') \in  E_1\times E_2$: %\{\widehat m_1,\dots, \widehat M_1\} \times \{\widehat m_2,\dots, \widehat M_2\}$: 

\vspace{2mm}

\hspace{10mm} $A_j ~= \big[\widehat r_1 + jh_1, ~\widehat r_1 + (j+1)h_1\big]$

\vspace{2mm}

\hspace{10mm} $B_{j'} = \big[\widehat r_2 + j' h_2, \widehat r_2 + (j'\!+1)h_2\big]$

\vspace{2mm}

\hspace{10mm} $C_{j,j'} = A_j \times B_{j'}$.


\hspace{10mm} $N^{(1)}_{j,j'} \leftarrow \sum\limits_{i = n/2+1}^{3n/4} \mathbb 1_{X_i \in C_{j,j'}}$; ~~ $N^{(2)}_{j,j'} \leftarrow \sum\limits_{i = 3n/4+1}^{n} \mathbb 1_{X_i \in C_{j,j'}}$;



\hspace{5mm} $\widehat P \leftarrow \text{Algorithm~\ref{alg:Alg}}\Big( \frac{n}{2},\alpha, |E_1| \lor |E_2|, N^{(1)}, N^{(2)}\Big)$

\vspace{2mm}

\hspace{5mm} {\color{black} For $j\in\{1,2\}$ set $m_j = \big\lfloor(\widehat R_j - \widehat r_j ) n^{1/3}L^{1/2}\big\rfloor$}

\vspace{2mm}

\hspace{5mm} {\color{black} $\mathcal{E}' = \bigcup_{i=0}^{m_1-1} \; \bigcup_{j=0}^{m_2-1} \{(i,j)\}$}.


\textbf{Return} $\widehat f = \frac{1}{ h_1 h_2}\sum\limits_{{\color{black}(j,j') \in \mathcal{E}'}}  \widehat P_{j,j'} \,\mathbb 1_{C_{j,j'}} + {\color{black}\frac{1}{h_1 h_2}\sum\limits_{(j,j') \notin \mathcal{E}'} \frac{2}{n} (N^{(1)}_{j,j'} + N^{(2)}_{j,j'})\,\mathbb 1_{C_{j,j'}}}$. %$\widehat f = \sum\limits_{j=\widehat m_1}^{\widehat M_1} \sum\limits_{j'=\widehat m_2}^{\widehat M_2} \frac{ N_{j,j'}}{h^2} \mathbb 1_{C_{j,j'}(h)}$
\caption{Two-dimensional density estimation procedure}
\end{algorithm}






\begin{algorithm}[H]\label{alg:Alg_densities_1D}
\SetAlgoLined
\vspace{1mm}
\textbf{Input:} $Z_1,\dots, Z_n \in \R$.\\

\vspace{3mm}

$\widehat r \leftarrow \min \left\{Z_i: i \in \{1,\dots, \lfloor \frac{n}{2}\rfloor\}\right\}$; 
$\widehat R \leftarrow \max \left\{Z_i: i \in \lfloor \frac{n}{2}\rfloor\right\}$.

\vspace{3mm}

$h^* \leftarrow n^{-1/3}L^{-1/2}.$

\vspace{3mm}

\textbf{If } $\widehat R - \widehat r < h^*$, \textbf{then return} $\frac{1}{\widehat R - \widehat r} \mathbb 1_{[\widehat r, \widehat R]}$.

\vspace{2mm}

\textbf{Else:} %$\widehat m = \lfloor \widehat r/h \rfloor$, $\widehat M = \lfloor \widehat R/h \rfloor$.

\vspace{2mm}

\hspace{10mm} $h = \big\lfloor(\widehat R - \widehat r ) /h^*\big\rfloor^{-1}(\widehat R - \widehat r)$

\vspace{2mm}

\hspace{10mm} $E = \big\{-\big\lfloor \widehat r/h\big\rfloor,\dots, \big\lceil (1-\widehat r)/h -1\big\rceil\big\}.$

\vspace{2mm}

\hspace{5mm} \textbf{For} $j \in E$:  %$j \in \{\widehat m,\dots,\widehat M\}$: 

\vspace{2mm}


\hspace{10mm} $A_j = \big[\widehat r + jh, \widehat r + (j+1)h\big]$

\vspace{2mm}

\hspace{10mm} $N_j \leftarrow \sum_{i=n/2 + 1}^n \mathbb 1_{Z_i \in A_j}$
\vspace{2mm}

\textbf{Return} $\widehat g = \sum\limits_{j\in E} \frac{1}{h} N_j \, \mathbb 1_{A_j}$.\footnote{The code of Algorithms~\ref{alg:Alg_densities} and \ref{alg:Alg_densities_1D} algorithm is available at https://github.com/hi-paris/Lowrankdensity}
\caption{One-dimensional density estimation procedure}
\end{algorithm}


\section{Simulations}

We  present the results of numerical experiments on synthetic data. We have performed simulations with different values of the parameters $d, n$ and the
number of components $K$. For the experiments we
use the Python implementation of our algorithm\footnote{The code of Lowrankdensity algorithm is available at https://github.com/hi-paris/Lowrankdensity}.
In the discrete case (Figures~\ref{fig:simul_discrete} and \ref{fig:simul_discrete_log}), we compare our estimator's total variation error with that of the classical histogram estimator. 
In Figure~\ref{fig:simul_discrete}, we fix $K=1$ and $n=10^5$, and apply the two estimators on square matrices of size ranging from $d=10$ to $d=1600$. 
As seen on Figure~\ref{fig:simul_discrete}, the behavior of the histogram estimator exhibits a phase transition at $d\asymp n$, which is coherent with its classical estimation risk given by $\sqrt{\frac{d_1 d_2}{n}} \land 1 = \frac{d}{\sqrt{n}}\land 1$. 
In contrast, our estimator does not exhibit this phase transition around $d \asymp n$ since its estimation risk is given by $\sqrt{\frac{Kd}{n}} \land 1 = \sqrt{\frac{d}{n}} \land 1$. 
To better appreciate the dependency in $d$, we also represent the same experiment on a log-log plot in Figure~\ref{fig:simul_discrete_log}. 
We can see that the histogram's $\ell_1$ error is proportional to $d$ in the first regime, whereas our estimator's error is always proportional to $\sqrt{d}$ for the ranges of values represented in this figure.

\vspace{2mm}

Next, we turn our attention to the dependency of the $\ell_1$ error with respect to the rank $K$, for fixed dimension $d=100$ and fixed number of observations $n=10^5$. 
In Figure~\ref{fig:simul_discrete_K_diric}, we observe that our estimator takes advantage of the underlying structure of the problem, by performing a dimension reduction. 
To better appreciate the dependency in $K$, we also provide a log-log representation of this error, which shows that the estimation error grows as $\sqrt{K}$. 
These first two figures are obtained for low-rank matrices close to the prior set in the lower bound. 
%To present the dependency in $K$ in a more general setting, not necessarily close to the worst-case scenario, we provide in Figure~\ref{fig:simul_discrete_K} another analysis of Algorithm~\ref{alg:Alg}'s estimation error for low-rank distributions closer to the uniform distribution. In this case, the estimation error can even be decreasing with $K$, as 
%We observe that the classical histogram does not exploit of the low-rank structure of the problem, in contrast to our estimator which performs a dimension reduction. 

\vspace{2mm}

Next, we consider the density case (Figures~\ref{fig:simul_continuous} and~\ref{fig:simul_continuous_log}). 
We compare the classical estimator by histogram with bandwidth $n^{-1/4}$ with our estimator (Algorithm~\ref{alg:Alg_densities}), which uses a binning with bandwidth $n^{-1/3}$ and performs a dimension reduction based on Algorithm~\ref{alg:Alg}. 
We take $K=1$ and let $n$ vary from $1000$ to $10^6$.
Again, we observe that our estimator performs better than the classical estimator, and allows us to recover the one-dimensional estimation rate $n^{-1/3}$.

\vspace{2mm}


\begin{figure}
\begin{minipage}[b]{0.45\textwidth}
    \centering
    \includegraphics[width = 1\textwidth]{New/Simulations/L1_error_discret_wrt_d_vraie.png}
    \caption{Total variation error between our estimator from Algorithm~\ref{alg:Alg} and the probability matrix to estimate, as a function of the dimension $d$. 
    Here, we take $n=10^5$ and $K=1$.
    \phantom{ }
    }
    \label{fig:simul_discrete}
\end{minipage}
\hfill 
\begin{minipage}[b]{0.45\textwidth}
    \centering
    \includegraphics[width = 1\textwidth]{New/Simulations/log_log_discret_wrt_dpng.png}
    \caption{Total variation error between our estimator from Algorithm~\ref{alg:Alg} and the probability matrix to estimate, as a function of the dimension $d$,  presented in log-log scale. 
    Here, we take $n=10^5$ and $K=1$.}
    \label{fig:simul_discrete_log}
\end{minipage}
\end{figure}

\begin{figure}

\begin{minipage}[b]{0.45\textwidth}
    \centering
    \includegraphics[width = 1\textwidth]{New/Simulations/discret_K_dirichlet.png}
    \caption{Total variation error between the estimator from Algorithm~\ref{alg:Alg} and the probability matrix to estimate, as a function of the rank $K$. Here, $d=100$ and $n=10^5$.}
    \label{fig:simul_discrete_K_diric}
\end{minipage}
\hfill
\begin{minipage}[b]{0.45\textwidth}
    \centering
    \includegraphics[width = 1\textwidth]{New/Simulations/discret_log_k_dirichlet.png}
    \caption{Total variation error between the estimator from Algorithm~\ref{alg:Alg} and the probability matrix to estimate, as a function of  the rank $K$, in log-log scale. Here, $d=100$ and $n=10^5$.}
    \label{fig:simul_discrete_log_K_diric}
\end{minipage}
\end{figure}

\begin{figure}
\begin{minipage}[b]{0.45\textwidth}
    \centering
    \includegraphics[width = 1\textwidth]{New/Simulations/L1_error_densities.png}
    \caption{Total variation error of Algorithm~\ref{alg:Alg_densities} as a function of $n$ for $K=1$.}
    \label{fig:simul_continuous}
\end{minipage}
\hfill
\begin{minipage}[b]{0.45\textwidth}
    \centering
    \includegraphics[width = 1\textwidth]{New/Simulations/log_L1_error_densities.png}
    \caption{Total variation error of Algorithm~\ref{alg:Alg_densities} as a function of $n$ for $K=1$, in log-log scale.}
    \label{fig:simul_continuous_log}
\end{minipage}
\end{figure}


\section{Conclusion}

In this paper, we obtained minimax near-optimal estimators for the problem of multinomial estimation under low-rank matrix constraints and for density estimation over a suitably defined class of low-rank Lipschitz-continuous distributions. 
In both cases, we demonstrated that the rank constrain can substantially reduce the  worst-case estimation error. 
For the discrete problem, we highlighted that the method is not a direct application of the classical PCA, due to the heterogeneity of the noise and the geometry of the $L^1$ distance. 
For the continuous problem, we provided a near-optimal algorithm that can be constructed explicitly, in contrast to~\cite{vandermeulen2021beyond}. 
Our findings suggest that low-rank matrix constraints can be a powerful tool for reducing error in estimation problems. 
It will be interesting to extend our results on density estimation to larger-dimensional settings, in particular, to low-rank multinomial tensors, which is left for future work. 



%\ju{Attention il faut rédiger le poiss trick}

==> contents_low_rank/Upper_bound.tex <==


\subsection{Upper bound: Proof of Proposition~\ref{prop:UB}}

%\ju{Note that we need to assume properties of the matrix $P$ ensuring that $\|W\|_{op} \leq \sqrt{\|\Lambda\|_{1,\infty} \lor \|\Lambda^\top\|_{1,\infty} \log d}$ in Olga's Lemma.} 
\begin{proof}[Proof of Proposition~\ref{prop:UB}]


\textbf{\underline{Fact:}} Given any estimator $\widehat{P}$ of $P$, that is allowed to be such that $\sum\limits_{i,j} \widehat P_{ij} \neq 1$ or $\widehat P_{ij} < 0$ for some $i,j$ we can modify $\widehat P$ in order to define $\widehat P^*$ that belongs to the simplex and has the same estimation guarantees up to a factor $2$. 
Namely, let $\widehat P_+ = \left(\widehat P_{ij} \land 0 \right)_{ij}$ and $\widehat{P}^* := \frac{\widehat P_+}{\|\widehat P_+\|_1}$. Then by construction, $\widehat P^*$ is in the simplex and satisfies:
\begin{align*}
    \big\|P - \widehat P^*\big\|_1 &\leq \big\|P - \widehat P_+\big\|_1 + \big\|\widehat P_+ - \widehat P^*\big\|_1 \leq \big\|P - \widehat P\big\|_1 + \bigg\|\widehat P_+\Big(1 - \frac{1}{\big\|\widehat P_+\big\|_1}\Big)\bigg\|_1\\
    & = \big\|P - \widehat P\big\|_1 +\left|\big\|\widehat P_+\big\|_1 -1 \right| \leq \big\|P - \widehat P\big\|_1 + \big\|P - \widehat P_+\big\|_1\\
    &\leq 2  \big\|P - \widehat P\big\|_1.
\end{align*}

We now therefore focus on constructing an estimator $\widehat P$ satisfying $\|\widehat P - P\|_1 \leq C \sqrt{\frac{K(d_1+d_2)}{n}} \log^2 d$ with probability at least $1 - \frac{1}{d^\alpha}$ for a given $\alpha >0$\\

Let $\widetilde n \sim \Poi(n)$ and assume that the total number of observations is $\widetilde N = 2\widetilde n$. 
We use sample splitting to define $\Yone \sim \text{Hist}(X_1,\dots, X_{\widetilde n})$ and $\Ytwo = \text{Hist}(X_{\widetilde n+1}, \dots, X_{\widetilde N})$. By the Poissonization trick, we therefore have that $\forall i,j,l: Y^{(l)}_{ij} \sim Poi(n p_{ij})$ and that the $Y^{(l)}_{ij}$ are mutually independent.\\





We denote by $\|\cdot\|$ the operator norm and for any matrix $\Lambda $, and we write 
\begin{align*}
    &\|\Lambda\|_{1,\infty} = \max_{j} \sum_{i} |\Lambda_{ij}| ~\text{ for the maximum column norm}\\
    & \normsquare{\Lambda} = \|\Lambda\|_{1,\infty} \lor \|\Lambda^\top\|_{1,\infty},\\
    &W = \frac{\Ytwo}{n} - P.
\end{align*}

%We recall that under technical assumptions (see Olga's document) with probability $1 - \frac{1}{d}$, we have $\|W\| \leq \sqrt{\normsquare{P} \log d}$ where $d = d_1 \lor d_2$.\\

We can also express the matrices $P$ and $Y$ as the family of their columns and of their rows.
\begin{align*}
    P = \Big[C_1,\dots, C_{d_2}\Big] = \left[\begin{array}{ccc}
     \!\!L_1\!\! \\
     \!\!\vdots\!\!\\
     \!\!L_{d_1}\!\!
\end{array}\right] ~~ \text{ and } ~~ \Yl = \Big[\hatCl_1,\dots, \hatCl_{d_2}\Big] = \left[\begin{array}{ccc}
     \!\!\hatLl_1\!\! \\
     \!\!\vdots\!\!\\
     \!\!\hatLl_{d_1}\!\!
\end{array}\right], \text{ for } l=1,2.
\end{align*}

%\textbf{\underline{Idea (heuristic!)}}: The first half of the sample, represented by $\Yone$, is used to select rows and columns that have `similar' $\ell_1$ norm. More precisely, for each $t=0,\dots, O(\log(d))$, we select from $\Yone$ the indices of the rows and columns whose $\ell_1$ norms is bracketed between $\left[\frac{1}{2^{t+1}}, \frac{1}{2^t}\right]$. On these rows and columns, the noise $W$ will be roughly homogeneous by Olga's Lemma.\\

%After having selected the indices, we extract the submatrix $\Mk$ of $\Ytwo$ whose entries are those of $\Ytwo$ on each selected index and $0$ everywhere else. We perform an SVD of this matrix. We repeat for all $t=0,\dots, T$ where $T = \lfloor C_T \log d \rfloor$ and $C_T$ is a large enough absolute constant. We finally combine all of these estimators to get the final one. \\

%Let $T = \lfloor C_T \log d \rfloor$ where $C_T$ is a large enough absolute constant. 
Let $T = \lfloor \log_2 d \rfloor -1$.
For any $t \in \{0,\dots, T\}$, define 
\begin{align}
    I_t &= \bigg\{i \in [d_1]: \frac{1}{n}\big\|\hatLone\big\|_1 \in \left(\frac{1}{2^{t+1}}, \frac{1}{2^t}\right]\bigg\}, \label{def_I}\\
    J_t &= \bigg\{j \in [d_2]: \frac{1}{n}\big\|\hatCone\big\|_1 \in \left(\frac{1}{2^{t+1}}, \frac{1}{2^t}\right]\bigg\}, \label{def_I}
\end{align}

Moreover, we define 
\begin{align}
    I_{T+1} &= \bigg\{i \in [d_1]: \frac{1}{n}\big\|\hatLone\big\|_1 \leq \frac{1}{2^{T+1}}\bigg\}, \label{def_I_infty}\\
    J_{T+1} &= \bigg\{j \in [d_2]: \frac{1}{n}\big\|\hatCone\big\|_1 \leq \frac{1}{2^{T+1}}\bigg\}, \label{def_J_infty}\\
\end{align}

For any $k = (t, t') \in \{0,\dots, T+1\}^2$ we define 
\begin{align}
    &U_k = I_t \times J_{t'}.\\
    &\Mk = \frac{1}{\widetilde n}\left(\Ytwo_{ij}\,\mathbb{1}\left\{(i,j) \in U_k\right\}\right)_{i,j},\label{eq:def_Mk}\\
    &\Pk = \left(P_{ij}\,\mathbb{1}\left\{(i,j) \in U_k\right\}\right)_{i,j}, \label{eq:def_Pk}\\
    &W_k = \Mk - \Pk. \label{eq:def_Wk}
\end{align}
\ju{Faut-il diviser par $n$ ou par $\widetilde n$ dans $\Mk$?}
We prove the next lemma. 

\begin{lemma}\label{lem:concent_poisson}
There exists a large enough absolute constant $C>0$ such that for any $N,N' \geq 1$, for any $\lambda_1,\dots, \lambda_N \geq 10C\log N'$ and for mutually independent random variables $Z_1\sim \Poi(\lambda_1),\dots, Z_N \sim \Poi(\lambda_N)$, we have
$$ \mathbb{P}\left(\forall j \in [N]: Z_j\in \left[\frac{1}{2}\lambda_j, \frac{3}{2}\lambda_j\right]\right) \geq 1- \frac{2N}{{N'}^C}.$$
\end{lemma}

\begin{proof}
\begin{align*}
    \mathbb{P}\left(\exists j \in [N]: Z_j\notin \left[\frac{1}{2}\lambda_j, \frac{3}{2}\lambda_j\right]\right) &\leq \sum_{j=1}^N \mathbb{P}\left(Z_j\notin \left[\frac{1}{2}\lambda_j, \frac{3}{2}\lambda_j\right]\right) \text{ by union bound}\\
    & \leq 2\sum_{j=1}^N e^{-\lambda_j} \left(\frac{e\lambda_j}{\lambda_j/2}\right)^{\lambda_j/2} \text{ by~\cite{vershynin2018high}, exercise 2.3.3}\\
    &\leq 2N e^{-10C\log N'\left[1-\log(2e)/2\right]} \\
    &\leq 2N e^{-C\log N'} = 2\frac{N}{{N'}^C}.
\end{align*}
\end{proof}



We now assume that $n \geq 10 C K d \log d$ \ju{revoir} where $K = \rk P$ and $C$ is a large enough absolute constant. We define 
\begin{align}
    \mathcal{A}_1 & = \left\{
    \begin{array}{lll}
         \forall i \in [d_1]\,: \text{ if } \|L_i\|_1 \geq 10C\frac{\log d}{n} ~ \text{ then } ~ \frac{\|\hatLone_i\|_1}{n} \geq \frac{1}{2} \|L_i\|_1 \\
         \text{and} \\
         \forall j \in [d_2]: \text{ if } \|C_j\|_1 \geq 10C\frac{\log d}{n} ~ \text{ then } ~\frac{\|\hatCone_j\|_1}{n} \geq \frac{1}{2} \|C_j\|_1
    \end{array}
    \right\},\label{eq:def_A1}\\
    &\nonumber\\
    \mathcal{A}_2 & = \left\{\forall k \in [T\!+\!1]^2, \text{ if } \normsquare{\Pk} \geq 10C \frac{\log d}{n} \text{ then } \frac{\normsquare{\Mk}}{\normsquare{\Pk}} \in \left[\frac{1}{2}, \frac{3}{2}\right] \right\}\label{eq:def_A2} \\
    &\nonumber\\
    \mathcal{A}_3 & = \left\{\forall k \in [T+1]^2, \text{ if } \normsquare{\Pk} < 10 C \frac{\log d}{n} \text{ then } \normsquare{\Mk} < 20 C \frac{\log d}{n} \label{eq:def_A3} \right\}.
\end{align}

We now apply Lemma~\ref{lem:concent_poisson} with $N = d_1$, $\lambda_i \!=\! n\|L_i\|_1$, $N \!=\! d$ and $Z_i \!=\! \|\hatLone_i\|_1$, then reapply it with  $N \!=\! d_2$, $\lambda_j \!=\! n\|C_j\|_1$, $N \!=\! d$ and $Z_j \!=\! \|\hatCone_j\|_1$ and use a union bound.
We get $\mathbb{P}(\mathcal{A}_1) \geq 1 - 4\,d^{1-C}$, since $\|\hatLone_i\|_1 \sim \Poi(n\|L_i\|_1)$ are independent, and $\|\hatCone_j\|_1 \sim \Poi(n\|C_j\|_1)$ are independent. \\

Still by Lemma~\ref{lem:concent_poisson}, we have that $\mathbb{P}(\mathcal{A}_2| \Yone) \geq 1 - 4(T+1)^2/ d^C$, since conditionally on $\Yone$, the matrices $\Mk$ defined only through $\Ytwo$ are mutually independent. \ju{Peut-être un détail à régler car on raisonne sur la norme $\normsquare{\cdot}$ plutôt que sur les variables poisson directement}\\

\ju{Aussi analyser la proba de $\mathcal{A}_3$.}

From now on we place ourselves on $\mathcal{A}= \mathcal{A}_1 \cap \mathcal{A}_2 \cap \mathcal{A}_3$. 
Note that 
\begin{align*}
    \forall t \in \{0,\dots, T+1\}: \frac{1}{2^{t-1}} \geq \frac{1}{d} \geq 10 C \frac{\log d}{n}.
\end{align*}
Fix $k = (t,t') \in \{0,\dots, T+1\}^2$ and $(i,j) \in U_k$.
We therefore have $\frac{1}{n}\|\hatLone_i\|_1 \leq \frac{1}{2^t}$ so that by the definition of $\mathcal{A}_1$, we have 
$\|L_i\|_1 \leq  2^{1-t} \lor  10 C \frac{\log d}{n} = 2^{1-t}$ and similarly $\|C_j\|_1 \leq 2^{1-t'}$. 
By definition of $U_k$, we therefore have $\normsquare{\Pk} \leq 2^{1-t\land t'}$ on event $\mathcal{A}$. 
Moreover, $\Pk$ has rank at most $K$. 
Now, there are two cases.\\

\textbf{\underline{First case:}} If $\normsquare{\Mk} < 20 C \frac{\log d}{n}$ then, by definition of $\mathcal{A}_2$, $\normsquare{\Pk} < 40 C \frac{\log d}{n}$. In this case we define $\hatPk = \Mk$ and this estimator satisfies
    \begin{equation}\label{eq:case_1_UB}
        \|\hatPk - \Pk\|_1 \leq \|\Pk\|_1 + \|\Mk\|_1 \leq d \left[\normsquare{\Pk} + \normsquare{\Mk}\right] \leq 60 C \frac{d\log d}{n}.
    \end{equation}
\textbf{\underline{Second case:}} If $\normsquare{\Mk} \geq 20 C \frac{\log d}{n}$ then, by definition of $\mathcal{A}_3$, $\normsquare{\Pk} \geq 10 C \frac{\log d}{n}$. In this case, applying Corollary~\ref{cor:poisson_noise} with $\Lambda = n\Pk$ and $W = n W_k$, we have $\|W_k\|_{op}^2 \leq c^* \frac{\normsquare{\Pk}}{n} \log^2 d$.
Conditional on $\Yone$, we perform a hard thresholding of the SVD of $\Mk$ \ju{Give the suitable threshold} in order to get the estimator $\hatPk$. 
By the classical guarantees of the hard thresholding of the SVD, we get:\ju{référence !}
\begin{align*}
    \|\hatPk - \Pk\|_F^2 &\leq K \|W_k\|_{op}^2 \\
    &\leq K \frac{c^*}{n} \log^2 d \normsquare{\Pk}  ~~ \text{ \textit{wp } $1-\frac{1}{d}$ \ju{compléter}}\\
    & \leq \frac{c^*}{n}\frac{K \log^2 d}{2^{t\land t'-1}}.
\end{align*}

Now, note that since the entries of $\frac{1}{n}\Yone$ sum to $1$, the definition of $I_t$ and $J_t$ ensure that $|I_t| \leq 2^t \land d$ and $|J_{t'}| \leq 2^{t'} \land d$, hence that $|U_k| \leq \left(2^t \land d\right)\left(2^{t'} \land d\right)$. Therefore, the $\ell_1$ norm of $\hatPk - \Pk$ can be linked to its Frobenius norm as:
\begin{align}
    \|\hatPk - \Pk\|_1 &\leq \sqrt{|U_k|}\|\hatPk - \Pk\|_F \leq \sqrt{ \left(2^t \land d\right)\left(2^{t'} \land d\right)} \sqrt{\frac{c^*}{n}\frac{K \log^2 d}{2^{t\land t'-1}}} \nonumber \\
    & = \sqrt{(2^{t\lor t'} \land d)\frac{2 c^* K \log^2 d}{n}}
    \leq \sqrt{\frac{2 c^* K d \log^2 d}{n}}. \label{eq:case_2_UB}
\end{align}
with probability at least $1-\frac{1}{d}$. \ju{Compléter}.
We can now define
\begin{align*}
    \widehat P := \sum_{k \in \{0,\dots, T+1\}^2} \hatPk
\end{align*}
and analyze its estimation guarantees. 
We have, with probability $\geq 1 - O\left(\frac{\log d}{d^\alpha}\right)$ \ju{compléter}:
\begin{align*}
    \|\widehat P - P\|_1 &= \sum_{k \in \{0,\dots, T+1\}^2} \|\hatPk - \Pk\|_1 \\
    & \leq  \sum_{k \in \{0,\dots, T+1\}^2} 60 C \frac{d\log d}{n} + \sqrt{\frac{2K d \log^2 d}{n}} \text{ by equations~\eqref{eq:case_1_UB} and~\eqref{eq:case_2_UB}}\\
    & \leq C'\sqrt{\frac{Kd}{n}} \log^3 d,
\end{align*}
where in the third line we used the fact that $\frac{d\log d}{n} \leq \sqrt{\frac{d \log d}{n}}$ since $n \geq 10C Kd\log d$.

\end{proof}


==> contents_low_rank/Upper_bound_normalized.tex <==

\section{Proofs}
For clarity, we recall the definition of the multinomial distribution: 
Given a discrete space $\Omega$ and $P = (P_\omega)_{\omega \in \Omega}$ a (discrete) probability distribution over $\Omega$, we say that a random vector $Y$ follows $\M(P,n)$ if for all $(n_\omega)_{\omega \in \Omega} \in \N^{\Omega}$ satisfying $\sum\limits_{\omega \in \Omega} n_\omega = n$, we have:
$$ \mathbb{P}\big(\forall \omega \in \Omega: Y_\omega = n_\omega\big)= {n \choose {(n_\omega)_{\omega \in \Omega}}}\prod_{\omega \in \Omega} p_\omega^{n_\omega},$$

where ${n \choose {(n_\omega)_{\omega \in \Omega}}} = \frac{n!}{\prod_{\omega \in \Omega} n_\omega!}$.
\subsection{Proofs for discrete distributions}

%\ju{Note that we need to assume properties of the matrix $P$ ensuring that $\|W\|_{op} \leq \sqrt{\|\Lambda\|_{1,\infty} \lor \|\Lambda^\top\|_{1,\infty} \log d}$ in Olga's Lemma.} 
\begin{proof}[Proof of Proposition~\ref{prop:UB}]
\text{ }

\vspace{1mm}

\textbf{\underline{Fact:}} Given any estimator $\widehat{P}$ of $P$ which is allowed to be such that $\sum\limits_{i,j} \widehat P_{ij} \neq 1$ or $\widehat P_{ij} < 0$ for some $i,j$ we can modify $\widehat P$ in order to define $\widehat P^*$ that belongs to the simplex and has the same estimation guarantees up to a factor $2$. 
Namely, let $\widehat P_+ = \left(\widehat P_{ij} \vee 0 \right)_{ij}$ and $\widehat{P}^* := \frac{\widehat P_+}{\|\widehat P_+\|_1}$. Then by construction, $\widehat P^*$ is in the simplex and satisfies:
\begin{align*}
    \big\|P \!-\! \widehat P^*\big\|_1 &\leq \big\|P - \widehat P_+\big\|_1 + \big\|\widehat P_+ \!-\! \widehat P^*\big\|_1 \leq \big\|P \!-\! \widehat P\big\|_1 + \bigg\|\widehat P_+\Big(1 \!-\! \frac{1}{\big\|\widehat P_+\big\|_1}\Big)\bigg\|_1\\
    & = \big\|P \!-\! \widehat P\big\|_1 +\left|\big\|\widehat P_+\big\|_1 \!-\!1 \right| \leq \big\|P \!-\! \widehat P\big\|_1 + \big\|P \!-\! \widehat P_+\big\|_1\\
    &\leq 2  \big\|P \!-\! \widehat P\big\|_1.
\end{align*}

We now therefore focus on constructing an estimator $\widehat P$ satisfying $\|\widehat P \!-\! P\|_1 \leq C \sqrt{\frac{K(d_1+d_2)}{n}} \log^3 d$ with probability at least $1 - O(\frac{1}{d^\alpha})$ for a given $\alpha >0$.
In what follows, we set for readability $\alpha > 1$ and will ensure the estimation guarantee with probability $1-O(d^{1-\alpha})$.\\


%Let $\widetilde n \sim \Poi(n)$ and assume that the total number of observations is $\widetilde N = 2\widetilde n$. 
%We use sample splitting to define $H^{(1)} \sim \text{Hist}(X_1,\dots, X_{\widetilde n})$ and $H^{(2)} = \text{Hist}(X_{\widetilde n+1}, \dots, X_{\widetilde N})$. By the Poissonization trick, we therefore have that $\forall i,j,l: H^{(l)}_{ij} \sim Poi(n p_{ij})$ and that the $H^{(l)}_{ij}$ are mutually independent.\\


We prove the next lemma. 

\begin{lemma}\label{lem:concent_poisson}
Let $\alpha>0$, $N,N' \geq 1$, and $m \geq 1$. 
There exists an absolute constant $\barc$ such that for any $\lambda_1,\dots, \lambda_N \geq \frac{\alpha}{m} \barc\,\log (N') $ and for any random variables $Z_1\sim \Bin(\lambda_1,m),\dots, Z_N \sim \Bin(\lambda_N,m)$ (not necessarily independent), we have
$$ \mathbb{P}\left(\forall j \in [N]: \frac{Z_j}{m}\in \left[\frac{1}{2}\lambda_j, \frac{3}{2}\lambda_j\right]\right) \geq 1- \frac{2N}{({N'})^\alpha}.$$
\end{lemma}

\begin{proof}
%By~\cite{vershynin2018high}, exercise 2.3.5, 
It is easy to see that there exists an absolute constant $c>0$ such that
\begin{align*}
    \mathbb{P}\left(\exists j \in [N]: \frac{Z_j}{m}\notin \left[\frac{1}{2}\lambda_j, \frac{3}{2}\lambda_j\right]\right) &\leq \sum_{j=1}^N \mathbb{P}\left(\frac{Z_j}{m}\notin \left[\frac{1}{2}\lambda_j, \frac{3}{2}\lambda_j\right]\right) \text{ by union bound}\\
    & \leq 2\sum_{j=1}^N e^{-c m\lambda_j/4} ~~~ \text{ (see, e. g., \cite{vershynin2018high}, exercise 2.3.5)}\\
    &\leq 2N e^{-\frac{c}{4} \barc \alpha \log(N')} \leq 2\frac{N}{({N'})^\alpha}, ~~ \text{ taking $\barc \geq \frac{4}{c}$.}
\end{align*}
\end{proof}

We fix the constant $\barc>1$ from Lemma~\ref{lem:concent_poisson}.
If $n < \barc \alpha d \log (d)$, then our algorithm will output $\widehat P = \frac{1}{2}(\Yone + \Ytwo)$, which satisfies $ \|\widehat P - P\|_1 \leq 2 \asymp 1 \land \sqrt{\frac{Kd}{n}} \log^3(d)$.\\

From now on, we assume without loss of generality that $n \geq \barc \alpha \, d \log (d)$.
We recall the notation of Subsection~\ref{subsec:discrete_Estimator} and define 
\begin{align}
    \mathcal{A}_1 & = \left\{
    \begin{array}{lll}
         \forall i \in [d_1]\,: \text{ if } \|L_i\|_1 \geq \barc \,\alpha\frac{\log d}{n} ~ \text{ then } ~ \|\hatLone_i\|_1 \geq \frac{1}{2} \|L_i\|_1 \\
         \text{and} \\
         \forall j \in [d_2]: \text{ if } \|C_j\|_1 \geq \barc\,\alpha\frac{\log d}{n}  ~ \text{ then } \|\hatCone_j\|_1 \geq \frac{1}{2} \|C_j\|_1
    \end{array}
    \right\},\label{eq:def_A1}\\
    &\nonumber\\
    \mathcal{A}_2 & = \left\{\forall k \in [T\!+\!1]^2, \text{ if } \normsquare{\Pk} \geq \barc\,\alpha\frac{\log d}{n}  \text{ then } \frac{\normsquare{\Mk}}{\normsquare{\Pk}} \in \left[\frac{1}{2}, \frac{3}{2}\right] \right\}.\label{eq:def_A2}
    %&\nonumber\\
    %\mathcal{A}_3 & = \left\{\forall k \in [T\!+\!1]^2, \text{ if } \normsquare{\Pk} < \barc \alpha \frac{\log d}{n} \text{ then } \normsquare{\Mk} < 2\barc \alpha \frac{\log d}{n} \right\}. \label{eq:def_A3}
\end{align}

\textbf{Probability of $\mathcal{A}_1$:} We set $m\!=\!n$ and apply Lemma~\ref{lem:concent_poisson} successively with
\begin{align*}
    & N = d_1, \; \lambda_i = \|L_i\|_1,\;\, N' = d ~\text{ and }~ \frac{Z_i}{m} =  \|\hatLone_i\|_1,\\
    &N = d_2,\; \lambda_j = \|C_j\|_1,\; N' = d ~\text{ and }~ \frac{Z_j}{m} \!=\|\hatCone_j\|_1
\end{align*}
and use a union bound to get 
\begin{equation}
    \mathbb{P}(\mathcal{A}_1) \geq 1 - 4\,d^{1-\alpha}. \label{eq:proba_A1}
\end{equation}
%\ju{Ca veut dire qu'il faudra modif la proba en conséquence}

\vspace{4mm}

\textbf{Probability of $\mathcal{A}_2$ conditionally on $\Yone$:}
For any $k \in \{0,\dots,T\!+\!1\}^2$, let $Q_k \in \{\Pk, {\Pk}^\top\}$ such that $\|Q_k\|_{1,\infty} = \normsquare{\Pk}$ and let $\mu_k = \Mk$ if $Q_k = \Pk$ or $\mu_k = {\Mk}^\top$ otherwise. 
We set $\lambda_k = \|Q_k\|_{1,\infty}$ and $\frac{Z_k}{n} = \|\mu_k\|_{1,\infty}$.
We have by Lemma~\ref{lem:concent_poisson}
\begin{align*}
    \mathbb{P} \left(\overline{\mathcal{A}}_2|\Yone\right)& \leq \mathbb{P}\left(\exists k \in \{0, T\!+\!1\}^2: \frac{Z_k}{n} \notin \left[\frac{\lambda_k}{2}, \frac{3\lambda_k}{2}\right] \right)+ \mathbb{P}\left( \exists k \in \{0, T\!+\!1\}^2: \|\mu_k^\top\|_{1,\infty}> \frac{3\lambda_k}{2} \right) \\
    & \leq \frac{2(T+2)^2}{d^\alpha} + \hspace{-3mm} \sum_{k \in \{0,\dots, T+1\}^2} \hspace{-3mm} \mathbb{P}\left(\| \mu_k^\top\|_{1,\infty}> \frac{3\lambda_k}{2} \right) ~~ \text{ by Lemma~\ref{lem:concent_poisson} and a union bound}\\
    & \leq \frac{2(T+2)^2}{d^\alpha} + \hspace{-3mm} \sum_{k \in \{0,\dots, T+1\}^2} \hspace{-3mm} \mathbb{P}\left(\| \mu_k\|_{1,\infty}> \frac{3\lambda_k}{2} \right)\\
    & \leq \frac{4(T+2)^2}{d^\alpha} ~~ \text{ by Lemma~\ref{lem:concent_poisson}},\numberthis \label{eq:proba_A2}
\end{align*}
where at the third line we used the fact that, if $\lambda < \lambda'$, then for any $c>0$, it holds that $\mathbb{P}\left(\Bin(\lambda,n)>c\right) \leq \mathbb{P}\left(\Bin(\lambda',n)>c\right)$.\\


%Still by Lemma~\ref{lem:concent_poisson}, we have that $\mathbb{P}(\mathcal{A}_2| \Yone) \geq 1 - 4(T\!+\!1)^2/ d^C$, since . \ju{Peut-être un détail à régler car on raisonne sur la norme $\normsquare{\cdot}$ plutôt que sur les variables poisson directement}\\

%\textbf{Probability of $\mathcal{A}_3$ conditionally on $\Yone$:} For all $k \in \{0,\dots,T\!+\!1\}^2$, we set $\lambda_k = \normsquare{\Pk}$ and $\frac{Z_k}{n} = \normsquare{\Mk}$. We have
%\begin{align*}
    %\mathbb{P} \left(\overline{\mathcal{A}}_3|\Yone\right)& \leq \mathbb{P}\left(\exists k \in [T\!+\!1]^2, \normsquare{\Pk} < \barc \alpha \frac{\log d}{n} \text{ and } \normsquare{\Mk} \geq 2\barc \alpha \frac{\log d}{n}\right)\\
    %& \leq (T+2)^2 \mathbb{P}\left(\Bin\Big(\barc \alpha \frac{\log d}{n}, n\Big)\geq 2\barc \alpha \log d\right)\\
    %& \leq 2\frac{(T+2)^2}{d^\alpha} ~~ \text{ by Lemma~\ref{lem:concent_poisson}},\numberthis \label{eq:proba_A3}
%\end{align*}
%using again that if $\lambda < \lambda'$, then for any $c>0$, it holds that $\mathbb{P}\left(\Bin(\lambda,n)>c\right) \leq \mathbb{P}\left(\Bin(\lambda',n)>c\right)$.

\hfill



From now on we place ourselves on %$\mathcal{A}= \mathcal{A}_1 \cap \mathcal{A}_2 \cap \mathcal{A}_3$
$\mathcal{A}= \mathcal{A}_1 \cap \mathcal{A}_2$ which has probability at least $1 - O(d^{1-\alpha})$ by~\eqref{eq:proba_A1}, and \eqref{eq:proba_A2}. %and \eqref{eq:proba_A3}. 
Note that
\begin{align*}
    \forall t \in \{0,\dots, T\!+\!1\}: \frac{1}{2^{t-1}} \geq \frac{1}{d} \geq \barc \alpha \frac{\log d}{n}.
\end{align*}

Fix $k = (t,t') \in \{0,\dots, T\!+\!1\}^2$ and $(i,j) \in U_k$.
We therefore have $\|\hatLone_i\|_1 \leq \frac{1}{2^t}$ so that by the definition of $\mathcal{A}_1$, we have 
$\|L_i\|_1 \leq  2^{1-t} \lor  \barc \alpha \frac{\log d}{n} = 2^{1-t}$ and similarly $\|C_j\|_1 \leq 2^{1-t'}$. 
By definition of $U_k$, we therefore have $\normsquare{\Pk} \leq 2^{1-t\land t'}$ on event $\mathcal{A}$. 
Moreover, $\Pk$ has rank at most $K$. 
Now, there are two cases.\\

\textbf{\underline{First case:}} If $\normsquare{\Mk} < 2\barc \alpha \frac{\log d}{n}$ then, by definition of $\mathcal{A}_2$, $\normsquare{\Pk} < 4\barc \alpha \frac{\log d}{n}$. In this case we define $\hatPk = \Mk$ which yields the following guarantee
    \begin{equation}\label{eq:case_1_UB}
        \|\hatPk - \Pk\|_1 \leq \|\Pk\|_1 + \|\Mk\|_1 \leq d \left[\normsquare{\Pk} + \normsquare{\Mk}\right] \leq 6 \barc \alpha  \frac{d\log d}{n}.
    \end{equation}

\vspace{3mm}

\textbf{\underline{Second case:}} If $\normsquare{\Mk} \geq 2\barc \alpha \frac{\log d}{n}$, % then, by definition of $\mathcal{A}_3$, $\normsquare{\Pk} \geq \barc \alpha \frac{\log d}{n}$. 
then applying Proposition~\ref{prop:bound_Mult_matrix} with $Q = \Pk$ and $w_Q = W_k$, we get $\|W_k\|_{op}^2 \leq c^* \frac{\normsquare{\Pk}}{n} \log^2 d \leq c^* \frac{\log^2 d}{n}2^{1-t\land t'}$ with probability $\geq 1-3d^{-\alpha}$.
Conditional on $\Yone$, we perform a soft thresholding of the SVD of $\Mk$
\begin{align*}
    \hatPk = \arg \min_{A \in \R^{d_1\times d_2}} \|\Mk - A\|_F^2 + \tau_k \|A\|_*
\end{align*}
where $\tau_k = \sqrt{c^* \frac{\log^2 d}{n}2^{1-t\land t'}}$. 
By the classical guarantees of the soft thresholding of the SVD, there exists an absolute constant $C>0$ such that
\begin{align*}
    \|\hatPk - \Pk\|_F^2 &\leq C K \tau_k^2 
    %&\leq K \frac{c^*}{n} \log^2 d \normsquare{\Pk} ~~ \text{ with probability  $\geq 1-\frac{1}{d^\alpha}$} \\
    \leq \frac{c^*}{n}\frac{K \log^2 d}{2^{t\land t'-1}}~~ \text{ with probability  $\geq 1-\frac{1}{d^\alpha}$}.
\end{align*}

Now, note that, since the entries of $\Yone$ sum to $1$, the definitions \eqref{def_I} - \eqref{def_J} of $I_t$ and $J_t$ ensure that $|I_t| \leq 2^{t+1} \land d$ and $|J_{t'}| \leq 2^{t'+1} \land d$. Which implies that for $U_k$ defined in \eqref{def_U} we have  $|U_k| \leq \left(2^{t+1} \land d\right)\left(2^{t'+1} \land d\right)$. Next we use this bound to link the $\ell_1$ norm of $\hatPk - \Pk$  to its Frobenius norm:
\begin{align}
    \|\hatPk - \Pk\|_1 &\leq \sqrt{|U_k|}\|\hatPk - \Pk\|_F \leq \sqrt{2\cdot \left(2^t \land d\right)\left(2^{t'} \land d\right)} \sqrt{\frac{c^*}{n}\frac{K \log^2 d}{2^{t\land t'-1}}} \nonumber \\
    & = \sqrt{(2^{t\lor t'} \land d)\frac{4 c^* K \log^2 d}{n}}
    \leq \sqrt{\frac{4 c^* K d \log^2 d}{n}} \label{eq:case_2_UB}
\end{align}
with probability at least $1-\frac{1}{d^\alpha}$.
We can now define
\begin{align*}
    \widehat P := \sum_{k \in \{0,\dots, T\!+\!1\}^2} \hatPk.
\end{align*}
By a union bound, we have, with probability $\geq 1 - O\left(\frac{\log^2 d}{d^\alpha}\right)$:
\begin{align*}
    \|\widehat P - P\|_1 &= \sum_{k \in \{0,\dots, T\!+\!1\}^2} \|\hatPk - \Pk\|_1 \\
    & \leq  \sum_{k \in \{0,\dots, T\!+\!1\}^2} 6 \barc \alpha \frac{d\log d}{n} + \sqrt{\frac{4c^* K d \log^2 d}{n}} \text{ by equations~\eqref{eq:case_1_UB} and~\eqref{eq:case_2_UB}}\\
    & \leq C'\sqrt{\frac{Kd}{n}} \log^3 d ~~ \text{ for some constant $C'(\alpha)$}
\end{align*}
where in the third line we used the fact that $\frac{d\log d}{n} \leq \sqrt{\frac{d \log d}{n}}$ since $n \geq d\log d$.

\end{proof}


==> contents_low_rank/Useful_tools.tex <==
\subsection{Technical results}

\begin{proposition}\label{prop:samp_comp_TV_discrete}[Theorem 1 in~\cite{canonne2020short}]
Let $\Phi(\operatorname{TV},d,\epsilon,\delta)$ denote the sample complexity of learning discrete distributions over a known domain of size $d$, to accuracy $\epsilon>0$, with error probability $\delta \in (0,1)$ in total variation. 
Then there exist two absolute constants $C,c>0$ such that we have:
$$ c\left(\frac{d+\log(1/\delta)}{\epsilon^2}\right) \leq \Phi(\operatorname{TV},d,\epsilon,\delta) \leq C\left(\frac{d+\log(1/\delta)}{\epsilon^2}\right),$$
and the upper bound is achieved by the empirical histogram.
\end{proposition}

\subsection{Poisson approximation (Poissonization trick)}

\begin{proposition}[Poissonization trick]\label{poissonization_trick}
Let $d \geq 2$, $n \in \N^*$ and $p = (p_1,\dots, p_d)$ be a probability vector over $\{1,\dots,d\}$. For all $k \in \N^*$, denote by $\mathcal{M}(p,k)$ the multinomial distribution with parameters $p$ and $k$. Let $\widetilde n \sim \Poi(n)$ and let $\;Y\,|\, \widetilde n \sim \mathcal{M}(p,\widetilde n)$. Write $Y=(Y_1, \dots, Y_d)$, then the $Y_j$ are mutually independent and it holds $\forall j \in\{1,\dots, d\}: Y_j \sim \Poi(n p_j)$. 
\end{proposition}

In short, the Poissonization trick can be summed up as: $\mathcal{M}(p,\widetilde n) = \bigotimes\limits_{j=1}^d \Poi(np_j)$ when $\widetilde n \sim \Poi(n)$.

\begin{proof}[Proof of Proposition \ref{poissonization_trick}]
Fix $(n_1, \dots, n_d) \in \N^d$ and write $N=\sum\limits_{j=1}^d n_j$. It holds:
\begin{align}
    \mathbb{P}(Y_1 = n_1, \dots, Y_d = n_d) &= \sum_{k=0}^\infty \mathbb{P}(\widetilde n = k)~\mathbb{P}\big(Y_1 = n_1, \dots, Y_d = n_d~|~\widetilde n = k\big) \nonumber\\
    & = \mathbb{P}(\widetilde n = N) ~ \mathbb{P}\big(Y_1 = n_1, \dots, Y_d = n_d~|~\widetilde n = N\big)\nonumber \\
    &= \frac{e^{-n}n^N}{N!} {N \choose {n_1 ~ \dots ~ n_d}}\prod_{j=1}^d p_j^{n_j}\nonumber\\
    & = \prod_{j=1}^d \frac{e^{-n_j} (np_j)^{n_j}}{n_j!}. \label{independence}
\end{align}
Fixing a particular $j \in \{1,\dots, d\}$ and summing for all possible values of $(n_k)_{k\neq j}$, we first get that $\forall j: Y_j \sim \Poi(np_j)$, which, again by equation \eqref{independence}, ensures the mutual independence of the~$(Y_j)_j$.
\end{proof}

\input{contents_low_rank/Bound_stoch}

==> contents_low_rank/lower_bounds_general.tex <==
\ju{In the lemmas below, we just rewrite the above proofs in the more general case of discrete distributions written as probability vectors (we no longer impose a matrix structure)}

In what follows, we denote by $\Delta_d = \left\{p \in \R_+^d : \sum_{j=1}^d p_j = 1\right\}$ the simplex of dimension $d$.

\begin{lemma}\label{LB_expectation_general}(Lower bound in expectation for general discrete distributions)
There exists an absolute constant $c>0$ such that $$\inf_{\hat p} \sup_{p \in \Delta_d} \mathbb E \|\widehat p - p\|_1 \geq c \, \sqrt{\frac{d}{n}}.$$
\end{lemma}



\begin{lemma}\label{LB_proba_general}(Lower bound in high probability)
There exist two absolute constants $c, c'>0$ such that, for all $\delta \in (0, c')$ and any estimator $\hat p$, we have:
$$ \inf_{\hat p} \sup_{p \in \Delta_d} ~ \mathbb{P}_p\left(\|\hat p - p\|_1 \geq c \; \sqrt{\frac{d}{n}}\right) \geq \delta$$.
\end{lemma}


\begin{proof}[Proof of Lemma~\ref{LB_expectation_general}]
We define $\gamma = \mbox{\fontsize{13pt}{12pt}\(\left(\frac{\cgamma}{\sqrt{n d}}\land \frac{1}{2d}\right)\)}$ where $\cgamma$ is an absolute constant which can be chosen small enough, and we let $D_2 = \lfloor d/2 \rfloor$. 
For all $\epsilon=(\epsilon_j) \in \{\pm 1\}^{D_2}$, define the vector $p_\epsilon$ as follows:

\begin{equation}\label{def_perturbed_mat_expect_general}
    \forall j \in \big[d\big]: ~ p_\epsilon(j) =  \begin{cases}\frac{1}{d} +  \epsilon_j \gamma & \text{ if } j \leq D_2, \\ \frac{1}{d} - \epsilon_{j} \gamma & \text{ if } 2D_2 \geq j > D_2, \\  0 & \text{ otherwise,}\end{cases}
\end{equation}
Consider the set of hypotheses 
\begin{equation}\label{Hypotheses_LB_expectation_general}
\mathcal{P} = \left\{p_\epsilon ~\big|~ \epsilon \in \{\pm 1\}^{D_2} \right\}.
\end{equation}

This set contains $2^{D_2}$ hypotheses. 
Any $p \in \mathcal{P}$ has nonnegative entries summing to $1$. 
Over $\mathcal{P}$, the $\ell_1$ distance simplifies as follows:
\begin{align}
    \forall \epsilon, \epsilon' \in \{\pm 1\}^{D_2}: \|p_\epsilon - p_{\epsilon'}\|_1 = 4\gamma\; \rho(\epsilon, \epsilon'), \label{TV_Hamming_general}
\end{align}
where $\rho(\epsilon,\epsilon') = \sum\limits_{j=1}^{D_2} \mathbb{1}_{\epsilon_j \neq \epsilon'_j}$ denotes the Hamming distance between $\epsilon$ and $\epsilon'$. 

Next, we apply Assouad's Lemma (see, e.g.,  Theorem 2.12. $(ii)$ in \cite{tsybakov2008introduction}). Let $\epsilon, \epsilon' \in \{\pm 1\}^{D_2}$ such that $\rho(\epsilon,\epsilon') = 1$ and denote by $j_0 \in [D_2]$ the unique index such that $\epsilon_{j_0} = -\epsilon'_{j_0}$. 
By Lemma 2.7 in \cite{tsybakov2008introduction}, we have
\begin{align}
   TV\left(p_\epsilon^{\otimes n}, p_{\epsilon'}^{\otimes n}\right) &\leq \sqrt{\chi^2\left(p_\epsilon^{\otimes n} \; || \; p_{\epsilon'}^{\otimes n}\right)}  = \sqrt{\left(1+\chi^2\left(p_\epsilon \; || \; p_{\epsilon'}\right)\right)^n -1}, \label{TV_leq_chi2_general}
\end{align}

and 
\begin{align*}
    \chi^2\left(p_\epsilon \; || \; p_{\epsilon'}\right) &= \sum_{j=1}^{d} \frac{\left(p_{\epsilon}(j) - p_{\epsilon'}(j)\right)^2}{p_{\epsilon'}(j)} \\
    &= \frac{\left(p_{\epsilon}(j_0) - p_{\epsilon'}(j_0)\right)^2}{p_{\epsilon'}(j_0)} + \frac{\left(p_{\epsilon}(j_0+D_2) - p_{\epsilon'}(j_0+D_2)\right)^2}{p_{\epsilon'}(j_0+D_2)} \\
    & \leq  \frac{4\gamma^2}{\frac{1}{d} - \gamma} \times 2 \leq 16 \gamma^2 d ~~ \text{ since } \gamma \leq \frac{1}{2d}\\
    & = 16 \left(\frac{\cgamma^2}{n} \land \frac{1}{4d}\right) \leq 16 \frac{\cgamma^2}{n}.
\end{align*}

Therefore, by \eqref{TV_leq_chi2_general}: $TV\left(p_\epsilon^{\otimes n}, p_{\epsilon'}^{\otimes n}\right) \leq \sqrt{\exp\left(16\cgamma^2\right) - 1} \leq \frac{1}{2}$ if the absolute constant $\cgamma$ is chosen small enough. 
Now Assouad's Lemma and  \eqref{TV_leq_chi2_general} imply
$$\inf\limits_{\widehat p} \max\limits_{p \in \Delta_d} \E\left[\|\widehat p - p\|_1\right] \geq \frac{4\cgamma}{\sqrt{nd}} \frac{d}{2} \left(1-\frac{1}{2}\right) \geq \frac{\cgamma}{2} \sqrt{\frac{d}{n}} \geq \frac{\cgamma}{4}\sqrt{\frac{K(d_1+d_2)}{n}}.$$

\end{proof}

\begin{proof}[Proof of Lemma \ref{LB_proba_general}]
Recall the definition of the cubic set of hypotheses $\mathcal{P}$ from \eqref{Hypotheses_LB_expectation}.
Let $\widehat{p}$ be any estimator of the probability parameter and write
\begin{equation}\label{def_r_general}
    r = \sqrt{\frac{d}{n}}.
\end{equation}
We first justify that for this particular set of hypotheses, it is possible to assume without loss of generality that 
\begin{equation}\label{maximum_discrepancy_general}
    \|p - \widehat p\|_1 \leq 6 \gamma d \,\leq\, 6 \, \cgamma r.
\end{equation} 
Indeed, define $U = \left(\frac{1}{d} \right)_{j=1}^d$. If for some observation $Y$ the estimate $\widehat{p}(Y)$ satisfies $\|\widehat p(Y) - U\|_1 > 4\gamma d$, then it is possible to improve $\widehat{p}$ by replacing it with the estimator $\overline{p}$ satisfying $\|\overline p(Y) - p\|_1 \leq 6 \gamma d$ and defined as:
\begin{align*}
    \overline{p} := \widehat p \,\mathbb{1}\left\{\big\|\widehat p - U\big\|_1 \leq 4 \gamma d\right\} + U \mathbb{1}\left\{\big\|\widehat p - U\big\|_1 > 4 \gamma d\right\}.
\end{align*}
Indeed, recalling that $\forall p \in \mathcal{P}: \big\|U - p\big\|_1 = 2 \gamma d$, there are two cases.
\begin{itemize}
    \item If $\big\|\widehat p(Y) - U\big\|_1 \leq 4\gamma d$, then $\widehat p = \overline p$ so that $\big\|p - \overline{p}\big\|_1 \leq \big\|p - U\big\|_1 + \big\|U - \overline{p}\big\|_1 \leq 2 \gamma d + 4 \gamma d = 6 \gamma d$.
    \item  Otherwise, $\overline{p} = U$ and we get
\begin{align*}
    \big\|\overline p(Y) - p\big\|_1 & = 2\gamma d = 4 \gamma d - 2 \gamma d< \big\|\widehat p(Y) - U\big\|_1 -  \big\|U - p\big\|_1 \leq \big\|\widehat p(Y) - p\big\|_1,
\end{align*}
\end{itemize}

which proves that \eqref{maximum_discrepancy} can be assumed \textit{wlog}. Now, from the proof of Proposition \ref{LB_expectation}, we also have
\begin{align}
    \sup_{p \in \mathcal{P}} \E_p\big\|\widehat p - p\big\|_1 \, \geq \, \frac{\cgamma}{4} r =: Cr. \nonumber
\end{align}
Now, we can define $\pi := \sup\limits_{p \in \mathcal{P}} \mathbb{P}_p\left(\|\hat p - p\|_1 \geq cr\right)$ for $c = \cgamma \left(\frac{1}{4} - 6 \delta\right)> 0 $ for $\delta < \frac{1}{24} =: c'$. 
It follows that
\begin{align*}
    C r &\leq \sup_{p \in \mathcal{P}} ~ \E_p\big\|\widehat p - p\big\|_1 \\
    & = \sup_{p \in \mathcal{P}}\left\{~ \E_p\Bigg[\big\|\widehat p - p\big\|_1 \; \mathbb{1}\left\{\big\|\widehat p - p\big\|_1 \geq cr\right\}\Bigg] ~+ ~ \E_p\Bigg[\big\|\widehat p - p\big\|_1\; \mathbb{1}\left\{\big\|\widehat p - p\big\|_1 < cr\right\}\Bigg]~\right\}\\
    & \leq 6 \cgamma r \cdot \pi \, + \, cr \hspace{3mm} \text{ by equation \eqref{maximum_discrepancy}, so that } ~ \pi \geq \frac{C-c}{6\cgamma} \geq \delta.
\end{align*}

\end{proof}

